KFPA Examinations of Young STellar Object Natal Environments (KEYSTONE): Hierarchical Ammonia Structures in Galactic Giant Molecular Clouds

We present initial results from the K-band focal plane array Examinations of Young STellar Object Natal Environments (KEYSTONE) survey, a large project on the 100-m Green Bank Telescope mapping ammonia emission across eleven giant molecular clouds at distances of $0.9-3.0$ kpc (Cygnus X North, Cygnus X South, M16, M17, MonR1, MonR2, NGC2264, NGC7538, Rosette, W3, and W48). This data release includes the NH$_3$ (1,1) and (2,2) maps for each cloud, which are modeled to produce maps of kinetic temperature, centroid velocity, velocity dispersion, and ammonia column density. Median cloud kinetic temperatures range from $11.4\pm2.2$ K in the coldest cloud (MonR1) to $23.0\pm6.5$ K in the warmest cloud (M17). Using dendrograms on the NH$_3$ (1,1) integrated intensity maps, we identify 856 dense gas clumps across the eleven clouds. Depending on the cloud observed, $40-100\%$ of the clumps are aligned spatially with filaments identified in H$_2$ column density maps derived from SED-fitting of dust continuum emission. A virial analysis reveals that 523 of the 835 clumps ($\sim63\%$) with mass estimates are bound by gravity alone. We find no significant difference between the virial parameter distributions for clumps aligned with the dust-continuum filaments and those unaligned with filaments. In some clouds, however, hubs or ridges of dense gas with unusually high mass and low virial parameters are located within a single filament or at the intersection of multiple filaments. These hubs and ridges tend to host water maser emission, multiple 70$\mu$m-detected protostars, and have masses and radii above an empirical threshold for forming massive stars.

==> CygX_N_leaf_stats.tex <==
\begin{tabular}{rrrrrrlrrllrrr}
\toprule
ID & RA & decl. & PA & $\sigma_{major}$ & $\sigma_{minor}$ &  $R_{eff}$ &  $M_{obs}$ &  $M_{clip}$ &  $T_K$ &  $\sigma_{NH_3}$ &  $V_{LSR, NH_3}$ &  log($N_{para-NH_3}$) &  log($N_{H_2}$) \\& (deg) & (deg) & (deg) & ($\arcsec$) & ($\arcsec$) & (pc) & (M$_\odot$) & (M$_\odot$) & (K) & (km s$^{-1}$) & (km s$^{-1}$) & (cm$^{-2}$) & (cm$^{-2}$) \\\midrule
   0 &  310.0592 &  41.1720 &  224 &         24.7 &         15.2 &  0.26 $^{+0.17}_{-0.09}$ &   31.3 &           6.1 &  10.3 $\pm$ 1.5 &  0.16 $\pm$ 0.01 &           5.5 &            14.0 &             21.7 \\
   1 &  310.0102 &  41.1755 &  142 &         30.8 &         15.4 &  0.31 $^{+0.18}_{-0.17}$ &   43.5 &           9.7 &  10.0 $\pm$ 1.4 &  0.19 $\pm$ 0.02 &           5.3 &            14.1 &             21.7 \\
   2 &  309.9854 &  41.2135 &   46 &         23.1 &          9.5 &  0.18 $^{+0.14}_{-0.16}$ &   15.3 &           2.0 &  16.4 $\pm$ 3.8 &  0.49 $\pm$ 0.09 &          -2.7 &            14.0 &             21.7 \\
   3 &  310.1076 &  41.2606 &  115 &         19.1 &         17.0 &  0.19 $^{+0.07}_{-0.17}$ &   17.2 &           2.1 &  17.7 $\pm$ 3.7 &  0.82 $\pm$ 0.14 &          -4.5 &            14.1 &             21.7 \\
   4 &  309.7531 &  41.2946 &  219 &         36.7 &         25.5 &   0.43 $^{+0.42}_{-0.2}$ &  103.7 &          48.5 &  15.1 $\pm$ 1.8 &  0.58 $\pm$ 0.05 &           8.5 &            14.1 &             21.6 \\
   5 &  310.2244 &  41.3259 &  137 &         10.8 &          8.9 &  0.13 $^{+0.06}_{-0.04}$ &    6.4 &           1.3 &  11.0 $\pm$ 3.8 &  0.16 $\pm$ 0.04 &           5.3 &            13.9 &             21.6 \\
   6 &  309.9024 &  41.3304 &  109 &         15.4 &         11.0 &  0.19 $^{+0.07}_{-0.02}$ &   26.0 &          11.8 &  24.3 $\pm$ 2.7 &  0.41 $\pm$ 0.05 &          -2.7 &            13.8 &             21.6 \\
   7 &  309.8784 &  41.3352 &  171 &         15.1 &         12.7 &  0.22 $^{+0.01}_{-0.03}$ &   31.3 &          21.3 &  22.3 $\pm$ 1.8 &  0.45 $\pm$ 0.03 &          -2.8 &            14.1 &             21.6 \\
   8 &  309.7541 &  41.3469 &  109 &         19.2 &         12.0 &  0.23 $^{+0.06}_{-0.02}$ &   28.4 &           7.1 &  14.6 $\pm$ 1.4 &  0.43 $\pm$ 0.03 &           9.4 &            14.1 &             21.6 \\
   9 &  309.8690 &  41.3582 &  131 &         36.4 &         12.9 &  0.32 $^{+0.24}_{-0.15}$ &   59.9 &          30.4 &  20.3 $\pm$ 2.4 &  0.32 $\pm$ 0.04 &          -2.5 &            13.9 &             21.7 \\
  10 &  309.9737 &  41.4009 &  118 &         23.6 &         13.8 &   0.22 $^{+0.11}_{-0.2}$ &   30.3 &           9.2 &  16.5 $\pm$ 3.9 &  0.63 $\pm$ 0.12 &          -3.5 &            14.1 &             21.7 \\
  11 &  309.9984 &  41.4232 &   93 &         17.3 &         10.0 &  0.17 $^{+0.12}_{-0.13}$ &   14.3 &           2.8 &  14.9 $\pm$ 3.2 &  0.36 $\pm$ 0.07 &          -4.8 &            13.7 &             21.7 \\
  12 &  309.8336 &  41.4190 &  175 &         16.1 &         10.5 &  0.17 $^{+0.07}_{-0.06}$ &   16.1 &           3.1 &  19.0 $\pm$ 3.4 &  0.37 $\pm$ 0.07 &          -2.1 &            13.5 &             21.7 \\
  13 &  310.0448 &  41.4464 &  145 &          9.8 &          7.4 &  0.12 $^{+-0.0}_{-0.01}$ &    6.5 &           0.9 &  13.3 $\pm$ 2.5 &  0.22 $\pm$ 0.04 &          -5.3 &            13.7 &             21.7 \\
  14 &  310.0204 &  41.4661 &  139 &         12.2 &          9.3 &  0.15 $^{+0.01}_{-0.01}$ &   31.6 &           8.3 &  20.9 $\pm$ 1.0 &  0.49 $\pm$ 0.02 &          -4.9 &            14.2 &             21.7 \\
  15 &  310.0262 &  41.4804 &   67 &         12.7 &          8.8 &  0.15 $^{+0.02}_{-0.01}$ &   25.9 &           4.1 &  17.6 $\pm$ 0.7 &  0.32 $\pm$ 0.01 &          -3.8 &            14.2 &             21.7 \\
  16 &  310.0262 &  41.5357 &  158 &         19.6 &         15.2 &  0.31 $^{+0.13}_{-0.05}$ &  115.6 &          62.9 &  18.6 $\pm$ 1.0 &  0.53 $\pm$ 0.02 &          -4.6 &            14.3 &             21.7 \\
  17 &  310.1191 &  41.5385 &  135 &         23.4 &         11.7 &   0.23 $^{+0.1}_{-0.08}$ &   26.0 &           6.8 &  14.3 $\pm$ 3.0 &  0.31 $\pm$ 0.05 &          -5.4 &            13.4 &             21.7 \\
  18 &  309.3513 &  41.5367 &  136 &         14.2 &          5.5 &  0.11 $^{+0.07}_{-0.04}$ &   10.3 &           1.2 &  16.6 $\pm$ 2.2 &  0.68 $\pm$ 0.07 &          -2.8 &            14.0 &             21.7 \\
  19 &  310.0730 &  41.5387 &  149 &         25.7 &          7.3 &  0.17 $^{+0.14}_{-0.08}$ &   14.7 &           1.9 &  14.7 $\pm$ 3.0 &  0.22 $\pm$ 0.04 &          -4.9 &            13.9 &             21.7 \\
  20 &  309.3557 &  41.5543 &   99 &         17.7 &         14.1 &  0.22 $^{+0.08}_{-0.04}$ &   43.6 &          12.6 &  15.8 $\pm$ 1.6 &  0.76 $\pm$ 0.06 &          -2.5 &            14.0 &             21.8 \\
  21 &  309.2983 &  41.5609 &   58 &         23.8 &         14.9 &   0.26 $^{+0.12}_{-0.1}$ &   67.0 &          19.3 &  18.0 $\pm$ 2.4 &  1.21 $\pm$ 0.12 &          -2.1 &            13.8 &             21.8 \\
  22 &  309.2688 &  41.5666 &  204 &         13.4 &          7.6 &  0.13 $^{+0.04}_{-0.03}$ &   13.7 &           1.6 &  18.8 $\pm$ 3.4 &   0.63 $\pm$ 0.1 &          -1.0 &            14.0 &             21.8 \\
  23 &  309.2530 &  41.5810 &  181 &         18.3 &         13.0 &  0.24 $^{+0.07}_{-0.03}$ &   59.0 &          32.3 &  30.7 $\pm$ 2.6 &  1.01 $\pm$ 0.08 &          -1.9 &            13.7 &             21.8 \\
  24 &  310.1553 &  41.5899 &   56 &         12.5 &          9.9 &  0.15 $^{+0.05}_{-0.04}$ &    9.1 &           1.6 &  16.0 $\pm$ 3.1 &  0.19 $\pm$ 0.04 &          -6.3 &            13.3 &             21.7 \\
  25 &  309.3565 &  41.5954 &  185 &         27.5 &         13.8 &   0.3 $^{+0.21}_{-0.12}$ &   62.1 &          24.5 &  15.3 $\pm$ 2.0 &  0.56 $\pm$ 0.06 &          -1.8 &            13.9 &             21.8 \\
  26 &  309.2095 &  41.6042 &  174 &         27.1 &         25.2 &  0.38 $^{+0.25}_{-0.14}$ &  143.0 &          84.3 &  23.5 $\pm$ 1.8 &  0.79 $\pm$ 0.05 &          -2.7 &            14.2 &             21.8 \\
  27 &  310.1620 &  41.6089 &  211 &         17.2 &         11.9 &   0.2 $^{+0.07}_{-0.05}$ &   20.4 &           3.3 &  15.9 $\pm$ 3.2 &  0.24 $\pm$ 0.05 &          -5.8 &            13.8 &             21.6 \\
  28 &  309.1746 &  41.6190 &  224 &         18.1 &         13.6 &   0.17 $^{+0.1}_{-0.08}$ &   19.6 &           2.4 &  16.6 $\pm$ 3.8 &  0.77 $\pm$ 0.13 &          -3.1 &            14.3 &             21.7 \\
  29 &  310.1405 &  41.6428 &  120 &         31.9 &         23.3 &   0.43 $^{+0.24}_{-0.1}$ &  135.1 &          63.7 &  16.0 $\pm$ 1.5 &  0.38 $\pm$ 0.03 &          -5.7 &            14.0 &             21.7 \\
  30 &  309.0296 &  41.6670 &  174 &         26.2 &         15.4 &  0.35 $^{+0.08}_{-0.11}$ &   97.8 &          56.1 &  22.1 $\pm$ 1.2 &  0.75 $\pm$ 0.03 &          11.3 &            14.3 &             21.6 \\
  31 &  308.9153 &  41.7133 &  106 &         13.3 &          8.5 &  0.12 $^{+0.04}_{-0.06}$ &    5.8 &           0.9 &  11.6 $\pm$ 4.5 &  0.36 $\pm$ 0.09 &          -3.0 &            14.1 &             21.6 \\
  32 &  310.1206 &  41.7557 &  159 &         42.3 &         20.6 &  0.48 $^{+0.31}_{-0.25}$ &  193.2 &          95.2 &  17.6 $\pm$ 1.4 &  0.78 $\pm$ 0.05 &          -4.2 &            14.1 &             21.7 \\
  33 &  310.0615 &  41.7525 &  154 &         21.9 &         10.7 &   0.2 $^{+0.13}_{-0.07}$ &   19.7 &           3.1 &  15.9 $\pm$ 3.4 &  0.86 $\pm$ 0.13 &          -2.3 &            13.8 &             21.7 \\
  34 &  310.1917 &  41.8087 &  120 &         18.5 &         13.2 &  0.17 $^{+0.06}_{-0.14}$ &   13.0 &           2.2 &  20.4 $\pm$ 3.4 &  0.38 $\pm$ 0.06 &          -6.6 &            13.9 &             21.8 \\
  35 &  310.1270 &  41.8266 &  109 &         19.4 &          8.4 &  0.18 $^{+0.09}_{-0.04}$ &   59.8 &          17.7 &  18.2 $\pm$ 0.5 &  0.54 $\pm$ 0.01 &          -4.4 &            14.4 &             21.8 \\
  36 &  310.1385 &  41.8433 &  129 &         13.6 &          8.3 &  0.15 $^{+0.02}_{-0.02}$ &   49.1 &           9.5 &  18.3 $\pm$ 0.5 &  0.66 $\pm$ 0.02 &          -4.8 &            14.4 &             21.8 \\
  37 &  309.2791 &  41.8503 &  113 &         21.0 &         10.1 &  0.18 $^{+0.09}_{-0.14}$ &   13.9 &           1.1 &  16.5 $\pm$ 3.8 &    0.5 $\pm$ 0.1 &           8.8 &            13.9 &             21.7 \\
  38 &  309.1768 &  41.8540 &  132 &         18.1 &         13.7 &  0.22 $^{+0.07}_{-0.04}$ &   23.8 &           6.7 &  20.3 $\pm$ 2.7 &  0.44 $\pm$ 0.06 &          12.9 &            13.9 &             21.7 \\
  39 &  310.2647 &  41.8562 &   58 &         17.3 &          8.5 &  0.14 $^{+0.07}_{-0.07}$ &   10.7 &           1.9 &  16.9 $\pm$ 4.3 &   0.41 $\pm$ 0.1 &           0.2 &            13.8 &             21.7 \\
  40 &  310.4130 &  41.8617 &  128 &         13.4 &          9.5 &  0.16 $^{+0.03}_{-0.02}$ &    9.8 &           1.6 &  12.5 $\pm$ 3.5 &   0.53 $\pm$ 0.1 &           8.9 &            14.1 &             21.6 \\
  41 &  310.1650 &  41.8810 &  169 &         26.3 &         14.1 &   0.28 $^{+0.12}_{-0.1}$ &   60.7 &          26.7 &  20.2 $\pm$ 1.8 &  0.36 $\pm$ 0.03 &          -5.6 &            13.9 &             21.8 \\
  42 &  309.3125 &  41.8919 &  116 &         35.0 &         17.1 &  0.36 $^{+0.17}_{-0.15}$ &   57.1 &          18.0 &  14.1 $\pm$ 2.4 &   0.4 $\pm$ 0.05 &           8.2 &            13.7 &             21.7 \\
  43 &  310.1438 &  41.8935 &  150 &         13.1 &          7.1 &  0.13 $^{+0.06}_{-0.04}$ &    9.2 &           1.0 &  23.7 $\pm$ 3.9 &  0.57 $\pm$ 0.09 &          -6.4 &            13.9 &             21.8 \\
  44 &  310.1361 &  41.9072 &  218 &         10.5 &          7.5 &  0.12 $^{+0.02}_{-0.01}$ &    8.8 &           0.7 &  18.5 $\pm$ 3.9 &  0.55 $\pm$ 0.09 &          -5.7 &            13.9 &             21.8 \\
  45 &  309.1422 &  41.9126 &   59 &         12.2 &          9.5 &  0.15 $^{+0.02}_{-0.03}$ &    9.9 &           2.0 &  13.6 $\pm$ 2.7 &  0.38 $\pm$ 0.06 &          16.1 &            14.1 &             21.7 \\
  46 &  310.3367 &  41.9444 &  159 &         10.5 &          9.2 &  0.14 $^{+0.01}_{-0.02}$ &    7.4 &           0.9 &  14.6 $\pm$ 3.4 &  0.25 $\pm$ 0.05 &           8.6 &            14.0 &             21.7 \\
  47 &  310.1195 &  41.9521 &  118 &         27.1 &          8.6 &   0.2 $^{+0.21}_{-0.09}$ &   62.1 &          28.6 &  18.4 $\pm$ 0.9 &   0.5 $\pm$ 0.02 &          -6.4 &            14.3 &             21.8 \\
  48 &  310.1882 &  41.9629 &   89 &         16.0 &         14.5 &  0.22 $^{+0.02}_{-0.03}$ &   38.2 &          18.9 &  24.9 $\pm$ 2.8 &  0.58 $\pm$ 0.06 &          -7.2 &            13.9 &             21.8 \\
  49 &  310.1377 &  41.9790 &  111 &         19.1 &          7.7 &  0.16 $^{+0.08}_{-0.07}$ &   37.9 &          13.8 &  19.6 $\pm$ 1.0 &  0.49 $\pm$ 0.02 &          -6.3 &            14.1 &             21.8 \\
  50 &  309.9857 &  41.9990 &   79 &         40.0 &         20.0 &  0.43 $^{+0.22}_{-0.15}$ &  163.3 &          79.3 &  15.3 $\pm$ 1.4 &  0.53 $\pm$ 0.04 &           8.3 &            14.2 &             21.7 \\
  51 &  309.1468 &  41.9885 &  145 &         27.4 &         16.4 &   0.33 $^{+0.16}_{-0.1}$ &   71.3 &          27.8 &  14.8 $\pm$ 1.5 &  0.33 $\pm$ 0.03 &          12.3 &            13.9 &             21.7 \\
  52 &  309.1729 &  41.9833 &  140 &         12.6 &          6.5 &  0.12 $^{+0.04}_{-0.03}$ &    7.2 &           1.2 &  13.3 $\pm$ 4.5 &  0.62 $\pm$ 0.13 &          12.3 &            13.9 &             21.7 \\
  53 &  309.6347 &  41.9860 &   50 &         12.4 &          8.7 &  0.14 $^{+0.02}_{-0.05}$ &    9.0 &           0.3 &  13.0 $\pm$ 3.7 &  0.15 $\pm$ 0.03 &           3.2 &            13.5 &             21.7 \\
  54 &  309.7383 &  42.0087 &  203 &         23.3 &         16.7 &   0.3 $^{+0.06}_{-0.04}$ &   32.8 &           4.7 &  10.2 $\pm$ 2.1 &  0.14 $\pm$ 0.01 &           3.3 &            13.9 &             21.7 \\
  55 &  309.4376 &  42.0066 &  171 &         14.9 &         13.7 &  0.19 $^{+0.07}_{-0.04}$ &   17.4 &           0.8 &  13.4 $\pm$ 2.9 &  0.22 $\pm$ 0.04 &           3.2 &            13.8 &             21.8 \\
  56 &  309.4029 &  42.0207 &  125 &         39.0 &         23.3 &  0.39 $^{+0.19}_{-0.22}$ &   82.6 &          10.0 &  12.0 $\pm$ 3.3 &  0.32 $\pm$ 0.06 &           3.6 &            13.7 &             21.8 \\
  57 &  309.6569 &  42.0154 &  187 &         20.7 &         14.8 &  0.26 $^{+0.08}_{-0.07}$ &   36.4 &           5.8 &  10.9 $\pm$ 2.4 &  0.19 $\pm$ 0.03 &           3.6 &            13.8 &             21.7 \\
  58 &  309.7670 &  42.0199 &   75 &         16.1 &         12.9 &  0.21 $^{+0.05}_{-0.03}$ &   16.1 &           2.7 &  10.1 $\pm$ 2.3 &  0.15 $\pm$ 0.02 &           3.4 &            14.1 &             21.7 \\
  59 &  309.1377 &  42.0136 &   48 &          9.3 &          6.7 &  0.11 $^{+0.02}_{-0.02}$ &    5.7 &           0.6 &  13.3 $\pm$ 3.2 &  0.23 $\pm$ 0.05 &          11.9 &            14.1 &             21.7 \\
  60 &  310.1853 &  42.0250 &  115 &         21.1 &         11.4 &  0.22 $^{+0.11}_{-0.11}$ &   30.0 &           7.5 &  21.1 $\pm$ 3.3 &  0.54 $\pm$ 0.08 &          -6.3 &            13.9 &             21.7 \\
  61 &  309.9638 &  42.0287 &   77 &         13.6 &          9.1 &  0.16 $^{+0.03}_{-0.01}$ &   19.7 &           2.6 &  13.1 $\pm$ 2.6 &   0.3 $\pm$ 0.05 &           8.8 &            14.0 &             21.7 \\
  62 &  309.4327 &  42.0398 &  127 &         17.3 &          9.9 &   0.15 $^{+0.08}_{-0.1}$ &   11.1 &           1.4 &  13.0 $\pm$ 3.0 &  0.17 $\pm$ 0.03 &           3.8 &            13.3 &             21.8 \\
  63 &  309.6706 &  42.0481 &  134 &         23.1 &         14.7 &  0.25 $^{+0.09}_{-0.12}$ &   28.1 &           2.1 &  19.3 $\pm$ 3.2 &  0.41 $\pm$ 0.07 &           8.1 &            13.5 &             21.7 \\
  64 &  309.6957 &  42.0543 &  133 &         11.1 &          8.3 &  0.13 $^{+0.01}_{-0.01}$ &    7.1 &           1.2 &  13.4 $\pm$ 3.4 &  0.18 $\pm$ 0.04 &           9.0 &            13.8 &             21.7 \\
  65 &  309.4483 &  42.0560 &  172 &         18.0 &         10.5 &  0.19 $^{+0.06}_{-0.05}$ &   19.6 &           2.2 &  10.6 $\pm$ 3.2 &  0.18 $\pm$ 0.03 &           3.8 &            13.7 &             21.8 \\
  66 &  309.4124 &  42.0703 &  103 &         17.4 &         15.5 &   0.21 $^{+0.09}_{-0.1}$ &   27.7 &           3.0 &  12.6 $\pm$ 2.4 &  0.35 $\pm$ 0.05 &           4.5 &            13.6 &             21.8 \\
  67 &  309.9355 &  42.0730 &  112 &         13.1 &         10.0 &  0.15 $^{+0.05}_{-0.03}$ &   14.0 &           3.1 &  18.4 $\pm$ 3.3 &  0.37 $\pm$ 0.06 &          -6.8 &            14.0 &             21.7 \\
  68 &  309.5170 &  42.0751 &  204 &         15.5 &         10.3 &  0.16 $^{+0.07}_{-0.11}$ &   13.1 &           1.7 &  15.9 $\pm$ 3.1 &  0.36 $\pm$ 0.06 &          -2.5 &            13.8 &             21.7 \\
  69 &  309.4275 &  42.0809 &   48 &         13.5 &         10.0 &  0.14 $^{+0.07}_{-0.04}$ &   12.3 &           0.7 &  13.4 $\pm$ 2.9 &  0.33 $\pm$ 0.06 &           4.3 &            13.8 &             21.8 \\
  70 &  309.4622 &  42.0883 &  197 &         14.8 &          9.9 &  0.16 $^{+0.04}_{-0.07}$ &   14.4 &           1.8 &  18.5 $\pm$ 4.6 &  0.36 $\pm$ 0.09 &          -1.5 &            14.1 &             21.8 \\
  71 &  309.6459 &  42.1033 &  120 &         25.3 &         19.0 &  0.34 $^{+0.14}_{-0.09}$ &   78.1 &          32.0 &  19.5 $\pm$ 2.2 &  0.62 $\pm$ 0.06 &           8.1 &            13.9 &             21.7 \\
  72 &  309.1380 &  42.0943 &  187 &         22.5 &         14.6 &    0.2 $^{+0.1}_{-0.18}$ &   17.4 &           2.8 &  14.8 $\pm$ 3.7 &  0.41 $\pm$ 0.08 &          12.9 &            13.5 &             21.7 \\
  73 &  309.0885 &  42.1123 &  205 &         34.4 &         20.4 &   0.38 $^{+0.3}_{-0.17}$ &   92.9 &          32.0 &  19.1 $\pm$ 1.4 &  0.86 $\pm$ 0.05 &          14.7 &            14.0 &             21.7 \\
  74 &  309.4131 &  42.1134 &   70 &         30.0 &         14.5 &   0.27 $^{+0.2}_{-0.11}$ &   39.8 &           8.8 &  20.2 $\pm$ 2.7 &  0.43 $\pm$ 0.06 &          -0.2 &            13.9 &             21.7 \\
  75 &  309.0404 &  42.1236 &   83 &         23.8 &         10.3 &  0.19 $^{+0.12}_{-0.17}$ &   21.3 &           4.3 &  16.3 $\pm$ 2.3 &  0.52 $\pm$ 0.06 &          15.6 &            13.7 &             21.7 \\
  76 &  309.0027 &  42.1231 &  216 &         23.1 &         12.1 &  0.21 $^{+0.18}_{-0.08}$ &   25.4 &           5.4 &  14.1 $\pm$ 2.5 &  0.53 $\pm$ 0.07 &          14.1 &            14.0 &             21.7 \\
  77 &  309.9779 &  42.1204 &  187 &         12.7 &         10.2 &   0.13 $^{+0.05}_{-0.1}$ &    8.5 &           1.7 &  10.3 $\pm$ 3.2 &  0.36 $\pm$ 0.07 &           3.8 &            14.7 &             21.7 \\
  78 &  309.3160 &  42.1303 &  108 &         12.6 &          9.5 &  0.15 $^{+0.02}_{-0.04}$ &    9.8 &           1.1 &  13.7 $\pm$ 2.8 &   0.3 $\pm$ 0.05 &          15.4 &            13.7 &             21.7 \\
  79 &  309.2862 &  42.1398 &   63 &         22.9 &         16.4 &  0.31 $^{+0.13}_{-0.09}$ &   52.1 &          16.5 &  14.2 $\pm$ 1.5 &  0.52 $\pm$ 0.04 &          15.7 &            14.2 &             21.7 \\
  80 &  309.8744 &  42.1376 &  218 &         12.0 &          7.3 &  0.13 $^{+0.04}_{-0.02}$ &    8.2 &           0.9 &  20.2 $\pm$ 3.5 &   0.3 $\pm$ 0.05 &          -6.3 &            13.9 &             21.7 \\
  81 &  309.5623 &  42.1466 &   51 &         14.9 &          8.3 &  0.15 $^{+0.06}_{-0.01}$ &    8.5 &           1.4 &  11.9 $\pm$ 2.8 &  0.26 $\pm$ 0.04 &          15.9 &            13.9 &             21.7 \\
  82 &  309.1136 &  42.1478 &   66 &         17.4 &         12.3 &  0.23 $^{+0.03}_{-0.03}$ &   22.6 &           8.5 &  16.4 $\pm$ 1.7 &  0.43 $\pm$ 0.04 &          15.2 &            14.1 &             21.7 \\
  83 &  309.0186 &  42.1655 &  108 &         48.6 &         35.5 &  0.56 $^{+0.59}_{-0.41}$ &  287.0 &         115.0 &  15.5 $\pm$ 0.9 &  0.63 $\pm$ 0.03 &          14.2 &            14.3 &             21.7 \\
  84 &  309.8860 &  42.1735 &  168 &         15.3 &         10.1 &  0.17 $^{+0.05}_{-0.05}$ &   10.6 &           0.6 &  14.4 $\pm$ 3.8 &  0.61 $\pm$ 0.11 &           8.7 &            13.8 &             21.7 \\
  85 &  309.3371 &  42.1889 &  208 &         19.7 &         12.7 &  0.23 $^{+0.06}_{-0.04}$ &   34.1 &           7.8 &  16.3 $\pm$ 1.7 &  0.59 $\pm$ 0.05 &          15.9 &            14.0 &             21.7 \\
  86 &  309.2437 &  42.1952 &  174 &         24.2 &         21.6 &  0.34 $^{+0.26}_{-0.08}$ &  203.5 &         117.8 &  20.4 $\pm$ 0.4 &  0.72 $\pm$ 0.01 &          15.2 &            14.6 &             21.7 \\
  87 &  309.8118 &  42.1961 &   89 &         17.4 &          6.1 &  0.13 $^{+0.11}_{-0.08}$ &   11.3 &           0.8 &  25.0 $\pm$ 2.9 &  0.41 $\pm$ 0.05 &          -4.0 &            13.6 &             21.7 \\
  88 &  309.5867 &  42.1928 &  161 &         16.0 &         11.7 &   0.2 $^{+0.08}_{-0.05}$ &   26.5 &          13.7 &  18.7 $\pm$ 2.4 &  0.42 $\pm$ 0.05 &          -2.2 &            14.3 &             21.7 \\
  89 &  309.3550 &  42.1940 &  216 &         10.2 &          6.8 &  0.11 $^{+0.03}_{-0.01}$ &    6.6 &           0.7 &  14.4 $\pm$ 2.3 &  0.37 $\pm$ 0.05 &          14.8 &            13.6 &             21.7 \\
  90 &  309.4188 &  42.2005 &   90 &         14.5 &         11.0 &  0.18 $^{+0.01}_{-0.01}$ &   13.1 &           1.6 &  12.7 $\pm$ 2.5 &  0.24 $\pm$ 0.04 &          15.7 &            14.0 &             21.7 \\
  91 &  309.8025 &  42.2150 &   58 &         26.6 &          8.1 &  0.17 $^{+0.14}_{-0.13}$ &   17.3 &           2.4 &  26.9 $\pm$ 3.2 &  0.46 $\pm$ 0.05 &          -3.4 &            13.7 &             21.8 \\
  92 &  309.3769 &  42.2277 &   91 &         22.4 &         15.6 &  0.29 $^{+0.08}_{-0.03}$ &   84.1 &          35.7 &  18.1 $\pm$ 1.0 &  0.46 $\pm$ 0.02 &          -1.7 &            14.1 &             21.7 \\
  93 &  309.0128 &  42.2244 &  197 &         19.3 &         17.3 &   0.24 $^{+0.11}_{-0.1}$ &   39.5 &           7.8 &  18.2 $\pm$ 1.6 &  0.49 $\pm$ 0.04 &          13.9 &            13.9 &             21.7 \\
  94 &  309.2371 &  42.2193 &   91 &         10.7 &          6.8 &   0.12 $^{+0.02}_{-0.0}$ &   16.2 &           2.4 &  16.7 $\pm$ 0.6 &  0.45 $\pm$ 0.01 &          16.5 &            14.4 &             21.7 \\
  95 &  308.9313 &  42.2389 &  120 &         26.1 &         17.0 &  0.26 $^{+0.11}_{-0.23}$ &   34.7 &           9.3 &  16.5 $\pm$ 3.1 &  0.62 $\pm$ 0.09 &          14.4 &            13.9 &             21.7 \\
  96 &  309.3111 &  42.2393 &  144 &         21.5 &         10.6 &  0.18 $^{+0.11}_{-0.08}$ &   10.8 &           0.9 &  15.2 $\pm$ 3.9 &   0.4 $\pm$ 0.09 &          -1.4 &            14.0 &             21.7 \\
  97 &  309.5473 &  42.2400 &  167 &         10.6 &          8.9 &  0.14 $^{+0.05}_{-0.02}$ &    7.7 &           1.2 &  16.2 $\pm$ 2.2 &  0.29 $\pm$ 0.04 &          16.8 &            14.3 &             21.6 \\
  98 &  309.7897 &  42.2498 &  225 &         31.4 &         13.8 &   0.25 $^{+0.2}_{-0.13}$ &   39.2 &          12.5 &  22.1 $\pm$ 3.8 &   0.64 $\pm$ 0.1 &          -2.5 &            14.1 &             21.9 \\
  99 &  309.3535 &  42.2498 &  217 &         20.2 &         17.5 &  0.28 $^{+0.05}_{-0.04}$ &   64.2 &          15.4 &  17.9 $\pm$ 1.1 &  0.35 $\pm$ 0.02 &          -2.0 &            14.1 &             21.7 \\
 100 &  309.4530 &  42.2511 &  165 &         12.5 &         10.2 &  0.16 $^{+0.05}_{-0.03}$ &    9.2 &           1.0 &  14.8 $\pm$ 2.7 &  0.35 $\pm$ 0.06 &          16.5 &            14.1 &             21.7 \\
 101 &  309.8935 &  42.2556 &   78 &         15.3 &          7.3 &   0.13 $^{+0.08}_{-0.1}$ &    8.2 &           0.8 &  16.8 $\pm$ 2.8 &  1.12 $\pm$ 0.14 &          15.8 &            13.4 &             21.8 \\
 102 &  309.8170 &  42.2556 &  204 &         13.5 &          8.8 &  0.14 $^{+0.04}_{-0.04}$ &   11.6 &           1.6 &  13.9 $\pm$ 2.6 &  0.31 $\pm$ 0.05 &          -3.9 &            13.6 &             21.9 \\
 103 &  309.8425 &  42.2679 &  186 &         48.6 &         15.9 &  0.43 $^{+0.39}_{-0.22}$ &  170.4 &          85.4 &  18.3 $\pm$ 0.9 &  0.74 $\pm$ 0.03 &          18.4 &            14.3 &             21.8 \\
 104 &  309.3811 &  42.2715 &  151 &         18.3 &         13.9 &  0.18 $^{+0.06}_{-0.12}$ &   21.1 &           3.1 &  16.0 $\pm$ 3.4 &  0.45 $\pm$ 0.08 &          15.8 &            13.5 &             21.7 \\
 105 &  308.9255 &  42.2679 &   74 &         13.9 &         11.3 &  0.18 $^{+0.02}_{-0.04}$ &   19.5 &           3.7 &  19.0 $\pm$ 2.9 &  0.43 $\pm$ 0.06 &          13.2 &            13.5 &             21.7 \\
 106 &  309.1334 &  42.2816 &  133 &         27.7 &         10.3 &   0.25 $^{+0.3}_{-0.11}$ &   33.5 &           6.5 &  13.4 $\pm$ 2.1 &  0.24 $\pm$ 0.03 &           3.1 &            14.0 &             21.7 \\
 107 &  309.3264 &  42.2745 &  174 &         12.4 &          6.6 &  0.13 $^{+0.05}_{-0.02}$ &   16.1 &           2.6 &  17.9 $\pm$ 0.8 &  0.46 $\pm$ 0.02 &          17.4 &            14.3 &             21.7 \\
 108 &  309.7550 &  42.2834 &  210 &         17.3 &          9.0 &  0.17 $^{+0.06}_{-0.09}$ &   33.4 &          12.0 &  25.1 $\pm$ 2.3 &  0.92 $\pm$ 0.07 &          -1.9 &            13.9 &             22.0 \\
 109 &  309.3902 &  42.2827 &  173 &         24.6 &          8.1 &  0.16 $^{+0.17}_{-0.12}$ &   16.5 &           2.7 &  18.0 $\pm$ 4.2 &   0.4 $\pm$ 0.09 &           3.8 &            13.9 &             21.7 \\
 110 &  308.9175 &  42.2828 &  198 &         14.4 &         11.4 &  0.18 $^{+0.02}_{-0.03}$ &   20.1 &           3.7 &  20.6 $\pm$ 3.7 &  0.38 $\pm$ 0.07 &          13.0 &            13.5 &             21.7 \\
 111 &  309.7576 &  42.3078 &  205 &         30.9 &         20.9 &  0.38 $^{+0.09}_{-0.07}$ &  333.7 &         162.9 &  22.6 $\pm$ 0.8 &  0.74 $\pm$ 0.02 &          -1.9 &            14.4 &             22.0 \\
 112 &  309.4034 &  42.3107 &  165 &         14.5 &          9.8 &   0.17 $^{+0.1}_{-0.05}$ &   11.3 &           2.0 &  16.4 $\pm$ 2.4 &  0.38 $\pm$ 0.05 &          -1.5 &            13.9 &             21.7 \\
 113 &  308.8782 &  42.3063 &  224 &         13.5 &          5.3 &  0.11 $^{+0.04}_{-0.04}$ &    5.9 &           0.4 &  17.3 $\pm$ 4.5 &  0.95 $\pm$ 0.19 &          14.8 &            14.7 &             21.7 \\
 114 &  308.8895 &  42.3338 &  138 &         23.9 &         18.2 &  0.39 $^{+0.17}_{-0.13}$ &  201.7 &         151.6 &  21.2 $\pm$ 0.9 &  0.65 $\pm$ 0.02 &          15.2 &            14.4 &             21.7 \\
 115 &  309.7207 &  42.3213 &  169 &         12.5 &          7.0 &  0.13 $^{+0.04}_{-0.02}$ &   21.8 &           7.9 &  26.7 $\pm$ 3.7 &  0.68 $\pm$ 0.09 &          -2.3 &            13.8 &             22.0 \\
 116 &  309.3083 &  42.3316 &   62 &         12.6 &          9.4 &  0.15 $^{+0.05}_{-0.02}$ &   13.2 &           2.2 &  16.2 $\pm$ 3.5 &  0.37 $\pm$ 0.07 &          -0.2 &            14.0 &             21.7 \\
 117 &  309.7487 &  42.3367 &  142 &         22.9 &         10.4 &  0.21 $^{+0.11}_{-0.07}$ &  103.7 &          41.3 &  26.0 $\pm$ 1.3 &  0.71 $\pm$ 0.03 &          -2.3 &            14.2 &             22.1 \\
 118 &  309.7467 &  42.3827 &   83 &         43.1 &         10.6 &  0.28 $^{+0.41}_{-0.17}$ &  640.1 &         272.7 &  25.0 $\pm$ 0.2 &  1.25 $\pm$ 0.01 &          -3.2 &            15.0 &             22.1 \\
 119 &  309.8153 &  42.3740 &  213 &         15.1 &         11.2 &   0.2 $^{+0.05}_{-0.02}$ &   17.0 &           2.8 &  12.4 $\pm$ 1.9 &  0.29 $\pm$ 0.04 &          16.1 &            14.2 &             22.1 \\
 120 &  309.5600 &  42.3804 &  165 &         14.2 &         11.5 &   0.15 $^{+0.06}_{-0.1}$ &   10.5 &           1.3 &  16.1 $\pm$ 3.6 &  0.27 $\pm$ 0.06 &          14.2 &            13.7 &             21.7 \\
 121 &  309.5882 &  42.3792 &  164 &         14.2 &         10.4 &  0.17 $^{+0.07}_{-0.02}$ &   11.4 &           2.5 &  13.1 $\pm$ 2.7 &  0.36 $\pm$ 0.06 &          13.9 &            13.8 &             21.8 \\
 122 &  309.8773 &  42.3874 &  186 &         20.3 &         12.2 &  0.23 $^{+0.12}_{-0.06}$ &   20.0 &           3.0 &  13.3 $\pm$ 2.6 &  0.39 $\pm$ 0.06 &           8.7 &            13.9 &             21.9 \\
 123 &  309.6921 &  42.4047 &  136 &         11.0 &          6.2 &  0.12 $^{+0.02}_{-0.01}$ &   11.0 &           1.2 &  18.2 $\pm$ 1.9 &  0.46 $\pm$ 0.04 &          -2.2 &            13.7 &             22.1 \\
 124 &  309.5169 &  42.4104 &  223 &         13.9 &         13.1 &  0.19 $^{+0.04}_{-0.04}$ &   24.8 &           5.0 &  14.2 $\pm$ 1.9 &  0.33 $\pm$ 0.04 &           8.4 &            13.7 &             21.7 \\
 125 &  309.5373 &  42.4168 &  172 &         11.9 &          8.8 &  0.14 $^{+0.04}_{-0.02}$ &   14.1 &           2.3 &  15.4 $\pm$ 2.5 &  0.28 $\pm$ 0.05 &           8.2 &            13.7 &             21.7 \\
 126 &  309.7572 &  42.4205 &  114 &         18.4 &          8.0 &  0.17 $^{+0.08}_{-0.06}$ &  180.2 &          37.4 &  20.9 $\pm$ 0.2 &   0.67 $\pm$ 0.0 &          -4.1 &            15.0 &             22.1 \\
 127 &  308.7175 &  42.4215 &   61 &         19.4 &         10.3 &  0.18 $^{+0.13}_{-0.04}$ &   14.5 &           2.8 &  14.6 $\pm$ 3.7 &  0.84 $\pm$ 0.14 &           4.4 &            14.1 &             21.6 \\
 128 &  309.4521 &  42.4271 &  186 &         32.3 &         10.8 &    0.26 $^{+0.2}_{-0.1}$ &   36.0 &          12.4 &  22.3 $\pm$ 3.1 &   0.3 $\pm$ 0.05 &          -0.6 &            13.6 &             21.6 \\
 129 &  309.6767 &  42.4323 &   85 &         18.3 &         11.6 &  0.21 $^{+0.08}_{-0.03}$ &   26.4 &          10.0 &  17.6 $\pm$ 2.8 &  0.31 $\pm$ 0.05 &          -2.5 &            13.6 &             22.0 \\
 130 &  309.4163 &  42.4234 &  161 &         17.8 &          5.3 &  0.13 $^{+0.09}_{-0.06}$ &    7.7 &           0.6 &  22.6 $\pm$ 4.5 &  0.23 $\pm$ 0.06 &          -0.4 &            13.4 &             21.6 \\
 131 &  309.7146 &  42.4553 &  206 &         19.9 &         16.3 &  0.26 $^{+0.09}_{-0.07}$ &   92.8 &          39.8 &  17.8 $\pm$ 0.7 &  0.53 $\pm$ 0.02 &          -2.8 &            14.2 &             22.0 \\
 132 &  309.6871 &  42.4724 &   68 &         24.9 &          9.2 &    0.2 $^{+0.2}_{-0.07}$ &   43.4 &           9.9 &  19.9 $\pm$ 0.9 &  0.39 $\pm$ 0.02 &          -3.3 &            14.0 &             22.0 \\
 133 &  309.7463 &  42.4862 &   64 &         26.5 &         15.7 &   0.26 $^{+0.15}_{-0.1}$ &   67.1 &          15.3 &  17.7 $\pm$ 1.5 &  0.57 $\pm$ 0.05 &          -2.1 &            13.9 &             22.0 \\
 134 &  309.7195 &  42.5327 &   62 &         11.6 &          8.9 &  0.13 $^{+0.04}_{-0.02}$ &    7.6 &           0.8 &  16.7 $\pm$ 3.5 &  0.33 $\pm$ 0.07 &          -2.4 &            13.6 &             21.9 \\
 135 &  309.8030 &  42.5437 &   46 &         20.5 &         12.0 &   0.23 $^{+0.1}_{-0.05}$ &   29.1 &           7.0 &  13.9 $\pm$ 2.0 &  0.42 $\pm$ 0.05 &           8.7 &            13.9 &             21.8 \\
 136 &  309.6502 &  42.5441 &  120 &         13.2 &         10.7 &  0.13 $^{+0.05}_{-0.07}$ &    8.5 &           0.7 &  19.8 $\pm$ 3.9 &  0.64 $\pm$ 0.11 &          -3.3 &            13.8 &             21.9 \\
 137 &  309.5605 &  42.5468 &  190 &         10.2 &          8.0 &   0.12 $^{+0.0}_{-0.01}$ &    8.7 &           1.3 &  18.6 $\pm$ 1.9 &  0.64 $\pm$ 0.06 &          -2.4 &            13.6 &             21.8 \\
 138 &  309.5275 &  42.5541 &  198 &         26.0 &          9.5 &  0.22 $^{+0.21}_{-0.07}$ &   31.1 &           8.9 &  18.6 $\pm$ 1.4 &   0.4 $\pm$ 0.03 &          -1.6 &            13.9 &             21.8 \\
 139 &  309.7823 &  42.5587 &  212 &         12.8 &         10.4 &  0.15 $^{+0.03}_{-0.04}$ &   12.9 &           2.5 &  14.7 $\pm$ 2.4 &  0.31 $\pm$ 0.05 &           8.8 &            13.6 &             21.8 \\
 140 &  309.4874 &  42.5606 &  218 &         19.5 &          9.5 &  0.19 $^{+0.13}_{-0.05}$ &   15.0 &           3.4 &  20.5 $\pm$ 2.8 &  0.37 $\pm$ 0.05 &          -1.4 &            13.8 &             21.7 \\
 141 &  309.7737 &  42.5718 &  203 &         10.3 &          7.5 &   0.12 $^{+0.03}_{-0.0}$ &    7.5 &           0.6 &  13.0 $\pm$ 2.1 &  0.24 $\pm$ 0.03 &           8.6 &            13.8 &             21.8 \\
 142 &  309.6865 &  42.5758 &   79 &         12.7 &          5.4 &  0.11 $^{+0.04}_{-0.04}$ &    8.5 &           0.9 &  18.6 $\pm$ 2.7 &  0.46 $\pm$ 0.06 &          -3.0 &            13.6 &             21.9 \\
 143 &  309.7295 &  42.5934 &  213 &         22.0 &         14.7 &  0.24 $^{+0.14}_{-0.08}$ &   31.6 &           6.7 &  13.7 $\pm$ 2.4 &  0.32 $\pm$ 0.05 &           8.6 &            14.0 &             21.9 \\
 144 &  309.6780 &  42.5868 &   99 &         11.4 &          8.7 &   0.14 $^{+0.0}_{--0.0}$ &   14.9 &           2.3 &  15.4 $\pm$ 2.2 &  0.42 $\pm$ 0.05 &          -3.1 &            13.9 &             21.9 \\
 145 &  309.4921 &  42.5911 &  213 &         13.6 &          7.3 &  0.12 $^{+0.07}_{-0.03}$ &    5.3 &           0.5 &  19.4 $\pm$ 4.4 &  0.29 $\pm$ 0.07 &          -0.9 &            13.8 &             21.8 \\
 146 &  309.6459 &  42.5949 &  148 &         16.4 &          8.1 &  0.15 $^{+0.07}_{-0.05}$ &   18.3 &           4.4 &  13.5 $\pm$ 1.7 &   0.3 $\pm$ 0.03 &          -2.6 &            13.9 &             21.9 \\
 147 &  309.6988 &  42.6064 &   49 &         16.5 &          8.7 &  0.14 $^{+0.05}_{-0.08}$ &   16.1 &           2.0 &  15.2 $\pm$ 2.9 &   0.66 $\pm$ 0.1 &           8.6 &            13.8 &             21.9 \\
 148 &  309.6301 &  42.6034 &  161 &         17.2 &          9.4 &  0.17 $^{+0.09}_{-0.04}$ &   25.3 &           9.9 &  26.2 $\pm$ 1.8 &  0.77 $\pm$ 0.05 &           9.3 &            13.8 &             21.9 \\
 149 &  309.6446 &  42.6285 &  194 &         39.8 &         21.6 &   0.5 $^{+0.18}_{-0.19}$ &  464.1 &         374.6 &  26.8 $\pm$ 0.6 &  0.91 $\pm$ 0.02 &           9.5 &            14.5 &             21.9 \\
 150 &  308.6955 &  42.6118 &  166 &         16.6 &          9.5 &   0.15 $^{+0.1}_{-0.06}$ &    8.4 &           1.2 &  14.2 $\pm$ 3.7 &  0.48 $\pm$ 0.09 &           3.7 &            14.0 &             21.6 \\
 151 &  309.5721 &  42.6168 &  200 &         19.7 &          9.5 &  0.19 $^{+0.09}_{-0.06}$ &   37.6 &           9.5 &  14.3 $\pm$ 0.7 &  0.34 $\pm$ 0.01 &          -2.6 &            14.1 &             21.9 \\
 152 &  309.7220 &  42.6238 &  210 &         16.4 &         10.7 &   0.2 $^{+0.04}_{-0.04}$ &   28.9 &          10.2 &  15.0 $\pm$ 1.2 &  0.24 $\pm$ 0.02 &           9.8 &            14.1 &             21.9 \\
 153 &  309.5459 &  42.6318 &   63 &         17.8 &         12.2 &  0.21 $^{+0.06}_{-0.04}$ &   60.1 &          23.4 &  15.4 $\pm$ 0.6 &  0.42 $\pm$ 0.01 &          -2.1 &            14.2 &             21.9 \\
 154 &  309.7519 &  42.6287 &  197 &         16.4 &         11.4 &  0.19 $^{+0.05}_{-0.03}$ &   18.9 &           2.6 &  15.8 $\pm$ 3.1 &  0.39 $\pm$ 0.07 &          10.1 &            13.3 &             21.8 \\
 155 &  309.6937 &  42.6317 &   56 &         10.5 &          7.2 &   0.12 $^{+0.02}_{-0.0}$ &   16.2 &           1.0 &  18.5 $\pm$ 1.9 &  0.46 $\pm$ 0.04 &          10.0 &            14.0 &             21.9 \\
 156 &  309.5957 &  42.6374 &   78 &         21.3 &         11.3 &  0.22 $^{+0.12}_{-0.05}$ &   36.1 &           7.2 &  15.0 $\pm$ 1.3 &  0.32 $\pm$ 0.03 &          -3.0 &            13.9 &             21.9 \\
 157 &  308.7366 &  42.6323 &   50 &         15.9 &          9.1 &  0.17 $^{+0.06}_{-0.03}$ &   12.2 &           1.8 &  14.1 $\pm$ 2.0 &  0.38 $\pm$ 0.05 &          11.6 &            14.1 &             21.6 \\
 158 &  309.4807 &  42.6376 &   80 &         10.8 &          7.0 &   0.12 $^{+0.03}_{-0.0}$ &   15.7 &           1.8 &  15.7 $\pm$ 0.7 &  0.35 $\pm$ 0.01 &          -1.0 &            14.1 &             21.8 \\
 159 &  309.5647 &  42.6559 &  150 &         22.6 &         18.7 &   0.3 $^{+0.06}_{-0.05}$ &   76.3 &          24.5 &  15.1 $\pm$ 1.1 &  0.38 $\pm$ 0.02 &          -2.6 &            14.0 &             21.9 \\
 160 &  309.4509 &  42.6447 &  180 &         15.4 &          4.3 &  0.12 $^{+0.06}_{-0.03}$ &   14.3 &           1.9 &  17.0 $\pm$ 0.9 &  0.42 $\pm$ 0.02 &          -0.8 &            14.1 &             21.8 \\
 161 &  309.4718 &  42.6494 &  150 &         11.8 &          6.6 &  0.12 $^{+0.02}_{-0.03}$ &   12.9 &           0.9 &  15.4 $\pm$ 0.8 &   0.4 $\pm$ 0.02 &          -0.7 &            14.1 &             21.8 \\
 162 &  309.3975 &  42.6564 &  193 &         21.4 &         13.0 &   0.26 $^{+0.1}_{-0.06}$ &   37.0 &           9.9 &  14.3 $\pm$ 1.5 &  0.26 $\pm$ 0.03 &          -0.2 &            13.9 &             21.7 \\
 163 &  309.6400 &  42.6663 &  140 &         29.0 &         19.1 &  0.37 $^{+0.27}_{-0.12}$ &  157.1 &          75.8 &  17.8 $\pm$ 0.9 &  0.61 $\pm$ 0.03 &          12.8 &            14.3 &             21.9 \\
 164 &  308.7055 &  42.6604 &  111 &         23.9 &         15.9 &   0.3 $^{+0.09}_{-0.09}$ &   42.7 &          12.0 &  12.6 $\pm$ 1.5 &  0.26 $\pm$ 0.03 &          12.7 &            14.1 &             21.6 \\
 165 &  309.5200 &  42.6644 &  192 &         21.9 &         17.9 &  0.29 $^{+0.05}_{-0.07}$ &  169.1 &          65.2 &  14.9 $\pm$ 0.3 &  0.38 $\pm$ 0.01 &          -2.3 &            14.5 &             21.9 \\
 166 &  309.5855 &  42.6741 &   66 &         13.1 &         12.9 &  0.18 $^{+-0.0}_{-0.01}$ &   24.9 &           3.0 &  14.7 $\pm$ 0.9 &  0.32 $\pm$ 0.02 &          -3.2 &            14.1 &             21.9 \\
 167 &  309.4875 &  42.6796 &  220 &         25.1 &         11.6 &  0.24 $^{+0.11}_{-0.06}$ &   92.8 &          24.8 &  15.2 $\pm$ 0.4 &  0.46 $\pm$ 0.01 &          -1.4 &            14.4 &             21.8 \\
 168 &  309.3559 &  42.6788 &  201 &         20.9 &         11.0 &  0.22 $^{+0.12}_{-0.07}$ &   22.2 &           4.0 &  13.9 $\pm$ 2.6 &  0.27 $\pm$ 0.04 &           0.4 &            13.9 &             21.7 \\
 169 &  309.4270 &  42.6841 &  121 &         16.8 &         11.5 &  0.19 $^{+0.14}_{-0.06}$ &   17.7 &           3.6 &  12.0 $\pm$ 3.0 &  0.31 $\pm$ 0.05 &          -0.3 &            14.0 &             21.8 \\
 170 &  309.3949 &  42.6803 &  126 &         21.9 &          8.3 &  0.16 $^{+0.09}_{-0.09}$ &   11.3 &           0.8 &  17.1 $\pm$ 3.8 &  0.26 $\pm$ 0.06 &          -0.3 &            13.4 &             21.7 \\
 171 &  309.7012 &  42.6796 &   97 &         12.0 &          6.5 &  0.11 $^{+0.02}_{-0.04}$ &    7.9 &           1.3 &  16.7 $\pm$ 3.4 &  0.66 $\pm$ 0.11 &          11.8 &            14.1 &             21.8 \\
 172 &  309.6025 &  42.6962 &  113 &         32.6 &          9.2 &   0.23 $^{+0.2}_{-0.11}$ &   40.0 &           6.8 &  14.7 $\pm$ 1.0 &  0.35 $\pm$ 0.02 &          -3.1 &            13.9 &             21.9 \\
 173 &  309.7123 &  42.6953 &   92 &         15.4 &         12.1 &   0.2 $^{+0.06}_{-0.02}$ &   23.5 &           2.8 &  15.1 $\pm$ 1.8 &  0.28 $\pm$ 0.03 &          12.9 &            13.9 &             21.8 \\
 174 &  308.8052 &  42.6920 &  199 &         10.6 &          6.6 &  0.12 $^{+0.02}_{-0.02}$ &    6.1 &           0.4 &  15.9 $\pm$ 3.7 &  0.56 $\pm$ 0.11 &          10.8 &            13.9 &             21.6 \\
 175 &  309.5203 &  42.6991 &  134 &         15.4 &          9.6 &  0.17 $^{+0.04}_{-0.05}$ &   13.3 &           2.1 &  17.2 $\pm$ 3.3 &  0.31 $\pm$ 0.06 &          -2.0 &            13.5 &             21.8 \\
 176 &  309.3899 &  42.7017 &  222 &         20.8 &          8.4 &  0.15 $^{+0.15}_{-0.05}$ &    9.4 &           2.3 &  14.2 $\pm$ 4.1 &  0.34 $\pm$ 0.09 &          -1.2 &            14.0 &             21.7 \\
 177 &  309.4653 &  42.7065 &   56 &         14.0 &          8.7 &  0.15 $^{+0.05}_{-0.02}$ &   12.3 &           2.2 &  12.8 $\pm$ 2.8 &  0.35 $\pm$ 0.06 &          -1.0 &            13.8 &             21.8 \\
 178 &  309.5005 &  42.7174 &  127 &         16.4 &          8.4 &  0.16 $^{+0.09}_{-0.02}$ &    9.4 &           1.5 &  14.6 $\pm$ 3.2 &  0.27 $\pm$ 0.06 &          -1.1 &            13.5 &             21.8 \\
 179 &  309.3741 &  42.7182 &   47 &         17.2 &          9.3 &  0.17 $^{+0.12}_{-0.05}$ &   11.8 &           1.8 &  15.4 $\pm$ 3.5 &  0.49 $\pm$ 0.09 &          -0.7 &            13.8 &             21.7 \\
 180 &  309.4436 &  42.7264 &  225 &         25.2 &         14.3 &  0.29 $^{+0.16}_{-0.07}$ &   50.0 &          17.1 &  14.4 $\pm$ 1.8 &  0.34 $\pm$ 0.04 &          -0.9 &            13.9 &             21.7 \\
 181 &  308.8296 &  42.7309 &  105 &         27.0 &         10.5 &   0.24 $^{+0.19}_{-0.1}$ &   28.0 &           7.7 &  17.1 $\pm$ 2.8 &  0.44 $\pm$ 0.06 &          12.8 &            14.0 &             21.6 \\
 182 &  309.5981 &  42.7297 &  123 &         18.7 &          8.3 &  0.16 $^{+0.08}_{-0.08}$ &   11.8 &           1.5 &  15.8 $\pm$ 4.4 &   0.3 $\pm$ 0.08 &          -2.9 &            13.8 &             21.8 \\
 183 &  309.4205 &  42.7468 &  142 &         12.5 &         10.2 &  0.16 $^{+0.02}_{-0.01}$ &   12.3 &           1.9 &  13.9 $\pm$ 2.9 &  0.32 $\pm$ 0.06 &          -0.3 &            13.7 &             21.7 \\
 184 &  309.4080 &  42.7591 &   89 &         16.2 &         11.4 &  0.19 $^{+0.03}_{-0.02}$ &   20.1 &           2.8 &  12.4 $\pm$ 2.3 &  0.25 $\pm$ 0.04 &           0.2 &            13.6 &             21.7 \\
 185 &  309.3775 &  42.7798 &   48 &         18.0 &         14.6 &  0.24 $^{+0.06}_{-0.03}$ &   34.2 &          11.8 &  12.6 $\pm$ 2.0 &  0.23 $\pm$ 0.03 &           0.2 &            13.8 &             21.6 \\
 186 &  308.9387 &  42.8101 &  102 &         23.0 &         11.8 &  0.24 $^{+0.12}_{-0.09}$ &   38.2 &           7.2 &  16.5 $\pm$ 2.4 &  0.42 $\pm$ 0.05 &          11.4 &            14.1 &             21.7 \\
 187 &  309.2974 &  42.8052 &  171 &         16.6 &          9.0 &   0.15 $^{+0.1}_{-0.08}$ &   10.7 &           2.1 &  13.0 $\pm$ 4.0 &  0.44 $\pm$ 0.09 &           2.0 &            13.8 &             21.6 \\
 188 &  309.2772 &  42.8128 &  192 &         16.8 &         10.5 &  0.18 $^{+0.07}_{-0.03}$ &   16.8 &           2.7 &  12.3 $\pm$ 3.6 &  0.35 $\pm$ 0.06 &           2.1 &            13.3 &             21.6 \\
 189 &  308.9723 &  42.8216 &   82 &         22.7 &         13.4 &   0.2 $^{+0.18}_{-0.07}$ &   24.3 &           3.4 &  12.2 $\pm$ 4.4 &  0.54 $\pm$ 0.12 &           4.8 &            14.3 &             21.7 \\
 190 &  309.2436 &  42.8218 &  200 &         15.8 &         11.8 &  0.21 $^{+0.07}_{-0.04}$ &   24.6 &           7.6 &  15.9 $\pm$ 1.9 &  0.39 $\pm$ 0.04 &           2.3 &            13.8 &             21.6 \\
 191 &  309.2739 &  42.8413 &  219 &         11.5 &          7.8 &  0.13 $^{+0.01}_{-0.01}$ &    7.2 &           1.0 &  15.3 $\pm$ 3.0 &   0.2 $\pm$ 0.04 &           1.6 &            13.6 &             21.6 \\
 192 &  309.1533 &  42.8527 &  193 &         33.9 &         21.0 &  0.45 $^{+0.31}_{-0.14}$ &  177.9 &         110.2 &  16.8 $\pm$ 1.0 &  0.51 $\pm$ 0.03 &          12.9 &            14.3 &             21.5 \\
 193 &  309.0271 &  42.8422 &  105 &         13.1 &         10.6 &  0.15 $^{+0.05}_{-0.08}$ &   11.9 &           1.1 &  22.0 $\pm$ 4.6 &  0.92 $\pm$ 0.16 &          10.1 &            14.2 &             21.6 \\
 194 &  308.9552 &  42.8811 &  171 &         34.0 &         14.8 &  0.35 $^{+0.19}_{-0.16}$ &    NaN &           NaN &  13.0 $\pm$ 1.7 &  0.33 $\pm$ 0.04 &           3.9 &            14.1 &              NaN \\
 195 &  309.0956 &  42.8832 &   48 &         18.6 &          9.1 &   0.15 $^{+0.08}_{-0.1}$ &    NaN &           NaN &  17.5 $\pm$ 2.5 &  0.73 $\pm$ 0.09 &          11.6 &            13.9 &              NaN \\
 196 &  309.0671 &  42.8808 &   46 &         13.5 &         10.1 &  0.17 $^{+0.07}_{-0.02}$ &    NaN &           NaN &  14.1 $\pm$ 1.5 &  0.48 $\pm$ 0.04 &          11.9 &            14.3 &              NaN \\
 197 &  309.0100 &  42.8825 &  111 &         15.7 &          7.2 &  0.13 $^{+0.08}_{-0.07}$ &    NaN &           NaN &  15.0 $\pm$ 4.4 &  0.88 $\pm$ 0.19 &          10.9 &            14.1 &              NaN \\
 198 &  309.1893 &  42.9114 &  157 &         33.0 &         17.8 &  0.37 $^{+0.38}_{-0.13}$ &    NaN &           NaN &  14.9 $\pm$ 1.3 &  0.35 $\pm$ 0.03 &          11.6 &            14.2 &              NaN \\
 199 &  309.1178 &  42.9102 &  105 &         14.8 &          8.0 &  0.14 $^{+0.04}_{-0.04}$ &    NaN &           NaN &  13.9 $\pm$ 4.1 &   0.48 $\pm$ 0.1 &          11.7 &            14.1 &              NaN \\
\bottomrule
\end{tabular}


==> CygX_N_leaf_stats_virial.tex <==
\begin{tabular}{rrrrrrrrllrr}
\toprule
 ID &  $\alpha_{vir}$ &  $M_{vir}$ &  $\sigma_{nt}$ & log$|\Omega_G|$ & log$\Omega_K$ & log$|\Omega_{Pw}|$ &  log$|\Omega_{Pt}|$ & on-filament & hub & $N_{proto}$ & Bad N(H$_2$) Pixels \\& & (M$_\odot$) & (km s$^{-1}$) & (erg) & (erg) & (erg) & (erg) & & & \\\midrule
   0 &   0.45 &              14.0 &      0.14 &  44.3 &     43.7 &     44.8 &         NaN &         True &  False &           0 &      0.00 \\
   1 &   0.45 &              19.6 &      0.18 &  44.5 &     43.9 &     45.0 &         NaN &         True &  False &           0 &      0.00 \\
   2 &   3.10 &              47.4 &      0.48 &  43.8 &     44.1 &     44.3 &         NaN &        False &  False &           0 &      0.00 \\
   3 &   7.48 &             128.5 &      0.81 &  43.9 &     44.6 &     44.4 &         NaN &         True &  False &           0 &      0.00 \\
   4 &   1.47 &             152.6 &      0.57 &  45.1 &     45.1 &     45.4 &         NaN &        False &  False &           3 &      0.00 \\
   5 &   1.17 &               7.5 &      0.14 &  43.2 &     43.1 &     43.8 &         NaN &        False &  False &           1 &      0.00 \\
   6 &   1.65 &              42.9 &      0.39 &  44.3 &     44.3 &     44.3 &         NaN &        False &  False &           1 &      0.00 \\
   7 &   1.78 &              55.8 &      0.44 &  44.4 &     44.4 &     44.5 &         NaN &        False &  False &           1 &      0.00 \\
   8 &   1.73 &              49.0 &      0.43 &  44.3 &     44.3 &     44.5 &         NaN &        False &  False &           1 &      0.00 \\
   9 &   0.82 &              49.2 &      0.31 &  44.8 &     44.5 &     45.0 &         NaN &        False &  False &           1 &      0.00 \\
  10 &   2.95 &              89.4 &      0.62 &  44.3 &     44.6 &     44.5 &         NaN &        False &  False &           0 &      0.00 \\
  11 &   1.97 &              28.2 &      0.35 &  43.8 &     43.9 &     44.3 &         NaN &        False &  False &           1 &      0.00 \\
  12 &   1.89 &              30.5 &      0.36 &  43.9 &     44.0 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
  13 &   1.45 &               9.5 &      0.20 &  43.3 &     43.2 &     43.8 &         NaN &         True &  False &           0 &      0.00 \\
  14 &   1.35 &              42.7 &      0.48 &  44.5 &     44.5 &     44.1 &         NaN &         True &  False &           1 &      0.00 \\
  15 &   0.86 &              22.3 &      0.31 &  44.4 &     44.1 &     44.1 &         NaN &         True &  False &           0 &      0.00 \\
  16 &   0.85 &              98.4 &      0.53 &  45.3 &     45.1 &     45.0 &         NaN &        False &  False &           1 &      0.00 \\
  17 &   1.12 &              29.1 &      0.29 &  44.2 &     44.0 &     44.6 &         NaN &        False &  False &           0 &      0.00 \\
  18 &   5.15 &              52.9 &      0.67 &  43.7 &     44.2 &     43.8 &         NaN &        False &  False &           0 &      0.00 \\
  19 &   1.01 &              14.9 &      0.20 &  43.8 &     43.6 &     44.3 &         NaN &        False &  False &           0 &      0.00 \\
  20 &   3.00 &             130.7 &      0.76 &  44.6 &     44.9 &     44.7 &         NaN &        False &  False &           2 &      0.00 \\
  21 &   5.49 &             367.5 &      1.21 &  44.9 &     45.5 &     44.9 &         NaN &         True &  False &           2 &      0.00 \\
  22 &   3.91 &              53.5 &      0.62 &  43.9 &     44.3 &     44.0 &         NaN &         True &  False &           0 &      0.00 \\
  23 &   4.12 &             243.1 &      1.00 &  44.9 &     45.3 &     44.8 &         NaN &         True &  False &           1 &      0.00 \\
  24 &   1.33 &              12.2 &      0.17 &  43.5 &     43.4 &     44.0 &         NaN &        False &  False &           0 &      0.00 \\
  25 &   1.62 &             100.6 &      0.55 &  44.8 &     44.8 &     45.1 &         NaN &        False &  False &           3 &      0.00 \\
  26 &   1.72 &             245.5 &      0.78 &  45.4 &     45.5 &     45.4 &         NaN &        False &  False &           2 &      0.00 \\
  27 &   0.99 &              20.1 &      0.22 &  44.0 &     43.8 &     44.4 &         NaN &        False &  False &           0 &      0.00 \\
  28 &   5.21 &             102.3 &      0.76 &  44.1 &     44.6 &     44.3 &         NaN &        False &  False &           0 &      0.00 \\
  29 &   0.57 &              76.8 &      0.37 &  45.3 &     44.9 &     45.4 &         NaN &        False &  False &           5 &      0.00 \\
  30 &   2.14 &             209.0 &      0.74 &  45.1 &     45.3 &     45.1 &         NaN &        False &  False &           3 &      0.00 \\
  31 &   3.23 &              18.7 &      0.35 &  43.2 &     43.5 &     43.7 &         NaN &        False &  False &           0 &      0.00 \\
  32 &   1.54 &             297.2 &      0.77 &  45.6 &     45.6 &     45.6 &         NaN &        False &  False &           1 &      0.00 \\
  33 &   7.36 &             145.1 &      0.85 &  44.0 &     44.7 &     44.5 &         NaN &        False &  False &           0 &      0.00 \\
  34 &   2.54 &              32.9 &      0.37 &  43.7 &     43.9 &     44.3 &         NaN &        False &  False &           0 &      0.00 \\
  35 &   0.97 &              58.0 &      0.53 &  45.0 &     44.8 &     44.4 &         NaN &        False &  False &           2 &      0.00 \\
  36 &   1.38 &              67.5 &      0.66 &  44.9 &     44.9 &     44.2 &         NaN &        False &  False &           0 &      0.00 \\
  37 &   3.76 &              52.2 &      0.50 &  43.7 &     44.1 &     44.3 &         NaN &        False &  False &           0 &      0.00 \\
  38 &   2.23 &              53.1 &      0.43 &  44.1 &     44.3 &     44.6 &         NaN &        False &  False &           0 &      0.00 \\
  39 &   2.68 &              28.7 &      0.40 &  43.6 &     43.9 &     44.0 &         NaN &        False &  False &           0 &      0.00 \\
  40 &   4.97 &              48.7 &      0.53 &  43.5 &     44.0 &     44.1 &         NaN &        False &  False &           1 &      0.00 \\
  41 &   0.84 &              50.7 &      0.35 &  44.8 &     44.5 &     45.0 &         NaN &        False &  False &           4 &      0.00 \\
  42 &   1.18 &              67.2 &      0.39 &  44.7 &     44.5 &     45.2 &         NaN &        False &  False &           0 &      0.00 \\
  43 &   5.29 &              48.6 &      0.56 &  43.5 &     44.0 &     44.0 &         NaN &        False &  False &           0 &      0.00 \\
  44 &   4.53 &              40.0 &      0.54 &  43.5 &     44.0 &     43.9 &         NaN &        False &  False &           1 &      0.00 \\
  45 &   2.63 &              26.0 &      0.37 &  43.5 &     43.7 &     44.1 &         NaN &        False &  False &           0 &      0.00 \\
  46 &   1.96 &              14.5 &      0.24 &  43.3 &     43.4 &     44.0 &         NaN &         True &  False &           0 &      0.00 \\
  47 &   0.94 &              58.4 &      0.50 &  45.0 &     44.8 &     44.6 &         NaN &         True &  False &           1 &      0.00 \\
  48 &   2.21 &              84.4 &      0.57 &  44.5 &     44.7 &     44.7 &         NaN &         True &  False &           1 &      0.00 \\
  49 &   1.18 &              44.9 &      0.48 &  44.7 &     44.5 &     44.3 &         NaN &         True &  False &           1 &      0.00 \\
  50 &   0.79 &             129.5 &      0.52 &  45.5 &     45.2 &     45.5 &         NaN &        False &  False &           3 &      0.00 \\
  51 &   0.66 &              47.2 &      0.32 &  44.9 &     44.5 &     45.1 &         NaN &        False &  False &           2 &      0.00 \\
  52 &   6.37 &              46.1 &      0.61 &  43.4 &     44.0 &     43.8 &         NaN &        False &  False &           0 &      0.00 \\
  53 &   0.89 &               8.0 &      0.13 &  43.5 &     43.2 &     44.0 &         NaN &        False &  False &           0 &      0.00 \\
  54 &   0.44 &              14.6 &      0.12 &  44.3 &     43.7 &     45.0 &         NaN &        False &  False &           0 &      0.00 \\
  55 &   0.89 &              15.5 &      0.20 &  43.9 &     43.7 &     44.5 &         NaN &         True &  False &           0 &      0.00 \\
  56 &   0.61 &              50.6 &      0.31 &  45.0 &     44.5 &     45.4 &         NaN &         True &  False &           0 &      0.00 \\
  57 &   0.45 &              16.5 &      0.17 &  44.4 &     43.9 &     44.8 &         NaN &        False &  False &           0 &      0.00 \\
  58 &   0.66 &              10.6 &      0.13 &  43.8 &     43.4 &     44.5 &         NaN &        False &  False &           0 &      0.00 \\
  59 &   1.75 &              10.0 &      0.22 &  43.2 &     43.2 &     43.7 &         NaN &        False &  False &           0 &      0.00 \\
  60 &   2.39 &              71.9 &      0.53 &  44.3 &     44.5 &     44.6 &         NaN &         True &  False &           1 &      0.00 \\
  61 &   0.97 &              19.1 &      0.29 &  44.1 &     43.9 &     44.2 &         NaN &        False &  False &           0 &      0.00 \\
  62 &   0.87 &               9.6 &      0.15 &  43.6 &     43.4 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
  63 &   1.84 &              51.6 &      0.40 &  44.2 &     44.3 &     44.7 &         NaN &        False &  False &           0 &      0.00 \\
  64 &   1.21 &               8.6 &      0.16 &  43.3 &     43.2 &     43.9 &         NaN &        False &  False &           0 &      0.00 \\
  65 &   0.60 &              11.8 &      0.17 &  44.0 &     43.6 &     44.5 &         NaN &         True &  False &           0 &      0.00 \\
  66 &   1.10 &              30.5 &      0.34 &  44.3 &     44.1 &     44.6 &         NaN &         True &  False &           0 &      0.00 \\
  67 &   1.99 &              27.9 &      0.36 &  43.8 &     43.9 &     44.1 &         NaN &        False &  False &           1 &      0.00 \\
  68 &   2.08 &              27.3 &      0.35 &  43.7 &     43.9 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
  69 &   1.59 &              19.5 &      0.32 &  43.7 &     43.7 &     44.1 &         NaN &         True &  False &           0 &      0.00 \\
  70 &   1.88 &              27.1 &      0.34 &  43.8 &     43.9 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
  71 &   1.81 &             141.8 &      0.62 &  45.0 &     45.0 &     45.2 &         NaN &         True &  False &           2 &      0.00 \\
  72 &   2.29 &              39.7 &      0.40 &  43.9 &     44.0 &     44.5 &         NaN &        False &  False &           0 &      0.00 \\
  73 &   3.08 &             286.0 &      0.86 &  45.1 &     45.3 &     45.4 &         NaN &         True &  False &           0 &      0.00 \\
  74 &   1.56 &              62.0 &      0.42 &  44.5 &     44.5 &     44.9 &         NaN &         True &  False &           0 &      0.00 \\
  75 &   2.64 &              56.3 &      0.51 &  44.1 &     44.3 &     44.4 &         NaN &         True &  False &           0 &      0.00 \\
  76 &   2.47 &              62.9 &      0.52 &  44.2 &     44.4 &     44.6 &         NaN &         True &  False &           0 &      0.00 \\
  77 &   2.23 &              19.0 &      0.36 &  43.5 &     43.6 &     43.9 &         NaN &        False &  False &           1 &      0.00 \\
  78 &   1.88 &              18.5 &      0.29 &  43.5 &     43.6 &     44.1 &         NaN &         True &  False &           0 &      0.00 \\
  79 &   1.77 &              92.1 &      0.52 &  44.6 &     44.7 &     45.1 &         NaN &         True &  False &           0 &      0.00 \\
  80 &   2.24 &              18.2 &      0.28 &  43.4 &     43.6 &     43.9 &         NaN &         True &  False &           0 &      0.00 \\
  81 &   1.72 &              14.6 &      0.25 &  43.4 &     43.4 &     44.1 &         NaN &        False &  False &           0 &      0.00 \\
  82 &   2.24 &              50.6 &      0.42 &  44.0 &     44.2 &     44.7 &         NaN &        False &  False &           0 &      0.00 \\
  83 &   0.82 &             234.7 &      0.63 &  45.9 &     45.6 &     45.9 &         NaN &         True &  False &           1 &      0.00 \\
  84 &   6.16 &              65.1 &      0.60 &  43.5 &     44.1 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
  85 &   2.50 &              85.1 &      0.59 &  44.4 &     44.6 &     44.7 &         NaN &        False &  False &           1 &      0.00 \\
  86 &   0.89 &             181.7 &      0.71 &  45.8 &     45.5 &     45.2 &         NaN &         True &  False &           2 &      0.00 \\
  87 &   2.71 &              30.6 &      0.39 &  43.7 &     43.9 &     44.0 &         NaN &         True &  False &           0 &      0.00 \\
  88 &   1.67 &              44.3 &      0.41 &  44.2 &     44.3 &     44.5 &         NaN &        False &  False &           1 &      0.00 \\
  89 &   2.83 &              18.7 &      0.36 &  43.3 &     43.6 &     43.8 &         NaN &        False &  False &           0 &      0.00 \\
  90 &   1.25 &              16.3 &      0.22 &  43.7 &     43.6 &     44.4 &         NaN &        False &  False &           0 &      0.00 \\
  91 &   2.72 &              47.1 &      0.45 &  44.0 &     44.2 &     44.3 &        44.9 &         True &  False &           0 &      0.00 \\
  92 &   0.84 &              70.7 &      0.45 &  45.1 &     44.8 &     45.0 &         NaN &        False &  False &           4 &      0.00 \\
  93 &   1.70 &              67.1 &      0.49 &  44.5 &     44.5 &     44.7 &         NaN &         True &  False &           1 &      0.00 \\
  94 &   1.75 &              28.3 &      0.44 &  44.0 &     44.1 &     43.8 &         NaN &        False &  False &           1 &      0.00 \\
  95 &   2.97 &             103.1 &      0.61 &  44.4 &     44.7 &     44.8 &         NaN &         True &  False &           0 &      0.00 \\
  96 &   3.13 &              33.9 &      0.39 &  43.5 &     43.8 &     44.4 &         NaN &        False &  False &           0 &      0.00 \\
  97 &   2.22 &              17.1 &      0.27 &  43.3 &     43.5 &     43.9 &         NaN &        False &  False &           1 &      0.00 \\
  98 &   2.87 &             112.5 &      0.63 &  44.5 &     44.7 &     44.9 &        45.6 &         True &  False &           1 &      0.00 \\
  99 &   0.73 &              46.9 &      0.34 &  44.9 &     44.5 &     44.9 &         NaN &        False &  False &           2 &      0.00 \\
 100 &   2.72 &              25.1 &      0.34 &  43.4 &     43.7 &     44.1 &         NaN &        False &  False &           0 &      0.00 \\
 101 &  19.37 &             158.5 &      1.12 &  43.4 &     44.5 &     44.0 &         NaN &        False &  False &           0 &      0.00 \\
 102 &   1.59 &              18.6 &      0.30 &  43.7 &     43.7 &     44.2 &        44.6 &        False &  False &           0 &      0.00 \\
 103 &   1.42 &             241.2 &      0.73 &  45.5 &     45.5 &     45.6 &        46.4 &        False &  False &           1 &      0.00 \\
 104 &   2.00 &              42.3 &      0.45 &  44.1 &     44.2 &     44.3 &         NaN &         True &  False &           0 &      0.00 \\
 105 &   2.00 &              38.9 &      0.41 &  44.0 &     44.1 &     44.3 &         NaN &         True &  False &           0 &      0.00 \\
 106 &   0.67 &              22.4 &      0.22 &  44.4 &     44.0 &     44.7 &         NaN &         True &  False &           0 &      0.00 \\
 107 &   1.93 &              31.1 &      0.45 &  44.0 &     44.1 &     43.9 &         NaN &         True &  False &           0 &      0.00 \\
 108 &   4.25 &             141.9 &      0.91 &  44.5 &     45.0 &     44.5 &        45.4 &         True &  False &           0 &      0.00 \\
 109 &   1.96 &              32.3 &      0.39 &  43.9 &     44.0 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
 110 &   1.67 &              33.6 &      0.37 &  44.1 &     44.1 &     44.3 &         NaN &         True &  False &           0 &      0.00 \\
 111 &   0.65 &             218.0 &      0.73 &  46.2 &     45.8 &     45.6 &        46.5 &         True &  False &           2 &      0.00 \\
 112 &   2.74 &              31.0 &      0.37 &  43.6 &     43.8 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
 113 &  16.95 &              99.2 &      0.95 &  43.2 &     44.2 &     43.7 &         NaN &        False &  False &           0 &      0.00 \\
 114 &   0.88 &             176.8 &      0.64 &  45.7 &     45.5 &     45.3 &         NaN &        False &  False &           1 &      0.00 \\
 115 &   2.94 &              64.3 &      0.67 &  44.3 &     44.6 &     44.2 &        45.5 &        False &  False &           0 &      0.00 \\
 116 &   2.05 &              27.0 &      0.36 &  43.8 &     43.9 &     44.1 &         NaN &        False &  False &           1 &      0.00 \\
 117 &   1.11 &             114.7 &      0.70 &  45.4 &     45.3 &     44.9 &        45.8 &         True &  False &           0 &      0.00 \\
 118 &   0.67 &             430.5 &      1.24 &  46.9 &     46.5 &     45.4 &        46.4 &         True &  False &           1 &      0.15 \\
 119 &   1.34 &              22.8 &      0.28 &  43.9 &     43.8 &     44.8 &         NaN &        False &  False &           1 &      0.00 \\
 120 &   1.59 &              16.7 &      0.25 &  43.6 &     43.6 &     44.1 &         NaN &        False &  False &           0 &      0.00 \\
 121 &   2.31 &              26.3 &      0.35 &  43.6 &     43.8 &     44.3 &         NaN &        False &  False &           0 &      0.00 \\
 122 &   2.00 &              40.2 &      0.38 &  44.0 &     44.1 &     44.8 &         NaN &        False &  False &           0 &      0.00 \\
 123 &   2.66 &              29.3 &      0.45 &  43.7 &     43.9 &     44.1 &        44.3 &        False &  False &           1 &      0.00 \\
 124 &   1.09 &              27.1 &      0.32 &  44.2 &     44.1 &     44.4 &         NaN &         True &  False &           0 &      0.00 \\
 125 &   1.18 &              16.6 &      0.27 &  43.9 &     43.7 &     44.0 &         NaN &         True &  False &           0 &      0.00 \\
 126 &   0.44 &              78.7 &      0.66 &  46.0 &     45.4 &     44.6 &        45.5 &         True &  False &           1 &      0.00 \\
 127 &   8.51 &             123.2 &      0.83 &  43.8 &     44.5 &     44.2 &         NaN &        False &  False &           1 &      0.00 \\
 128 &   1.03 &              37.1 &      0.28 &  44.4 &     44.2 &     44.7 &         NaN &         True &  False &           0 &      0.00 \\
 129 &   1.10 &              29.1 &      0.30 &  44.2 &     44.1 &     44.8 &        44.9 &        False &  False &           0 &      0.00 \\
 130 &   1.90 &              14.5 &      0.21 &  43.4 &     43.5 &     43.8 &         NaN &         True &  False &           0 &      0.00 \\
 131 &   0.86 &              80.0 &      0.52 &  45.2 &     45.0 &     45.1 &        45.6 &        False &  False &           0 &      0.00 \\
 132 &   0.90 &              39.0 &      0.37 &  44.7 &     44.4 &     44.7 &        45.0 &        False &  False &           1 &      0.00 \\
 133 &   1.40 &              93.7 &      0.57 &  44.9 &     44.9 &     45.1 &        45.8 &         True &  False &           0 &      0.00 \\
 134 &   2.59 &              19.8 &      0.32 &  43.4 &     43.6 &     44.1 &         NaN &         True &  False &           0 &      0.00 \\
 135 &   1.62 &              47.3 &      0.41 &  44.3 &     44.3 &     44.8 &         NaN &         True &  False &           0 &      0.00 \\
 136 &   6.83 &              58.4 &      0.63 &  43.4 &     44.1 &     44.1 &         NaN &        False &  False &           0 &      0.00 \\
 137 &   6.03 &              52.2 &      0.63 &  43.5 &     44.1 &     43.9 &         NaN &         True &  False &           0 &      0.00 \\
 138 &   1.42 &              44.2 &      0.39 &  44.4 &     44.3 &     44.6 &         NaN &         True &  False &           1 &      0.00 \\
 139 &   1.54 &              20.0 &      0.30 &  43.7 &     43.7 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
 140 &   2.32 &              34.8 &      0.36 &  43.8 &     43.9 &     44.4 &         NaN &         True &  False &           0 &      0.00 \\
 141 &   1.46 &              11.0 &      0.23 &  43.4 &     43.3 &     43.9 &         NaN &         True &  False &           0 &      0.00 \\
 142 &   3.28 &              28.0 &      0.45 &  43.5 &     43.8 &     43.9 &         NaN &         True &  False &           0 &      0.00 \\
 143 &   1.03 &              32.5 &      0.31 &  44.3 &     44.1 &     44.9 &         NaN &         True &  False &           0 &      0.00 \\
 144 &   1.92 &              28.5 &      0.41 &  43.9 &     44.0 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
 145 &   2.92 &              15.5 &      0.27 &  43.1 &     43.4 &     43.8 &         NaN &        False &  False &           0 &      0.00 \\
 146 &   1.04 &              19.0 &      0.29 &  44.0 &     43.9 &     44.4 &         NaN &        False &  False &           0 &      0.00 \\
 147 &   3.95 &              63.6 &      0.65 &  44.0 &     44.4 &     44.2 &         NaN &         True &  False &           1 &      0.00 \\
 148 &   4.11 &             103.9 &      0.76 &  44.3 &     44.7 &     44.4 &         NaN &        False &  False &           0 &      0.00 \\
 149 &   0.92 &             426.4 &      0.91 &  46.3 &     46.1 &     45.9 &         NaN &         True &  False &           0 &      0.03 \\
 150 &   4.62 &              38.9 &      0.47 &  43.4 &     43.8 &     44.0 &         NaN &        False &  False &           0 &      0.00 \\
 151 &   0.77 &              28.7 &      0.33 &  44.6 &     44.3 &     44.6 &         NaN &         True &  False &           2 &      0.00 \\
 152 &   0.65 &              18.8 &      0.22 &  44.3 &     43.9 &     44.6 &         NaN &         True &  False &           0 &      0.00 \\
 153 &   0.73 &              43.6 &      0.41 &  44.9 &     44.6 &     44.8 &         NaN &         True &  False &           1 &      0.00 \\
 154 &   1.89 &              35.8 &      0.38 &  44.0 &     44.1 &     44.5 &         NaN &         True &  False &           0 &      0.00 \\
 155 &   1.81 &              29.3 &      0.45 &  44.1 &     44.1 &     44.0 &         NaN &         True &  False &           1 &      0.00 \\
 156 &   0.83 &              30.0 &      0.31 &  44.5 &     44.2 &     44.8 &         NaN &        False &  False &           0 &      0.00 \\
 157 &   2.40 &              29.4 &      0.37 &  43.6 &     43.8 &     44.2 &         NaN &        False &  False &           0 &      0.00 \\
 158 &   1.22 &              19.3 &      0.34 &  44.0 &     43.9 &     44.0 &         NaN &         True &  False &           1 &      0.00 \\
 159 &   0.70 &              53.8 &      0.37 &  45.0 &     44.6 &     45.2 &         NaN &         True &  False &           1 &      0.00 \\
 160 &   1.73 &              24.8 &      0.41 &  44.0 &     44.0 &     43.9 &         NaN &         True &  False &           2 &      0.00 \\
 161 &   1.76 &              22.6 &      0.39 &  43.9 &     43.9 &     43.9 &         NaN &         True &  False &           0 &      0.00 \\
 162 &   0.73 &              26.8 &      0.24 &  44.4 &     44.1 &     44.9 &         NaN &         True &  False &           0 &      0.00 \\
 163 &   0.92 &             144.1 &      0.60 &  45.5 &     45.3 &     45.5 &         NaN &        False &  False &           2 &      0.00 \\
 164 &   0.68 &              29.0 &      0.24 &  44.5 &     44.1 &     44.9 &         NaN &        False &  False &           0 &      0.00 \\
 165 &   0.30 &              50.8 &      0.37 &  45.7 &     45.0 &     45.1 &         NaN &        False &  False &           3 &      0.00 \\
 166 &   1.03 &              25.6 &      0.31 &  44.2 &     44.0 &     44.6 &         NaN &         True &  False &           0 &      0.00 \\
 167 &   0.63 &              58.6 &      0.45 &  45.3 &     44.9 &     44.9 &         NaN &        False &  False &           4 &      0.00 \\
 168 &   1.08 &              24.0 &      0.26 &  44.1 &     43.9 &     44.6 &         NaN &         True &  False &           0 &      0.00 \\
 169 &   1.30 &              23.0 &      0.30 &  43.9 &     43.8 &     44.5 &         NaN &         True &  False &           0 &      0.00 \\
 170 &   1.62 &              18.3 &      0.25 &  43.6 &     43.6 &     44.2 &         NaN &         True &  False &           1 &      0.00 \\
 171 &   6.39 &              50.6 &      0.65 &  43.5 &     44.1 &     43.9 &         NaN &        False &  False &           0 &      0.00 \\
 172 &   0.91 &              36.3 &      0.34 &  44.5 &     44.3 &     44.8 &         NaN &         True &  False &           0 &      0.00 \\
 173 &   1.00 &              23.4 &      0.27 &  44.2 &     43.9 &     44.6 &         NaN &        False &  False &           0 &      0.00 \\
 174 &   6.51 &              39.5 &      0.55 &  43.2 &     43.8 &     43.7 &         NaN &        False &  False &           0 &      0.00 \\
 175 &   1.74 &              23.1 &      0.29 &  43.7 &     43.8 &     44.4 &         NaN &        False &  False &           0 &      0.00 \\
 176 &   2.41 &              22.6 &      0.33 &  43.5 &     43.6 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
 177 &   1.85 &              22.7 &      0.34 &  43.7 &     43.8 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
 178 &   1.91 &              18.0 &      0.26 &  43.4 &     43.5 &     44.3 &         NaN &        False &  False &           0 &      0.00 \\
 179 &   3.78 &              44.4 &      0.48 &  43.6 &     44.0 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
 180 &   0.86 &              43.1 &      0.33 &  44.6 &     44.4 &     45.0 &         NaN &         True &  False &           2 &      0.00 \\
 181 &   1.94 &              54.2 &      0.43 &  44.2 &     44.3 &     44.6 &         NaN &        False &  False &           0 &      0.00 \\
 182 &   1.78 &              20.9 &      0.29 &  43.6 &     43.7 &     44.3 &         NaN &         True &  False &           1 &      0.00 \\
 183 &   1.74 &              21.3 &      0.31 &  43.7 &     43.7 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
 184 &   0.91 &              18.3 &      0.24 &  44.0 &     43.8 &     44.4 &         NaN &         True &  False &           0 &      0.00 \\
 185 &   0.59 &              20.1 &      0.21 &  44.4 &     44.0 &     44.7 &         NaN &         True &  False &           0 &      0.00 \\
 186 &   1.31 &              50.2 &      0.41 &  44.5 &     44.4 &     44.7 &         NaN &        False &  False &           0 &      0.00 \\
 187 &   3.10 &              33.2 &      0.44 &  43.6 &     43.9 &     44.0 &         NaN &        False &  False &           0 &      0.00 \\
 188 &   1.61 &              26.9 &      0.34 &  43.9 &     43.9 &     44.3 &         NaN &        False &  False &           0 &      0.00 \\
 189 &   2.54 &              61.8 &      0.54 &  44.2 &     44.4 &     44.4 &         NaN &        False &  False &           0 &      0.00 \\
 190 &   1.62 &              39.9 &      0.38 &  44.2 &     44.2 &     44.5 &         NaN &        False &  False &           0 &      0.00 \\
 191 &   1.51 &              10.9 &      0.18 &  43.3 &     43.3 &     43.8 &         NaN &        False &  False &           0 &      0.00 \\
 192 &   0.74 &             131.2 &      0.50 &  45.6 &     45.2 &     45.4 &         NaN &        False &  False &           4 &      0.00 \\
 193 &  10.48 &             124.7 &      0.91 &  43.7 &     44.5 &     44.0 &         NaN &        False &  False &           0 &      0.00 \\
 194 &    NaN &              47.6 &      0.32 &   NaN &      NaN &      NaN &         NaN &        False &  False &           1 &      0.00 \\
 195 &    NaN &              81.7 &      0.72 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &      0.00 \\
 196 &    NaN &              42.8 &      0.47 &   NaN &      NaN &      NaN &         NaN &        False &  False &           1 &      0.00 \\
 197 &    NaN &              99.8 &      0.88 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &      0.00 \\
 198 &    NaN &              56.8 &      0.34 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &      0.00 \\
 199 &    NaN &              35.9 &      0.47 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &      0.00 \\
\bottomrule
\end{tabular}


==> CygX_S_leaf_stats.tex <==
\begin{tabular}{rrrrrrlrrllrrr}
\toprule
ID & RA & decl. & PA & $\sigma_{major}$ & $\sigma_{minor}$ &  $R_{eff}$ &  $M_{obs}$ &  $M_{clip}$ &  $T_K$ &  $\sigma_{NH_3}$ &  $V_{LSR, NH_3}$ &  log($N_{para-NH_3}$) &  log($N_{H_2}$) \\& (deg) & (deg) & (deg) & ($\arcsec$) & ($\arcsec$) & (pc) & (M$_\odot$) & (M$_\odot$) & (K) & (km s$^{-1}$) & (km s$^{-1}$) & (cm$^{-2}$) & (cm$^{-2}$) \\\midrule
   0 &  308.3976 &  38.5130 &   92 &         12.9 &          9.9 &   0.16 $^{+0.06}_{-0.03}$ &    9.6 &           0.6 &  12.4 $\pm$ 2.9 &  0.34 $\pm$ 0.05 &          -2.6 &            14.0 &             21.7 \\
   1 &  308.3713 &  38.5369 &  221 &         21.3 &         13.9 &    0.26 $^{+0.2}_{-0.08}$ &   26.9 &           3.8 &  11.9 $\pm$ 1.8 &  0.28 $\pm$ 0.03 &          -2.9 &            13.9 &             21.7 \\
   2 &  308.4271 &  38.5588 &  142 &         14.7 &         11.9 &   0.19 $^{+0.03}_{-0.02}$ &   18.2 &           5.8 &  12.8 $\pm$ 2.3 &  0.19 $\pm$ 0.03 &          -1.7 &            13.7 &             21.7 \\
   3 &  308.3334 &  38.5773 &  173 &         35.5 &         18.6 &   0.42 $^{+0.32}_{-0.15}$ &   95.4 &          34.9 &  14.9 $\pm$ 1.3 &   0.4 $\pm$ 0.03 &          -0.9 &            14.1 &             21.7 \\
   4 &  308.2804 &  38.5865 &  118 &         19.7 &         15.9 &    0.22 $^{+0.1}_{-0.09}$ &   23.5 &           6.5 &  14.4 $\pm$ 2.8 &  0.39 $\pm$ 0.06 &          -1.1 &            13.7 &             21.7 \\
   5 &  308.4036 &  38.5938 &  119 &         23.0 &         14.3 &   0.21 $^{+0.14}_{-0.16}$ &   21.0 &           4.2 &  12.4 $\pm$ 3.0 &  0.54 $\pm$ 0.08 &           1.8 &            13.4 &             21.8 \\
   6 &  308.3819 &  38.6140 &  112 &         23.0 &         20.8 &    0.28 $^{+0.13}_{-0.2}$ &   48.9 &           8.8 &  14.1 $\pm$ 4.1 &  1.07 $\pm$ 0.19 &           0.5 &            14.2 &             21.8 \\
   7 &  308.4574 &  38.6348 &  172 &         22.4 &         14.5 &   0.24 $^{+0.09}_{-0.13}$ &   48.1 &           6.4 &  15.6 $\pm$ 3.7 &  0.46 $\pm$ 0.09 &           0.9 &            13.5 &             21.8 \\
   8 &  308.4640 &  38.6538 &  153 &         26.4 &         15.5 &   0.23 $^{+0.21}_{-0.16}$ &   32.2 &           7.9 &  13.2 $\pm$ 3.8 &   0.55 $\pm$ 0.1 &           1.4 &            13.9 &             21.7 \\
   9 &  308.2060 &  38.6649 &   81 &         19.5 &          8.0 &   0.17 $^{+0.13}_{-0.07}$ &   11.9 &           1.1 &  16.1 $\pm$ 3.3 &  0.17 $\pm$ 0.04 &          -0.7 &            13.7 &             21.7 \\
  10 &  308.3408 &  38.6987 &  125 &         27.2 &         15.6 &     0.29 $^{+0.2}_{-0.1}$ &   46.4 &          10.9 &  14.9 $\pm$ 2.1 &   0.4 $\pm$ 0.05 &          -1.7 &            13.8 &             21.7 \\
  11 &  308.8029 &  38.6970 &  207 &         22.1 &         12.8 &   0.23 $^{+0.09}_{-0.04}$ &   39.6 &           9.4 &  14.6 $\pm$ 1.9 &  0.58 $\pm$ 0.06 &          -2.7 &            14.2 &             21.7 \\
  12 &  308.7735 &  38.7086 &  163 &         18.9 &         11.1 &   0.22 $^{+0.09}_{-0.06}$ &   40.0 &          10.8 &  15.0 $\pm$ 1.2 &  0.46 $\pm$ 0.03 &          -3.4 &            14.2 &             21.7 \\
  13 &  308.1824 &  38.7321 &  138 &         31.9 &         27.5 &    0.45 $^{+0.15}_{-0.1}$ &  190.7 &          93.9 &  13.9 $\pm$ 0.8 &  0.43 $\pm$ 0.02 &          -0.0 &            14.3 &             21.7 \\
  14 &  308.1681 &  38.7713 &  115 &         30.6 &         22.2 &   0.45 $^{+0.21}_{-0.08}$ &  274.8 &         168.1 &  16.3 $\pm$ 0.6 &  0.58 $\pm$ 0.02 &          -0.7 &            14.4 &             21.7 \\
  15 &  308.2061 &  38.7609 &   93 &         12.7 &         10.2 &   0.17 $^{+0.02}_{-0.01}$ &   16.7 &           5.4 &  15.6 $\pm$ 1.5 &  0.28 $\pm$ 0.03 &           0.2 &            14.1 &             21.7 \\
  16 &  308.1507 &  38.8163 &  121 &         30.8 &         13.9 &   0.31 $^{+0.32}_{-0.12}$ &   49.9 &          15.0 &  15.6 $\pm$ 1.8 &  0.36 $\pm$ 0.04 &           1.0 &            14.1 &             21.7 \\
  17 &  307.6774 &  38.8283 &  118 &         29.4 &         10.3 &   0.23 $^{+0.26}_{-0.12}$ &   21.5 &           4.3 &  12.6 $\pm$ 3.1 &   0.4 $\pm$ 0.06 &          -4.1 &            14.0 &             21.6 \\
  18 &  307.9428 &  38.9525 &   55 &         46.3 &         14.3 &     0.3 $^{+0.31}_{-0.2}$ &   58.3 &          21.3 &  22.4 $\pm$ 3.6 &  0.54 $\pm$ 0.08 &           0.5 &            13.6 &             21.7 \\
  19 &  307.8325 &  38.9579 &  224 &         19.9 &         13.4 &   0.25 $^{+0.11}_{-0.05}$ &   73.0 &          32.3 &  21.6 $\pm$ 1.3 &  0.74 $\pm$ 0.04 &          -0.5 &            14.1 &             21.7 \\
  20 &  308.1021 &  38.9645 &   66 &         11.8 &         10.5 &   0.14 $^{+0.04}_{-0.02}$ &    8.2 &           1.1 &  14.3 $\pm$ 4.5 &  0.53 $\pm$ 0.13 &           0.8 &            13.9 &             21.6 \\
  21 &  307.9971 &  38.9762 &  132 &         19.3 &         11.2 &    0.2 $^{+0.15}_{-0.08}$ &   28.1 &          10.3 &  30.7 $\pm$ 3.2 &  0.69 $\pm$ 0.07 &          -4.5 &            13.5 &             21.7 \\
  22 &  307.8106 &  38.9757 &  170 &         22.0 &         13.8 &   0.22 $^{+0.12}_{-0.09}$ &   44.4 &           9.7 &  22.6 $\pm$ 2.2 &  0.76 $\pm$ 0.07 &          -0.0 &            13.6 &             21.7 \\
  23 &  307.4157 &  38.9689 &  208 &         10.7 &          7.8 &   0.13 $^{+0.03}_{-0.01}$ &    7.3 &           0.6 &  16.9 $\pm$ 3.2 &  0.26 $\pm$ 0.05 &          -3.2 &            13.8 &             21.6 \\
  24 &  308.0311 &  38.9812 &   51 &         15.3 &          9.4 &   0.15 $^{+0.08}_{-0.09}$ &    7.8 &           0.5 &  12.4 $\pm$ 4.6 &  0.71 $\pm$ 0.16 &           0.1 &            14.1 &             21.6 \\
  25 &  307.7785 &  38.9787 &  179 &         16.3 &         11.6 &   0.19 $^{+0.07}_{-0.04}$ &   25.4 &           5.8 &  20.0 $\pm$ 2.0 &   0.6 $\pm$ 0.05 &          -0.3 &            13.7 &             21.7 \\
  26 &  307.3896 &  38.9809 &  196 &         24.3 &         16.3 &    0.3 $^{+0.18}_{-0.05}$ &   47.2 &          14.7 &  19.1 $\pm$ 2.4 &  0.46 $\pm$ 0.05 &          -3.4 &            13.9 &             21.6 \\
  27 &  307.8590 &  38.9836 &  176 &         23.3 &         14.5 &   0.23 $^{+0.12}_{-0.07}$ &   32.4 &           7.4 &  20.6 $\pm$ 3.3 &  1.04 $\pm$ 0.14 &          -0.5 &            13.9 &             21.7 \\
  28 &  307.8921 &  38.9950 &  194 &         30.6 &         22.0 &   0.25 $^{+0.25}_{-0.19}$ &   33.1 &           9.1 &  17.0 $\pm$ 3.3 &   0.7 $\pm$ 0.11 &          -0.5 &            14.0 &             21.7 \\
  29 &  307.9459 &  39.0174 &  104 &         15.6 &          7.0 &   0.14 $^{+0.05}_{-0.07}$ &   12.2 &           2.8 &  21.6 $\pm$ 3.6 &  0.56 $\pm$ 0.09 &           0.2 &            13.9 &             21.7 \\
  30 &  307.3779 &  39.0166 &   92 &         16.2 &          9.5 &   0.17 $^{+0.08}_{-0.09}$ &   11.6 &           3.1 &  24.8 $\pm$ 4.4 &  0.59 $\pm$ 0.09 &          -3.7 &            14.0 &             21.6 \\
  31 &  307.8351 &  39.0319 &  185 &         27.4 &          9.6 &    0.2 $^{+0.17}_{-0.08}$ &   19.7 &           4.7 &  14.3 $\pm$ 3.3 &  0.27 $\pm$ 0.06 &          -0.1 &            13.9 &             21.7 \\
  32 &  307.9625 &  39.0403 &  170 &         12.0 &         10.2 &    0.16 $^{+0.0}_{-0.02}$ &   13.6 &           3.5 &  23.7 $\pm$ 3.3 &  0.39 $\pm$ 0.06 &          -1.7 &            13.3 &             21.7 \\
  33 &  307.8092 &  39.1478 &  184 &          9.9 &          8.1 &   0.12 $^{+0.01}_{-0.03}$ &    5.9 &           0.9 &  17.5 $\pm$ 3.9 &  0.21 $\pm$ 0.04 &           1.5 &            13.3 &             21.6 \\
  34 &  308.2332 &  39.4054 &  168 &         10.8 &          9.3 &   0.14 $^{+0.01}_{-0.02}$ &    8.7 &           0.6 &  14.0 $\pm$ 4.0 &  0.39 $\pm$ 0.09 &          -3.8 &            13.8 &             21.7 \\
  35 &  308.5313 &  39.4177 &   49 &         14.1 &         11.5 &   0.18 $^{+0.04}_{-0.01}$ &   19.5 &           4.1 &  19.7 $\pm$ 3.1 &   0.6 $\pm$ 0.08 &          -2.1 &            13.6 &             21.7 \\
  36 &  308.5291 &  39.4770 &   73 &         19.8 &          8.1 &   0.15 $^{+0.08}_{-0.09}$ &    9.6 &           1.6 &  17.6 $\pm$ 4.2 &  0.37 $\pm$ 0.08 &          -0.9 &            13.7 &             21.7 \\
  37 &  308.2222 &  39.4983 &   48 &         10.3 &          9.0 &   0.12 $^{+0.04}_{-0.02}$ &    7.6 &           0.9 &  14.9 $\pm$ 3.8 &  0.21 $\pm$ 0.05 &          -3.4 &            13.7 &             21.7 \\
  38 &  308.5202 &  39.5116 &   76 &         16.5 &         11.4 &     0.2 $^{+0.1}_{-0.05}$ &   22.1 &           6.5 &  14.6 $\pm$ 2.5 &  0.48 $\pm$ 0.07 &           0.5 &            14.0 &             21.7 \\
  39 &  308.4727 &  39.5170 &   52 &         28.5 &         14.6 &   0.33 $^{+0.24}_{-0.09}$ &   70.1 &          28.9 &  14.9 $\pm$ 1.4 &  0.29 $\pm$ 0.03 &          -1.4 &            14.0 &             21.7 \\
  40 &  308.6433 &  39.5787 &  211 &         18.2 &         15.9 &   0.25 $^{+0.11}_{-0.02}$ &   26.3 &           5.1 &  14.1 $\pm$ 2.7 &  0.33 $\pm$ 0.05 &           4.5 &            13.4 &             21.6 \\
  41 &  308.8231 &  39.6453 &  177 &         10.8 &          9.1 &   0.13 $^{+0.01}_{-0.02}$ &    8.4 &           0.9 &  18.7 $\pm$ 3.7 &  0.68 $\pm$ 0.12 &           7.8 &            14.0 &             21.6 \\
  42 &  309.0952 &  39.6732 &  130 &         30.5 &         13.5 &   0.29 $^{+0.19}_{-0.11}$ &   44.6 &           9.5 &  12.0 $\pm$ 2.4 &  0.31 $\pm$ 0.04 &           4.6 &            13.9 &             21.7 \\
  43 &  308.6195 &  39.6769 &  177 &         23.6 &         14.1 &     0.25 $^{+0.1}_{-0.1}$ &   32.0 &           5.6 &  14.0 $\pm$ 3.0 &  0.26 $\pm$ 0.05 &           4.8 &            13.5 &             21.7 \\
  44 &  308.3668 &  39.6871 &   76 &         18.0 &         15.2 &    0.29 $^{+0.1}_{-0.05}$ &   86.3 &          32.6 &  14.4 $\pm$ 0.9 &   0.3 $\pm$ 0.02 &           0.8 &            14.3 &             21.8 \\
  45 &  308.6309 &  39.6908 &  163 &         13.1 &          7.7 &   0.12 $^{+0.03}_{-0.07}$ &    6.9 &           0.6 &  13.3 $\pm$ 3.9 &   0.2 $\pm$ 0.05 &           4.3 &            13.8 &             21.7 \\
  46 &  309.1187 &  39.7126 &   72 &         34.3 &         15.8 &   0.38 $^{+0.17}_{-0.14}$ &  115.1 &          54.2 &  13.1 $\pm$ 1.3 &  0.38 $\pm$ 0.03 &           3.9 &            14.1 &             21.7 \\
  47 &  308.3459 &  39.7129 &  208 &         20.1 &         14.5 &    0.3 $^{+0.11}_{-0.06}$ &   85.9 &          33.3 &  15.9 $\pm$ 1.1 &  0.39 $\pm$ 0.03 &           1.3 &            14.2 &             21.8 \\
  48 &  308.6142 &  39.7167 &   75 &         20.5 &         10.2 &    0.2 $^{+0.08}_{-0.09}$ &   19.3 &           2.1 &  11.9 $\pm$ 2.8 &  0.16 $\pm$ 0.03 &           5.0 &            13.7 &             21.8 \\
  49 &  308.6775 &  39.7493 &  182 &         22.8 &         20.4 &   0.42 $^{+0.24}_{-0.09}$ &  206.8 &         126.5 &  18.4 $\pm$ 0.6 &  0.74 $\pm$ 0.02 &           6.0 &            14.5 &             21.8 \\
  50 &  308.9449 &  39.8238 &  211 &         26.8 &         11.3 &   0.21 $^{+0.22}_{-0.09}$ &   26.7 &           6.9 &  11.5 $\pm$ 4.1 &  0.31 $\pm$ 0.07 &           1.1 &            13.5 &             21.7 \\
  51 &  309.3104 &  39.8201 &   80 &         14.7 &         13.2 &   0.24 $^{+0.01}_{-0.02}$ &   39.7 &          15.9 &  22.0 $\pm$ 1.5 &  0.45 $\pm$ 0.03 &           6.9 &            14.4 &             21.7 \\
  52 &  308.9603 &  39.8463 &   70 &         30.8 &         18.5 &    0.35 $^{+0.33}_{-0.1}$ &   70.1 &          25.8 &  11.4 $\pm$ 2.0 &  0.27 $\pm$ 0.03 &           1.6 &            14.0 &             21.7 \\
  53 &  309.4505 &  39.8286 &  210 &         19.0 &         11.4 &     0.2 $^{+0.1}_{-0.05}$ &   58.8 &          20.1 &  16.2 $\pm$ 0.4 &   0.4 $\pm$ 0.01 &           5.5 &            14.4 &             21.7 \\
  54 &  309.0248 &  39.8299 &  190 &         20.7 &          9.7 &   0.21 $^{+0.11}_{-0.07}$ &   27.8 &           4.6 &  12.6 $\pm$ 2.2 &  0.37 $\pm$ 0.05 &           5.3 &            14.0 &             21.7 \\
  55 &  309.2540 &  39.8435 &   68 &         36.0 &         12.5 &   0.25 $^{+0.24}_{-0.18}$ &   37.5 &           9.5 &  13.3 $\pm$ 2.4 &  0.38 $\pm$ 0.06 &           3.5 &            13.7 &             21.7 \\
  56 &  309.2754 &  39.8414 &  202 &         16.8 &          7.1 &   0.14 $^{+0.07}_{-0.07}$ &   11.2 &           0.7 &  17.6 $\pm$ 3.5 &   0.52 $\pm$ 0.1 &           3.9 &            13.7 &             21.7 \\
  57 &  309.4273 &  39.8480 &   51 &         16.3 &         11.2 &    0.2 $^{+0.05}_{-0.01}$ &   60.8 &          25.0 &  18.2 $\pm$ 0.4 &  0.43 $\pm$ 0.01 &           6.0 &            14.6 &             21.7 \\
  58 &  309.3497 &  39.8475 &  181 &         14.9 &         10.9 &   0.17 $^{+0.03}_{-0.05}$ &   13.8 &           2.0 &  14.0 $\pm$ 3.1 &  0.31 $\pm$ 0.06 &           3.5 &            13.9 &             21.7 \\
  59 &  309.0827 &  39.8493 &  160 &         15.9 &          9.2 &   0.16 $^{+0.05}_{-0.05}$ &   12.4 &           2.1 &  12.4 $\pm$ 3.8 &  0.43 $\pm$ 0.09 &           5.1 &            13.6 &             21.7 \\
  60 &  308.3482 &  39.8515 &  118 &         13.2 &          7.3 &   0.13 $^{+0.04}_{-0.02}$ &    7.1 &           0.7 &  10.1 $\pm$ 4.1 &  0.23 $\pm$ 0.06 &           1.2 &            14.1 &             21.7 \\
  61 &  309.2759 &  39.8671 &   76 &         27.1 &         17.0 &   0.32 $^{+0.18}_{-0.09}$ &   76.4 &          19.9 &  13.1 $\pm$ 1.9 &  0.58 $\pm$ 0.05 &           3.6 &            13.8 &             21.7 \\
  62 &  309.2229 &  39.8600 &   77 &         15.2 &          6.1 &   0.12 $^{+0.09}_{-0.05}$ &    8.4 &           0.7 &  14.2 $\pm$ 4.0 &  0.78 $\pm$ 0.13 &           3.3 &            14.0 &             21.7 \\
  63 &  309.2473 &  39.8717 &  190 &         12.1 &          6.0 &   0.12 $^{+0.05}_{-0.03}$ &    8.1 &           0.2 &  13.0 $\pm$ 3.4 &  1.08 $\pm$ 0.16 &           3.3 &            14.4 &             21.7 \\
  64 &  308.8255 &  39.8894 &  212 &         23.7 &         11.9 &   0.24 $^{+0.09}_{-0.07}$ &   37.4 &          12.0 &  20.6 $\pm$ 3.0 &  0.53 $\pm$ 0.07 &          -2.5 &            13.7 &             21.7 \\
  65 &  308.4474 &  39.8883 &   84 &         16.4 &         11.6 &   0.18 $^{+0.03}_{-0.14}$ &   13.8 &           1.7 &  13.1 $\pm$ 3.5 &  0.15 $\pm$ 0.03 &           1.3 &            13.4 &             21.8 \\
  66 &  309.3154 &  39.8853 &  201 &         10.8 &          7.0 &    0.13 $^{+0.01}_{-0.0}$ &    9.7 &           0.9 &  13.8 $\pm$ 2.9 &  0.31 $\pm$ 0.05 &           3.1 &            13.9 &             21.8 \\
  67 &  308.4240 &  39.9146 &   61 &         26.0 &         13.3 &   0.26 $^{+0.12}_{-0.08}$ &   31.5 &           3.6 &  11.5 $\pm$ 2.3 &  0.29 $\pm$ 0.04 &           1.5 &            13.7 &             21.7 \\
  68 &  309.4527 &  39.9074 &  105 &          9.5 &          6.6 &  0.11 $^{+0.01}_{--0.01}$ &    6.3 &           0.4 &  11.6 $\pm$ 3.4 &  0.22 $\pm$ 0.05 &           3.2 &            13.9 &             21.7 \\
  69 &  308.4860 &  39.9206 &   46 &         14.3 &          9.0 &   0.14 $^{+0.07}_{-0.07}$ &    9.5 &           0.4 &  11.8 $\pm$ 3.1 &  0.17 $\pm$ 0.03 &           1.3 &            13.7 &             21.8 \\
  70 &  308.4638 &  39.9269 &  224 &         14.9 &          9.4 &   0.16 $^{+0.02}_{-0.01}$ &   11.7 &           1.1 &  13.7 $\pm$ 3.9 &  0.49 $\pm$ 0.12 &           0.9 &            14.1 &             21.8 \\
  71 &  308.4103 &  39.9386 &  217 &         17.8 &          6.4 &    0.14 $^{+0.1}_{-0.03}$ &    8.5 &           0.5 &  11.5 $\pm$ 2.5 &  0.21 $\pm$ 0.03 &           1.1 &            13.7 &             21.7 \\
  72 &  308.3569 &  39.9418 &  109 &         15.0 &         10.8 &   0.19 $^{+0.04}_{-0.04}$ &   16.7 &           5.2 &  15.2 $\pm$ 2.0 &  0.29 $\pm$ 0.04 &           8.5 &            14.2 &             21.7 \\
  73 &  308.5785 &  39.9475 &  164 &         15.5 &         10.9 &   0.19 $^{+0.06}_{-0.02}$ &   18.9 &           1.9 &  11.3 $\pm$ 2.7 &  0.18 $\pm$ 0.03 &           0.8 &            13.8 &             21.8 \\
  74 &  309.0812 &  39.9570 &  122 &         13.3 &         12.7 &   0.18 $^{+0.07}_{-0.01}$ &   24.1 &           7.1 &  16.0 $\pm$ 2.8 &  0.45 $\pm$ 0.07 &           4.8 &            13.9 &             21.7 \\
  75 &  308.7757 &  39.9644 &   59 &         19.7 &         14.7 &   0.24 $^{+0.04}_{-0.08}$ &   42.7 &           9.9 &  13.4 $\pm$ 2.9 &  0.41 $\pm$ 0.06 &          -1.4 &            13.9 &             21.8 \\
  76 &  308.1250 &  39.9614 &  107 &         14.1 &          7.9 &   0.14 $^{+0.05}_{-0.06}$ &   12.6 &           4.1 &  24.3 $\pm$ 4.5 &  0.39 $\pm$ 0.07 &           2.7 &            13.9 &             21.7 \\
  77 &  308.5829 &  39.9839 &   84 &         31.7 &         16.6 &   0.34 $^{+0.29}_{-0.14}$ &   84.4 &          26.8 &  10.8 $\pm$ 2.3 &  0.25 $\pm$ 0.03 &           0.8 &            14.2 &             21.8 \\
  78 &  308.5224 &  39.9643 &  167 &         11.6 &          6.1 &   0.12 $^{+0.01}_{-0.03}$ &    8.4 &           0.6 &  11.2 $\pm$ 3.6 &  0.18 $\pm$ 0.04 &          -2.5 &            14.1 &             21.8 \\
  79 &  308.3540 &  39.9749 &   81 &         11.9 &         11.0 &   0.16 $^{+0.04}_{-0.04}$ &    8.8 &           1.0 &  11.1 $\pm$ 3.3 &  0.15 $\pm$ 0.03 &           1.4 &            13.9 &             21.6 \\
  80 &  308.5208 &  39.9793 &  205 &         12.5 &          8.1 &   0.15 $^{+0.04}_{-0.03}$ &   12.8 &           1.1 &  11.9 $\pm$ 3.3 &   0.1 $\pm$ 0.02 &           0.9 &            13.6 &             21.8 \\
  81 &  308.0914 &  40.0096 &   48 &         11.2 &          9.3 &   0.15 $^{+0.02}_{-0.02}$ &   12.7 &           3.3 &  18.9 $\pm$ 3.4 &  0.42 $\pm$ 0.07 &           2.6 &            13.9 &             21.7 \\
  82 &  308.0706 &  40.0424 &  212 &         17.3 &          8.9 &    0.13 $^{+0.1}_{-0.07}$ &    7.7 &           1.0 &  14.9 $\pm$ 4.2 &  0.25 $\pm$ 0.07 &           7.8 &            13.9 &             21.7 \\
  83 &  307.8022 &  40.0564 &  208 &         44.7 &         26.4 &   0.62 $^{+0.53}_{-0.33}$ &  426.1 &         247.8 &  18.3 $\pm$ 0.7 &  0.63 $\pm$ 0.02 &           5.9 &            14.4 &             21.8 \\
  84 &  307.9396 &  40.0687 &   67 &         15.0 &          5.4 &   0.12 $^{+0.07}_{-0.04}$ &    6.8 &           1.0 &  15.5 $\pm$ 4.4 &  0.35 $\pm$ 0.08 &           9.3 &            13.9 &             21.8 \\
  85 &  308.0682 &  40.1153 &  158 &          8.7 &          7.3 &    0.12 $^{+0.01}_{-0.0}$ &    6.1 &           0.8 &  14.7 $\pm$ 2.7 &   0.2 $\pm$ 0.04 &           3.8 &            14.0 &             21.6 \\
  86 &  307.9533 &  40.1201 &  101 &         12.9 &          8.8 &   0.14 $^{+0.07}_{-0.03}$ &    6.9 &           0.4 &  11.9 $\pm$ 3.7 &  0.12 $\pm$ 0.03 &           3.7 &            13.7 &             21.7 \\
  87 &  308.2001 &  40.1487 &  216 &         10.2 &          7.0 &   0.11 $^{+0.04}_{-0.02}$ &    4.1 &           0.4 &  11.2 $\pm$ 3.2 &  0.32 $\pm$ 0.07 &           2.3 &            14.4 &             21.6 \\
  88 &  307.5984 &  40.1557 &   96 &         21.8 &         16.9 &   0.31 $^{+0.09}_{-0.08}$ &    NaN &           NaN &  14.0 $\pm$ 1.4 &  0.44 $\pm$ 0.03 &           6.5 &            14.3 &              NaN \\
  89 &  307.8877 &  40.1635 &   95 &         18.4 &          9.7 &   0.18 $^{+0.08}_{-0.07}$ &   16.3 &           1.3 &  12.0 $\pm$ 3.8 &  0.12 $\pm$ 0.03 &           3.8 &            13.8 &             21.8 \\
  90 &  308.2034 &  40.1811 &   88 &         13.5 &         11.4 &   0.18 $^{+0.02}_{-0.06}$ &    8.9 &           1.6 &  10.7 $\pm$ 2.0 &  0.13 $\pm$ 0.02 &           2.6 &            14.2 &             21.5 \\
  91 &  307.5358 &  40.1923 &  200 &         12.0 &          7.2 &   0.13 $^{+0.04}_{-0.01}$ &    NaN &           NaN &  16.9 $\pm$ 2.9 &   0.3 $\pm$ 0.05 &           6.1 &            13.7 &              NaN \\
  92 &  307.5210 &  40.2020 &  172 &         19.2 &         10.4 &   0.17 $^{+0.12}_{-0.08}$ &    NaN &           NaN &  13.9 $\pm$ 3.7 &  0.37 $\pm$ 0.07 &           6.7 &            13.9 &              NaN \\
  93 &  308.1366 &  40.2115 &  111 &         18.2 &         14.1 &    0.24 $^{+0.1}_{-0.04}$ &   27.4 &           8.7 &  20.3 $\pm$ 2.1 &  0.48 $\pm$ 0.05 &           3.7 &            13.6 &             21.6 \\
  94 &  307.7446 &  40.2195 &  163 &         14.3 &          9.4 &   0.15 $^{+0.02}_{-0.04}$ &   15.8 &           2.4 &  13.1 $\pm$ 3.2 &  0.41 $\pm$ 0.09 &          -2.4 &            14.3 &             21.7 \\
  95 &  307.5560 &  40.2270 &  198 &         19.0 &         13.4 &   0.18 $^{+0.09}_{-0.09}$ &    NaN &           NaN &  14.8 $\pm$ 3.9 &  0.26 $\pm$ 0.07 &           7.4 &            13.5 &              NaN \\
  96 &  307.9002 &  40.2307 &  134 &         10.3 &          7.5 &   0.12 $^{+0.02}_{-0.03}$ &    7.5 &           0.7 &  12.8 $\pm$ 3.7 &  0.14 $\pm$ 0.03 &           4.3 &            13.9 &             21.8 \\
  97 &  308.1251 &  40.2331 &  223 &         13.3 &          8.2 &   0.14 $^{+0.04}_{-0.02}$ &    8.5 &           1.5 &  23.3 $\pm$ 3.8 &  0.25 $\pm$ 0.04 &           3.7 &            14.0 &             21.6 \\
  98 &  307.5347 &  40.2362 &  175 &         12.9 &          7.8 &   0.11 $^{+0.06}_{-0.08}$ &    NaN &           NaN &  14.2 $\pm$ 3.8 &   0.2 $\pm$ 0.04 &           7.2 &            14.0 &              NaN \\
  99 &  308.0158 &  40.2425 &  223 &         16.7 &          7.1 &   0.14 $^{+0.05}_{-0.05}$ &    7.0 &           0.6 &  13.0 $\pm$ 4.2 &  0.17 $\pm$ 0.04 &           3.1 &            13.4 &             21.7 \\
 100 &  307.6482 &  40.2461 &  209 &         15.4 &          8.0 &   0.15 $^{+0.04}_{-0.05}$ &    NaN &           NaN &  15.0 $\pm$ 3.0 &   0.3 $\pm$ 0.05 &           4.3 &            14.0 &              NaN \\
 101 &  308.1636 &  40.2636 &   57 &         21.2 &          6.4 &   0.15 $^{+0.11}_{-0.06}$ &    7.2 &           1.6 &  22.7 $\pm$ 3.8 &  0.32 $\pm$ 0.06 &           5.7 &            13.9 &             21.6 \\
 102 &  307.4890 &  40.2609 &  148 &         24.5 &         13.0 &   0.27 $^{+0.12}_{-0.07}$ &    NaN &           NaN &  17.8 $\pm$ 0.8 &  0.77 $\pm$ 0.03 &           5.9 &            14.4 &              NaN \\
 103 &  307.3847 &  40.2731 &   99 &         14.2 &          5.3 &   0.11 $^{+0.08}_{-0.02}$ &    NaN &           NaN &  11.9 $\pm$ 4.1 &   0.1 $\pm$ 0.02 &           0.2 &            13.5 &              NaN \\
 104 &  307.5201 &  40.2763 &  172 &         18.1 &         10.7 &   0.19 $^{+0.06}_{-0.02}$ &    NaN &           NaN &  16.6 $\pm$ 1.1 &  0.43 $\pm$ 0.03 &           6.9 &            14.2 &              NaN \\
 105 &  307.9065 &  40.2864 &  104 &         10.1 &          8.3 &    0.13 $^{+0.0}_{--0.0}$ &   11.0 &           0.9 &  12.8 $\pm$ 3.1 &  0.19 $\pm$ 0.04 &           2.0 &            14.0 &             21.9 \\
 106 &  307.9416 &  40.3144 &  153 &         36.6 &         24.5 &    0.4 $^{+0.24}_{-0.13}$ &  234.1 &          69.5 &  12.1 $\pm$ 0.7 &  0.34 $\pm$ 0.01 &           1.7 &            14.4 &             21.9 \\
 107 &  308.1886 &  40.3031 &  188 &         12.7 &          8.8 &   0.13 $^{+0.04}_{-0.09}$ &    5.2 &           0.5 &  13.2 $\pm$ 4.4 &  0.37 $\pm$ 0.09 &           0.0 &            13.8 &             21.7 \\
 108 &  307.9910 &  40.3081 &  160 &         20.5 &         15.1 &   0.27 $^{+0.09}_{-0.03}$ &  115.3 &          54.2 &  12.1 $\pm$ 0.5 &  0.65 $\pm$ 0.02 &           1.5 &            14.7 &             21.8 \\
 109 &  308.0390 &  40.3153 &  149 &         31.3 &          8.9 &     0.23 $^{+0.2}_{-0.1}$ &   25.9 &           5.5 &  12.1 $\pm$ 1.0 &  0.36 $\pm$ 0.02 &           0.4 &            14.1 &             21.8 \\
 110 &  308.0939 &  40.3358 &   67 &         43.9 &         26.7 &   0.51 $^{+0.17}_{-0.18}$ &  376.5 &         235.9 &  15.0 $\pm$ 0.7 &  0.56 $\pm$ 0.02 &           0.9 &            14.2 &             21.8 \\
 111 &  308.2267 &  40.3250 &  112 &         14.4 &          7.4 &   0.13 $^{+0.05}_{-0.04}$ &    5.5 &           0.5 &  12.5 $\pm$ 3.7 &  0.14 $\pm$ 0.03 &           0.5 &            13.8 &             21.6 \\
 112 &  307.6781 &  40.3230 &  132 &         22.7 &         13.4 &   0.24 $^{+0.25}_{-0.08}$ &    NaN &           NaN &  15.0 $\pm$ 2.2 &  0.47 $\pm$ 0.05 &          -0.4 &            14.0 &              NaN \\
 113 &  307.5925 &  40.3194 &  151 &         11.8 &          8.3 &    0.14 $^{+0.02}_{-0.0}$ &    NaN &           NaN &  13.8 $\pm$ 2.9 &  0.19 $\pm$ 0.04 &          -0.2 &            13.7 &              NaN \\
 114 &  308.1744 &  40.3258 &  217 &         12.7 &          9.5 &   0.14 $^{+0.05}_{-0.07}$ &    7.1 &           0.8 &  14.6 $\pm$ 4.0 &  0.61 $\pm$ 0.12 &           0.6 &            14.0 &             21.7 \\
 115 &  308.1393 &  40.3291 &  219 &         15.9 &         10.7 &   0.18 $^{+0.04}_{-0.04}$ &   26.1 &           5.9 &  11.9 $\pm$ 1.1 &  0.55 $\pm$ 0.03 &           1.7 &            14.2 &             21.7 \\
 116 &  307.9058 &  40.3292 &  170 &         19.0 &         14.2 &   0.25 $^{+0.03}_{-0.02}$ &   69.5 &          18.0 &  11.8 $\pm$ 0.6 &  0.22 $\pm$ 0.01 &           1.1 &            14.4 &             21.9 \\
 117 &  307.8530 &  40.3319 &  214 &         10.8 &          9.3 &   0.14 $^{+-0.0}_{-0.03}$ &   12.3 &           1.5 &  11.9 $\pm$ 2.8 &  0.18 $\pm$ 0.03 &           1.0 &            14.2 &             21.9 \\
 118 &  307.5920 &  40.3363 &   52 &         17.8 &         13.3 &   0.22 $^{+0.05}_{-0.05}$ &    NaN &           NaN &  12.1 $\pm$ 2.5 &  0.18 $\pm$ 0.03 &          -0.1 &            13.9 &              NaN \\
 119 &  307.7139 &  40.3423 &  116 &         24.7 &         13.7 &   0.26 $^{+0.18}_{-0.08}$ &   41.7 &           8.0 &  10.2 $\pm$ 1.9 &  0.15 $\pm$ 0.02 &           0.2 &            14.0 &             21.6 \\
 120 &  307.8618 &  40.3560 &  185 &         26.1 &         20.5 &    0.32 $^{+0.06}_{-0.1}$ &   95.9 &          32.5 &  10.7 $\pm$ 1.8 &  0.42 $\pm$ 0.03 &           0.0 &            14.2 &             21.8 \\
 121 &  308.2126 &  40.3584 &  141 &         28.3 &         12.0 &   0.27 $^{+0.13}_{-0.12}$ &   28.2 &           5.0 &  11.8 $\pm$ 2.2 &  0.27 $\pm$ 0.04 &           0.8 &            14.0 &             21.7 \\
 122 &  308.1382 &  40.3657 &  159 &         22.3 &         14.5 &   0.25 $^{+0.09}_{-0.07}$ &   30.3 &           6.8 &  13.2 $\pm$ 2.7 &  0.57 $\pm$ 0.08 &           1.7 &            14.1 &             21.7 \\
 123 &  308.2442 &  40.3692 &  220 &         15.3 &          9.7 &   0.16 $^{+0.08}_{-0.09}$ &    9.9 &           1.8 &  12.2 $\pm$ 3.3 &  0.21 $\pm$ 0.04 &           0.5 &            14.1 &             21.7 \\
 124 &  307.8303 &  40.3736 &  150 &         26.6 &         21.1 &   0.32 $^{+0.06}_{-0.15}$ &  103.0 &          38.8 &  12.7 $\pm$ 2.0 &  0.58 $\pm$ 0.05 &           0.2 &            14.2 &             21.8 \\
 125 &  308.0717 &  40.3979 &  124 &         51.9 &         27.3 &   0.48 $^{+0.36}_{-0.31}$ &  101.2 &          25.4 &  16.2 $\pm$ 2.6 &  0.62 $\pm$ 0.08 &           0.7 &            13.7 &             21.8 \\
 126 &  308.0198 &  40.3785 &  210 &         15.9 &         13.1 &   0.18 $^{+0.08}_{-0.08}$ &   12.9 &           1.4 &  13.8 $\pm$ 2.6 &  0.21 $\pm$ 0.04 &           1.1 &            13.9 &             21.8 \\
 127 &  308.0229 &  40.3996 &   91 &         13.4 &          7.9 &   0.13 $^{+0.07}_{-0.03}$ &    6.0 &           0.1 &  17.2 $\pm$ 4.2 &   0.49 $\pm$ 0.1 &           0.5 &            14.2 &             21.8 \\
 128 &  308.1445 &  40.4052 &   84 &         11.0 &          8.6 &   0.12 $^{+0.03}_{-0.05}$ &    4.5 &           0.2 &  14.0 $\pm$ 3.6 &  0.43 $\pm$ 0.09 &           0.4 &            13.8 &             21.7 \\
 129 &  307.6897 &  40.4132 &  188 &         16.1 &          8.9 &   0.17 $^{+0.06}_{-0.07}$ &    NaN &           NaN &  11.9 $\pm$ 3.2 &  0.24 $\pm$ 0.05 &           9.4 &            13.9 &              NaN \\
 130 &  308.1384 &  40.4302 &  176 &         22.8 &         11.2 &   0.21 $^{+0.09}_{-0.06}$ &   16.1 &           2.7 &  15.6 $\pm$ 3.6 &  0.35 $\pm$ 0.07 &           0.1 &            13.8 &             21.7 \\
 131 &  308.0719 &  40.4565 &  108 &         30.3 &         13.5 &   0.25 $^{+0.15}_{-0.21}$ &   21.0 &           3.0 &  13.9 $\pm$ 3.8 &  0.37 $\pm$ 0.08 &           0.5 &            13.7 &             21.6 \\
 132 &  307.7029 &  40.4483 &   64 &         10.9 &          9.0 &   0.13 $^{+0.02}_{-0.02}$ &    NaN &           NaN &  19.7 $\pm$ 3.8 &  0.54 $\pm$ 0.09 &          10.0 &            14.3 &              NaN \\
\bottomrule
\end{tabular}


==> CygX_S_leaf_stats_virial.tex <==
\begin{tabular}{rrrrrrrrllrr}
\toprule
 ID &  $\alpha_{vir}$ &  $M_{vir}$ &  $\sigma_{nt}$ & log$|\Omega_G|$ & log$\Omega_K$ & log$|\Omega_{Pw}|$ &  log$|\Omega_{Pt}|$ & on-filament & hub & $N_{proto}$ & Bad N(H$_2$) Pixels \\& & (M$_\odot$) & (km s$^{-1}$) & (erg) & (erg) & (erg) & (erg) & & & \\\midrule
   0 &   2.38 &              22.9 &      0.33 &  43.5 &     43.6 &     44.1 &         NaN &        False &  False &           0 &         0 \\
   1 &   1.02 &              27.4 &      0.27 &  44.2 &     44.0 &     44.8 &         NaN &        False &  False &           0 &         0 \\
   2 &   0.73 &              13.4 &      0.17 &  43.9 &     43.6 &     44.4 &         NaN &         True &  False &           0 &         0 \\
   3 &   0.83 &              79.0 &      0.39 &  45.0 &     44.8 &     45.4 &         NaN &        False &  False &           1 &         0 \\
   4 &   1.75 &              41.0 &      0.38 &  44.1 &     44.1 &     44.6 &         NaN &        False &  False &           0 &         0 \\
   5 &   3.01 &              63.1 &      0.53 &  44.0 &     44.3 &     44.6 &         NaN &         True &  False &           0 &         0 \\
   6 &   6.32 &             309.2 &      1.07 &  44.6 &     45.2 &     44.9 &         NaN &         True &  False &           0 &         0 \\
   7 &   1.21 &              58.2 &      0.45 &  44.7 &     44.6 &     44.8 &         NaN &         True &  False &           0 &         0 \\
   8 &   2.21 &              71.2 &      0.54 &  44.4 &     44.5 &     44.7 &         NaN &         True &  False &           0 &         0 \\
   9 &   1.04 &              12.4 &      0.15 &  43.6 &     43.4 &     44.2 &         NaN &        False &  False &           0 &         0 \\
  10 &   1.19 &              55.1 &      0.39 &  44.6 &     44.5 &     44.9 &         NaN &         True &  False &           0 &         0 \\
  11 &   2.05 &              81.4 &      0.57 &  44.5 &     44.7 &     44.6 &         NaN &        False &  False &           0 &         0 \\
  12 &   1.33 &              53.0 &      0.45 &  44.6 &     44.5 &     44.6 &         NaN &        False &  False &           1 &         0 \\
  13 &   0.49 &              94.1 &      0.42 &  45.6 &     45.1 &     45.5 &         NaN &        False &  False &           3 &         0 \\
  14 &   0.59 &             163.4 &      0.58 &  45.9 &     45.5 &     45.5 &         NaN &        False &  False &           4 &         0 \\
  15 &   1.20 &              20.1 &      0.27 &  43.9 &     43.8 &     44.2 &         NaN &        False &  False &           1 &         0 \\
  16 &   1.00 &              50.0 &      0.35 &  44.6 &     44.4 &     45.0 &         NaN &        False &  False &           0 &         0 \\
  17 &   1.97 &              42.3 &      0.40 &  44.0 &     44.1 &     44.5 &         NaN &         True &  False &           1 &         0 \\
  18 &   1.69 &              98.8 &      0.53 &  44.8 &     44.8 &     44.9 &         NaN &         True &  False &           4 &         0 \\
  19 &   1.96 &             143.5 &      0.73 &  45.0 &     45.1 &     44.8 &         NaN &         True &  False &           3 &         0 \\
  20 &   5.22 &              43.0 &      0.52 &  43.4 &     43.9 &     43.9 &         NaN &        False &  False &           0 &         0 \\
  21 &   3.83 &             107.6 &      0.68 &  44.3 &     44.7 &     44.4 &         NaN &         True &  False &           1 &         0 \\
  22 &   3.01 &             133.8 &      0.76 &  44.7 &     44.9 &     44.6 &         NaN &         True &  False &           2 &         0 \\
  23 &   1.95 &              14.2 &      0.25 &  43.3 &     43.4 &     43.8 &         NaN &         True &  False &           1 &         0 \\
  24 &   9.50 &              74.0 &      0.71 &  43.3 &     44.1 &     44.0 &         NaN &         True &  False &           0 &         0 \\
  25 &   2.93 &              74.6 &      0.59 &  44.2 &     44.5 &     44.4 &         NaN &         True &  False &           0 &         0 \\
  26 &   1.59 &              75.2 &      0.45 &  44.6 &     44.6 &     44.9 &         NaN &         True &  False &           1 &         0 \\
  27 &   7.45 &             241.3 &      1.03 &  44.4 &     45.0 &     44.6 &         NaN &         True &  False &           0 &         0 \\
  28 &   3.86 &             127.6 &      0.69 &  44.3 &     44.7 &     44.8 &         NaN &         True &  False &           0 &         0 \\
  29 &   4.14 &              50.3 &      0.55 &  43.7 &     44.1 &     44.0 &         NaN &        False &  False &           1 &         0 \\
  30 &   5.63 &              65.6 &      0.58 &  43.6 &     44.2 &     44.1 &         NaN &        False &  False &           0 &         0 \\
  31 &   1.13 &              22.3 &      0.26 &  44.0 &     43.8 &     44.5 &         NaN &        False &  False &           0 &         0 \\
  32 &   2.50 &              34.0 &      0.38 &  43.8 &     44.0 &     44.1 &         NaN &        False &  False &           0 &         0 \\
  33 &   1.84 &              10.8 &      0.18 &  43.2 &     43.2 &     43.7 &         NaN &        False &  False &           1 &         0 \\
  34 &   2.92 &              25.5 &      0.38 &  43.4 &     43.7 &     44.0 &         NaN &        False &  False &           1 &         0 \\
  35 &   3.64 &              70.9 &      0.59 &  44.0 &     44.4 &     44.3 &         NaN &        False &  False &           0 &         0 \\
  36 &   2.69 &              25.7 &      0.35 &  43.5 &     43.7 &     44.1 &         NaN &        False &  False &           0 &         0 \\
  37 &   1.33 &              10.1 &      0.19 &  43.4 &     43.3 &     43.9 &         NaN &         True &  False &           0 &         0 \\
  38 &   2.30 &              50.8 &      0.47 &  44.1 &     44.3 &     44.5 &         NaN &        False &  False &           1 &         0 \\
  39 &   0.57 &              39.8 &      0.28 &  44.9 &     44.4 &     45.1 &         NaN &        False &  False &           2 &         0 \\
  40 &   1.34 &              35.3 &      0.32 &  44.2 &     44.1 &     44.7 &         NaN &        False &  False &           0 &         0 \\
  41 &   7.66 &              64.3 &      0.67 &  43.4 &     44.1 &     43.9 &         NaN &        False &  False &           0 &         0 \\
  42 &   0.80 &              35.6 &      0.30 &  44.5 &     44.2 &     44.9 &         NaN &        False &  False &           1 &         0 \\
  43 &   0.82 &              26.1 &      0.25 &  44.3 &     44.0 &     44.8 &         NaN &        False &  False &           0 &         0 \\
  44 &   0.43 &              36.8 &      0.29 &  45.1 &     44.5 &     45.1 &         NaN &        False &  False &           0 &         0 \\
  45 &   1.30 &               9.0 &      0.18 &  43.3 &     43.2 &     43.8 &         NaN &        False &  False &           0 &         0 \\
  46 &   0.56 &              64.2 &      0.37 &  45.3 &     44.8 &     45.3 &         NaN &        False &  False &           3 &         0 \\
  47 &   0.65 &              55.7 &      0.38 &  45.1 &     44.7 &     45.1 &         NaN &        False &  False &           1 &         0 \\
  48 &   0.60 &              11.5 &      0.14 &  44.0 &     43.5 &     44.6 &         NaN &        False &  False &           0 &         0 \\
  49 &   1.15 &             237.9 &      0.73 &  45.7 &     45.6 &     45.5 &         NaN &        False &  False &           2 &         0 \\
  50 &   0.96 &              25.7 &      0.30 &  44.2 &     44.0 &     44.5 &         NaN &        False &  False &           2 &         0 \\
  51 &   1.55 &              61.7 &      0.44 &  44.5 &     44.5 &     44.7 &         NaN &        False &  False &           0 &         0 \\
  52 &   0.49 &              34.1 &      0.26 &  44.9 &     44.3 &     45.2 &         NaN &        False &  False &           3 &         0 \\
  53 &   0.68 &              39.9 &      0.39 &  44.9 &     44.6 &     44.5 &         NaN &        False &  False &           1 &         0 \\
  54 &   1.27 &              35.4 &      0.37 &  44.3 &     44.2 &     44.5 &         NaN &        False &  False &           1 &         0 \\
  55 &   1.12 &              42.1 &      0.37 &  44.5 &     44.3 &     44.8 &         NaN &        False &  False &           0 &         0 \\
  56 &   3.87 &              43.3 &      0.51 &  43.7 &     44.0 &     44.1 &         NaN &        False &  False &           0 &         0 \\
  57 &   0.75 &              45.5 &      0.42 &  45.0 &     44.6 &     44.5 &         NaN &        False &  False &           1 &         0 \\
  58 &   1.58 &              21.8 &      0.30 &  43.8 &     43.8 &     44.3 &         NaN &        False &  False &           1 &         0 \\
  59 &   2.60 &              32.1 &      0.42 &  43.7 &     43.9 &     44.1 &         NaN &        False &  False &           0 &         0 \\
  60 &   1.41 &              10.0 &      0.22 &  43.3 &     43.3 &     43.9 &         NaN &         True &  False &           0 &         0 \\
  61 &   1.48 &             113.0 &      0.57 &  45.0 &     44.9 &     45.1 &         NaN &        False &  False &           0 &         0 \\
  62 &   8.71 &              73.0 &      0.77 &  43.5 &     44.2 &     43.8 &         NaN &        False &  False &           0 &         0 \\
  63 &  16.09 &             129.9 &      1.07 &  43.5 &     44.5 &     43.8 &         NaN &        False &  False &           0 &         0 \\
  64 &   2.05 &              76.6 &      0.52 &  44.5 &     44.6 &     44.7 &         NaN &        False &  False &           3 &         0 \\
  65 &   0.75 &              10.3 &      0.13 &  43.7 &     43.4 &     44.3 &         NaN &         True &  False &           0 &         0 \\
  66 &   1.67 &              16.2 &      0.30 &  43.6 &     43.6 &     43.9 &         NaN &        False &  False &           0 &         0 \\
  67 &   0.90 &              28.4 &      0.28 &  44.3 &     44.0 &     44.8 &         NaN &         True &  False &           0 &         0 \\
  68 &   1.37 &               8.7 &      0.21 &  43.3 &     43.2 &     43.7 &         NaN &         True &  False &           1 &         0 \\
  69 &   0.88 &               8.4 &      0.15 &  43.5 &     43.3 &     44.1 &         NaN &         True &  False &           0 &         0 \\
  70 &   3.61 &              42.3 &      0.48 &  43.6 &     44.0 &     44.2 &         NaN &         True &  False &           0 &         0 \\
  71 &   1.24 &              10.6 &      0.20 &  43.4 &     43.3 &     44.0 &         NaN &         True &  False &           0 &         0 \\
  72 &   1.44 &              24.0 &      0.28 &  43.9 &     43.8 &     44.4 &         NaN &        False &  False &           0 &         0 \\
  73 &   0.62 &              11.7 &      0.16 &  44.0 &     43.6 &     44.5 &         NaN &        False &  False &           0 &         0 \\
  74 &   1.78 &              42.8 &      0.44 &  44.2 &     44.3 &     44.3 &         NaN &        False &  False &           0 &         0 \\
  75 &   1.09 &              46.5 &      0.40 &  44.6 &     44.4 &     44.8 &         NaN &        False &  False &           1 &         0 \\
  76 &   2.30 &              29.0 &      0.37 &  43.8 &     43.9 &     44.0 &         NaN &        False &  False &           0 &         0 \\
  77 &   0.36 &              30.4 &      0.24 &  45.0 &     44.4 &     45.3 &         NaN &         True &  False &           0 &         0 \\
  78 &   0.90 &               7.5 &      0.16 &  43.5 &     43.2 &     43.9 &         NaN &         True &  False &           0 &         0 \\
  79 &   0.95 &               8.3 &      0.13 &  43.4 &     43.2 &     44.1 &         NaN &        False &  False &           0 &         0 \\
  80 &   0.50 &               6.4 &      0.07 &  43.8 &     43.3 &     44.1 &         NaN &         True &  False &           0 &         0 \\
  81 &   2.53 &              32.2 &      0.41 &  43.8 &     44.0 &     44.1 &         NaN &        False &  False &           0 &         0 \\
  82 &   1.69 &              13.1 &      0.23 &  43.4 &     43.4 &     43.9 &         NaN &         True &  False &           0 &         0 \\
  83 &   0.60 &             257.6 &      0.62 &  46.2 &     45.8 &     46.1 &         NaN &        False &  False &           4 &         0 \\
  84 &   2.83 &              19.4 &      0.34 &  43.3 &     43.5 &     43.9 &         NaN &        False &  False &           0 &         0 \\
  85 &   1.50 &               9.1 &      0.18 &  43.2 &     43.2 &     43.7 &         NaN &        False &  False &           0 &         0 \\
  86 &   0.92 &               6.4 &      0.09 &  43.2 &     43.0 &     44.0 &         NaN &        False &  False &           0 &         0 \\
  87 &   3.39 &              14.0 &      0.31 &  42.9 &     43.2 &     43.6 &         NaN &        False &  False &           0 &         0 \\
  88 &    NaN &              66.4 &      0.43 &   NaN &      NaN &      NaN &         NaN &        False &  False &           1 &         0 \\
  89 &   0.54 &               8.8 &      0.10 &  43.9 &     43.4 &     44.4 &         NaN &        False &  False &           0 &         0 \\
  90 &   0.92 &               8.1 &      0.10 &  43.3 &     43.1 &     44.2 &         NaN &        False &  False &           0 &         0 \\
  91 &    NaN &              17.1 &      0.29 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &         0 \\
  92 &    NaN &              27.9 &      0.36 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &         0 \\
  93 &   2.42 &              66.4 &      0.47 &  44.2 &     44.4 &     44.6 &        45.2 &         True &  False &           1 &         0 \\
  94 &   1.90 &              30.1 &      0.40 &  43.9 &     44.0 &     44.2 &         NaN &         True &  False &           0 &         0 \\
  95 &    NaN &              19.3 &      0.25 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &         0 \\
  96 &   0.89 &               6.7 &      0.12 &  43.4 &     43.1 &     43.9 &         NaN &        False &  False &           1 &         0 \\
  97 &   2.12 &              18.0 &      0.23 &  43.4 &     43.5 &     43.9 &        44.5 &         True &  False &           0 &         0 \\
  98 &    NaN &               8.7 &      0.18 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &         0 \\
  99 &   1.29 &               9.1 &      0.15 &  43.3 &     43.2 &     44.0 &         NaN &        False &  False &           0 &         0 \\
 100 &    NaN &              18.8 &      0.29 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &         0 \\
 101 &   3.41 &              24.4 &      0.30 &  43.2 &     43.6 &     44.0 &        44.5 &        False &  False &           0 &         0 \\
 102 &    NaN &             159.2 &      0.76 &   NaN &      NaN &      NaN &         NaN &        False &  False &           3 &         0 \\
 103 &    NaN &               4.9 &      0.07 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &         0 \\
 104 &    NaN &              41.8 &      0.42 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &         0 \\
 105 &   0.85 &               9.4 &      0.18 &  43.7 &     43.4 &     44.0 &         NaN &         True &  False &           0 &         0 \\
 106 &   0.24 &              57.3 &      0.33 &  45.8 &     45.0 &     45.5 &         NaN &         True &  False &           4 &         0 \\
 107 &   4.12 &              21.4 &      0.36 &  43.0 &     43.4 &     43.9 &         NaN &        False &  False &           0 &         0 \\
 108 &   0.99 &             114.0 &      0.64 &  45.4 &     45.2 &     45.0 &         NaN &         True &  False &           1 &         0 \\
 109 &   1.34 &              34.7 &      0.35 &  44.2 &     44.1 &     44.7 &         NaN &         True &  False &           0 &         0 \\
 110 &   0.45 &             169.2 &      0.55 &  46.2 &     45.6 &     45.8 &         NaN &        False &  False &           6 &         0 \\
 111 &   1.33 &               7.2 &      0.12 &  43.1 &     43.0 &     43.9 &         NaN &        False &  False &           0 &         0 \\
 112 &    NaN &              59.2 &      0.46 &   NaN &      NaN &      NaN &         NaN &        False &  False &           2 &         0 \\
 113 &    NaN &              10.2 &      0.17 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &         0 \\
 114 &   7.53 &              53.3 &      0.60 &  43.3 &     43.9 &     44.0 &         NaN &        False &  False &           0 &         0 \\
 115 &   2.20 &              57.3 &      0.55 &  44.3 &     44.4 &     44.4 &         NaN &        False &  False &           0 &         0 \\
 116 &   0.29 &              19.9 &      0.21 &  45.0 &     44.3 &     44.9 &         NaN &         True &  False &           2 &         0 \\
 117 &   0.76 &               9.4 &      0.17 &  43.7 &     43.4 &     44.2 &         NaN &        False &  False &           0 &         0 \\
 118 &    NaN &              14.6 &      0.17 &   NaN &      NaN &      NaN &         NaN &        False &  False &           1 &         0 \\
 119 &   0.32 &              13.3 &      0.14 &  44.5 &     43.8 &     44.7 &         NaN &        False &  False &           0 &         0 \\
 120 &   0.66 &              62.8 &      0.41 &  45.2 &     44.8 &     45.2 &         NaN &        False &  False &           0 &         0 \\
 121 &   0.95 &              26.7 &      0.26 &  44.2 &     44.0 &     44.8 &         NaN &        False &  False &           1 &         0 \\
 122 &   2.85 &              86.4 &      0.56 &  44.3 &     44.5 &     44.8 &         NaN &        False &  False &           0 &         0 \\
 123 &   1.25 &              12.3 &      0.20 &  43.5 &     43.4 &     44.1 &         NaN &        False &  False &           0 &         0 \\
 124 &   1.08 &             111.3 &      0.57 &  45.2 &     45.1 &     45.2 &         NaN &        False &  False &           1 &         0 \\
 125 &   1.96 &             198.3 &      0.62 &  45.0 &     45.1 &     45.7 &         NaN &         True &  False &           0 &         0 \\
 126 &   1.10 &              14.3 &      0.20 &  43.7 &     43.5 &     44.4 &         NaN &         True &  False &           0 &         0 \\
 127 &   5.70 &              34.3 &      0.48 &  43.2 &     43.7 &     43.9 &         NaN &         True &  False &           0 &         0 \\
 128 &   5.54 &              25.1 &      0.43 &  43.0 &     43.5 &     43.8 &         NaN &        False &  False &           0 &         0 \\
 129 &    NaN &              14.4 &      0.22 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &         0 \\
 130 &   2.05 &              33.1 &      0.33 &  43.8 &     43.9 &     44.5 &         NaN &         True &  False &           0 &         0 \\
 131 &   2.01 &              42.2 &      0.36 &  44.0 &     44.1 &     44.7 &         NaN &         True &  False &           0 &         0 \\
 132 &    NaN &              43.0 &      0.53 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &         0 \\
\bottomrule
\end{tabular}


==> M16_leaf_stats.tex <==
\begin{tabular}{rrrrrrlrrllrrr}
\toprule
ID & RA & decl. & PA & $\sigma_{major}$ & $\sigma_{minor}$ &  $R_{eff}$ &  $M_{obs}$ &  $M_{clip}$ &  $T_K$ &  $\sigma_{NH_3}$ &  $V_{LSR, NH_3}$ &  log($N_{para-NH_3}$) &  log($N_{H_2}$) \\& (deg) & (deg) & (deg) & ($\arcsec$) & ($\arcsec$) & (pc) & (M$_\odot$) & (M$_\odot$) & (K) & (km s$^{-1}$) & (km s$^{-1}$) & (cm$^{-2}$) & (cm$^{-2}$) \\\midrule
  0 &  274.7056 & -13.8326 &   70 &          8.9 &          8.1 &   0.16 $^{+-0.0}_{-0.03}$ &    14.1 &           2.4 &  16.6 $\pm$ 3.5 &  0.53 $\pm$ 0.09 &          22.8 &            13.6 &              NaN \\
  1 &  274.7125 & -13.8160 &   58 &         12.7 &         12.2 &   0.25 $^{+0.04}_{-0.03}$ &    36.4 &          15.6 &  22.0 $\pm$ 2.4 &  0.47 $\pm$ 0.05 &          24.9 &            14.3 &             21.5 \\
  2 &  274.5189 & -13.8058 &  141 &         23.3 &          8.5 &   0.25 $^{+0.14}_{-0.11}$ &    34.1 &           1.7 &  13.0 $\pm$ 2.0 &  0.37 $\pm$ 0.04 &          20.2 &            13.8 &             21.8 \\
  3 &  274.5047 & -13.7902 &  143 &         31.9 &         16.9 &   0.46 $^{+0.29}_{-0.15}$ &   135.9 &          42.9 &  12.9 $\pm$ 0.9 &  0.28 $\pm$ 0.02 &          20.8 &            14.1 &             21.9 \\
  4 &  274.5413 & -13.8005 &  218 &         17.1 &          7.9 &   0.19 $^{+0.12}_{-0.08}$ &    22.2 &           1.5 &  12.2 $\pm$ 1.9 &   0.4 $\pm$ 0.04 &          21.0 &            14.0 &             21.9 \\
  5 &  274.5439 & -13.7509 &  113 &         61.1 &         35.8 &    0.98 $^{+0.6}_{-0.42}$ &  1405.7 &         931.9 &  16.3 $\pm$ 0.6 &  0.61 $\pm$ 0.02 &          20.8 &            14.4 &             22.2 \\
  6 &  274.8560 & -13.7584 &  171 &         18.7 &         15.2 &    0.3 $^{+0.13}_{-0.12}$ &    76.7 &          21.4 &  15.7 $\pm$ 2.9 &   0.72 $\pm$ 0.1 &          21.6 &            13.8 &             21.9 \\
  7 &  274.7816 & -13.7548 &  177 &         17.9 &         13.6 &   0.34 $^{+0.14}_{-0.07}$ &    92.1 &          43.3 &  22.9 $\pm$ 1.5 &  0.75 $\pm$ 0.04 &          24.7 &            14.3 &             21.8 \\
  8 &  274.6596 & -13.7542 &  181 &          9.7 &          8.1 &   0.16 $^{+0.04}_{-0.02}$ &    10.2 &           0.6 &  17.1 $\pm$ 3.1 &  0.25 $\pm$ 0.05 &          20.2 &            13.8 &             21.7 \\
  9 &  274.6960 & -13.7402 &  194 &         15.3 &         11.7 &   0.26 $^{+0.05}_{-0.03}$ &    84.2 &          40.1 &  24.3 $\pm$ 1.6 &  0.72 $\pm$ 0.04 &          19.9 &            14.2 &             21.9 \\
 10 &  274.6080 & -13.7393 &  166 &         14.4 &         10.1 &   0.22 $^{+0.03}_{-0.05}$ &    22.9 &           4.1 &  11.7 $\pm$ 0.8 &  0.23 $\pm$ 0.01 &          21.7 &            14.1 &             21.8 \\
 11 &  274.6275 & -13.7322 &  127 &         18.9 &          9.0 &   0.23 $^{+0.09}_{-0.08}$ &    24.4 &           3.3 &  11.6 $\pm$ 1.0 &   0.2 $\pm$ 0.01 &          21.8 &            14.0 &             21.8 \\
 12 &  274.6955 & -13.7213 &  117 &         14.7 &          8.9 &    0.2 $^{+0.09}_{-0.05}$ &    37.0 &           8.3 &  21.9 $\pm$ 1.9 &  0.62 $\pm$ 0.05 &          20.7 &            14.0 &             22.0 \\
 13 &  274.6686 & -13.7007 &   88 &         27.2 &         14.5 &   0.37 $^{+0.15}_{-0.15}$ &   127.1 &          40.2 &  23.1 $\pm$ 2.7 &   0.6 $\pm$ 0.06 &          28.6 &            13.8 &             22.0 \\
 14 &  274.6405 & -13.7108 &  200 &         11.3 &         10.2 &   0.19 $^{+0.02}_{-0.02}$ &    20.8 &           3.1 &  13.1 $\pm$ 2.0 &  0.29 $\pm$ 0.04 &          22.3 &            14.1 &             21.9 \\
 15 &  274.7550 & -13.7123 &  176 &         16.3 &          6.1 &   0.16 $^{+0.13}_{-0.06}$ &    13.4 &           1.0 &  16.8 $\pm$ 3.9 &  0.14 $\pm$ 0.03 &          22.4 &            13.9 &             21.8 \\
 16 &  274.5915 & -13.7040 &  213 &         26.2 &         13.3 &   0.37 $^{+0.19}_{-0.12}$ &    99.6 &          40.9 &  22.4 $\pm$ 2.2 &  0.66 $\pm$ 0.06 &          26.4 &            13.9 &             21.9 \\
 17 &  274.7298 & -13.6936 &  136 &         29.4 &         12.9 &   0.34 $^{+0.22}_{-0.12}$ &    89.9 &          28.7 &  18.4 $\pm$ 2.4 &  0.59 $\pm$ 0.07 &          20.2 &            14.0 &             21.9 \\
 18 &  274.7992 & -13.6927 &  126 &         14.7 &          5.7 &   0.16 $^{+0.08}_{-0.06}$ &    15.1 &           0.8 &  13.3 $\pm$ 4.4 &  0.78 $\pm$ 0.17 &          22.8 &            14.3 &             21.9 \\
 19 &  274.5480 & -13.6897 &   48 &         15.5 &         11.7 &   0.26 $^{+0.06}_{-0.04}$ &    80.0 &          35.5 &  22.2 $\pm$ 1.5 &  0.55 $\pm$ 0.03 &          19.2 &            14.2 &             22.0 \\
 20 &  274.5642 & -13.6761 &  163 &         17.8 &          7.5 &   0.18 $^{+0.08}_{-0.08}$ &    19.3 &           3.2 &  25.9 $\pm$ 4.7 &  0.84 $\pm$ 0.13 &          24.7 &            14.0 &             21.9 \\
 21 &  274.5344 & -13.6704 &  220 &         21.1 &         11.1 &   0.29 $^{+0.12}_{-0.08}$ &    79.9 &          25.4 &  19.4 $\pm$ 1.3 &   0.5 $\pm$ 0.03 &          25.4 &            14.1 &             22.0 \\
 22 &  274.7923 & -13.6701 &  177 &         30.3 &         11.8 &   0.34 $^{+0.22}_{-0.17}$ &    77.9 &          10.4 &  12.9 $\pm$ 1.7 &  0.23 $\pm$ 0.03 &          22.9 &            14.0 &             21.9 \\
 23 &  274.7307 & -13.6715 &  141 &         15.4 &          9.5 &    0.2 $^{+0.08}_{-0.08}$ &    26.9 &           2.6 &  16.2 $\pm$ 3.7 &  1.72 $\pm$ 0.27 &          22.7 &            14.9 &             21.9 \\
 24 &  274.8157 & -13.6569 &  145 &         14.3 &         11.8 &   0.22 $^{+0.11}_{-0.06}$ &    48.9 &          14.0 &  18.4 $\pm$ 3.1 &  0.94 $\pm$ 0.13 &          21.9 &            14.5 &             22.0 \\
 25 &  274.5110 & -13.6579 &  213 &         13.9 &          8.4 &   0.19 $^{+0.03}_{-0.04}$ &    32.0 &           7.7 &  21.5 $\pm$ 2.1 &  0.51 $\pm$ 0.05 &          24.9 &            13.5 &             22.0 \\
 26 &  274.7497 & -13.6565 &   52 &         11.5 &          9.1 &   0.19 $^{+0.04}_{-0.04}$ &    23.0 &           1.2 &  11.6 $\pm$ 4.5 &  0.68 $\pm$ 0.13 &          22.6 &            14.2 &             21.9 \\
 27 &  274.7133 & -13.6527 &   95 &         11.8 &          7.8 &   0.16 $^{+0.02}_{-0.05}$ &    18.5 &           2.1 &  15.4 $\pm$ 3.9 &  0.29 $\pm$ 0.07 &          25.1 &            13.5 &             22.0 \\
 28 &  274.7320 & -13.6481 &  153 &         21.6 &         13.3 &    0.31 $^{+0.17}_{-0.1}$ &    62.8 &          14.0 &  13.0 $\pm$ 3.0 &  0.46 $\pm$ 0.08 &          23.5 &            14.1 &             21.9 \\
 29 &  274.6854 & -13.6516 &  164 &         14.3 &          6.4 &   0.17 $^{+0.04}_{-0.07}$ &    24.1 &           2.0 &  16.3 $\pm$ 2.2 &  0.61 $\pm$ 0.07 &          22.9 &            14.0 &             22.0 \\
 30 &  274.6849 & -13.6319 &   54 &         34.4 &         14.6 &   0.39 $^{+0.29}_{-0.23}$ &   144.8 &          46.7 &  16.3 $\pm$ 1.9 &   0.6 $\pm$ 0.06 &          23.8 &            13.9 &             22.0 \\
 31 &  274.5111 & -13.6214 &  135 &         13.3 &          7.1 &   0.17 $^{+0.03}_{-0.06}$ &    58.6 &           4.4 &  16.4 $\pm$ 0.4 &  0.45 $\pm$ 0.01 &          19.5 &            14.5 &             22.2 \\
 32 &  274.4910 & -13.6162 &  211 &         20.7 &         13.3 &   0.28 $^{+0.12}_{-0.09}$ &   187.1 &          36.3 &  16.1 $\pm$ 0.4 &  0.49 $\pm$ 0.01 &          19.8 &            14.6 &             22.3 \\
 33 &  274.4583 & -13.6144 &  219 &         19.7 &         13.4 &   0.29 $^{+0.08}_{-0.06}$ &    78.8 &          18.6 &  23.2 $\pm$ 2.9 &  0.65 $\pm$ 0.08 &          23.9 &            13.5 &             22.1 \\
 34 &  274.6487 & -13.6150 &  154 &          8.1 &          7.3 &  0.14 $^{+0.01}_{--0.01}$ &     9.7 &           0.7 &  19.5 $\pm$ 3.4 &  0.28 $\pm$ 0.05 &          20.6 &            13.4 &             21.8 \\
 35 &  274.6239 & -13.5921 &  208 &         22.1 &         17.9 &   0.33 $^{+0.22}_{-0.15}$ &    53.9 &          15.1 &  16.6 $\pm$ 3.3 &  0.42 $\pm$ 0.08 &          20.5 &            13.7 &             21.8 \\
 36 &  274.5341 & -13.5826 &  187 &         34.0 &         18.5 &   0.48 $^{+0.18}_{-0.17}$ &   270.9 &         102.3 &  17.0 $\pm$ 1.0 &  0.52 $\pm$ 0.03 &          19.1 &            14.2 &             22.1 \\
 37 &  274.4981 & -13.5851 &  222 &         23.0 &         12.2 &   0.31 $^{+0.12}_{-0.07}$ &   126.3 &          39.4 &  15.8 $\pm$ 0.9 &  0.58 $\pm$ 0.03 &          18.9 &            14.2 &             22.2 \\
 38 &  274.5939 & -13.5876 &  175 &         16.4 &          8.3 &    0.21 $^{+0.1}_{-0.05}$ &    17.8 &           2.9 &  15.6 $\pm$ 3.2 &  0.47 $\pm$ 0.08 &          20.0 &            13.7 &             21.7 \\
 39 &  274.4785 & -13.5665 &   51 &         21.2 &         10.6 &    0.27 $^{+0.2}_{-0.06}$ &   104.3 &          14.8 &  17.5 $\pm$ 1.0 &  0.61 $\pm$ 0.03 &          18.9 &            14.2 &             22.1 \\
 40 &  274.5505 & -13.5559 &   87 &         19.1 &         11.6 &    0.25 $^{+0.1}_{-0.08}$ &    43.9 &           8.5 &  19.8 $\pm$ 3.5 &   0.66 $\pm$ 0.1 &          17.8 &            13.7 &             21.9 \\
 41 &  274.4450 & -13.5347 &  178 &         18.5 &         14.1 &   0.27 $^{+0.05}_{-0.08}$ &    73.9 &          17.4 &  17.5 $\pm$ 2.3 &   0.6 $\pm$ 0.07 &          19.9 &            13.7 &             21.9 \\
 42 &  274.5085 & -13.5329 &  122 &         12.4 &         11.1 &   0.22 $^{+0.07}_{-0.07}$ &    25.8 &           6.4 &  12.2 $\pm$ 3.7 &  1.03 $\pm$ 0.18 &          19.0 &            13.9 &             21.8 \\
\bottomrule
\end{tabular}


==> M16_leaf_stats_virial.tex <==
\begin{tabular}{rrrrrrrrllrr}
\toprule
 ID &  $\alpha_{vir}$ &  $M_{vir}$ &  $\sigma_{nt}$ & log$|\Omega_G|$ & log$\Omega_K$ & log$|\Omega_{Pw}|$ &  log$|\Omega_{Pt}|$ & on-filament & hub & $N_{proto}$ & Bad N(H$_2$) Pixels \\& & (M$_\odot$) & (km s$^{-1}$) & (erg) & (erg) & (erg) & (erg) & & & \\\midrule
  0 &   3.37 &              47.6 &      0.52 &  43.8 &     44.1 &      NaN &        45.0 &        False &  False &           3 &         0 \\
  1 &   1.80 &              65.6 &      0.46 &  44.4 &     44.5 &     44.7 &         NaN &        False &  False &           1 &         0 \\
  2 &   1.21 &              41.3 &      0.36 &  44.4 &     44.3 &     45.1 &         NaN &        False &  False &           0 &         0 \\
  3 &   0.36 &              49.2 &      0.26 &  45.3 &     44.7 &     46.0 &         NaN &        False &  False &           1 &         0 \\
  4 &   1.55 &              34.3 &      0.39 &  44.1 &     44.1 &     44.8 &         NaN &        False &  False &           0 &         0 \\
  5 &   0.27 &             381.2 &      0.60 &  47.0 &     46.2 &     47.3 &         NaN &        False &   True &           2 &         0 \\
  6 &   2.06 &             157.8 &      0.71 &  45.0 &     45.1 &     45.4 &         NaN &        False &  False &           1 &         0 \\
  7 &   2.18 &             200.6 &      0.75 &  45.1 &     45.2 &     45.5 &         NaN &        False &  False &           0 &         0 \\
  8 &   1.68 &              17.2 &      0.23 &  43.5 &     43.5 &     44.4 &         NaN &        False &  False &           1 &         0 \\
  9 &   1.70 &             143.5 &      0.71 &  45.1 &     45.2 &     45.3 &         NaN &         True &  False &           2 &         0 \\
 10 &   0.79 &              18.2 &      0.22 &  44.1 &     43.8 &     44.9 &         NaN &        False &  False &           1 &         0 \\
 11 &   0.63 &              15.5 &      0.18 &  44.1 &     43.7 &     44.9 &         NaN &        False &  False &           1 &         0 \\
 12 &   2.26 &              83.8 &      0.61 &  44.5 &     44.7 &     45.0 &         NaN &         True &  False &           1 &         0 \\
 13 &   1.17 &             148.4 &      0.59 &  45.3 &     45.2 &     45.8 &         NaN &         True &  False &           2 &         0 \\
 14 &   1.08 &              22.4 &      0.28 &  44.1 &     43.9 &     44.8 &         NaN &        False &  False &           0 &         0 \\
 15 &   0.79 &              10.6 &      0.10 &  43.8 &     43.5 &     44.6 &         NaN &        False &  False &           0 &         0 \\
 16 &   1.75 &             174.0 &      0.66 &  45.1 &     45.2 &     45.7 &         NaN &        False &  False &           3 &         0 \\
 17 &   1.41 &             126.8 &      0.58 &  45.1 &     45.0 &     45.6 &         NaN &         True &  False &           1 &         0 \\
 18 &   6.21 &              93.6 &      0.77 &  43.9 &     44.5 &     44.6 &         NaN &         True &  False &           0 &         0 \\
 19 &   1.15 &              91.8 &      0.54 &  45.1 &     45.0 &     45.3 &         NaN &        False &  False &           1 &         0 \\
 20 &   6.71 &             129.3 &      0.83 &  44.0 &     44.7 &     44.7 &         NaN &        False &  False &           0 &         0 \\
 21 &   1.02 &              81.6 &      0.49 &  45.1 &     44.9 &     45.4 &         NaN &         True &  False &           1 &         0 \\
 22 &   0.38 &              29.3 &      0.22 &  45.0 &     44.3 &     45.6 &         NaN &         True &  False &           0 &         0 \\
 23 &  20.62 &             554.1 &      1.72 &  44.3 &     45.4 &     44.9 &         NaN &         True &  False &           0 &         0 \\
 24 &   3.93 &             192.4 &      0.93 &  44.7 &     45.1 &     45.1 &         NaN &         True &  False &           0 &         0 \\
 25 &   1.83 &              58.4 &      0.50 &  44.4 &     44.5 &     44.9 &         NaN &         True &  False &           0 &         0 \\
 26 &   3.75 &              86.3 &      0.67 &  44.2 &     44.5 &     44.8 &         NaN &         True &  False &           0 &         0 \\
 27 &   1.02 &              18.8 &      0.27 &  44.0 &     43.9 &     44.6 &         NaN &         True &  False &           0 &         0 \\
 28 &   1.14 &              71.5 &      0.45 &  44.8 &     44.7 &     45.5 &         NaN &         True &  False &           0 &         0 \\
 29 &   2.76 &              66.5 &      0.61 &  44.2 &     44.5 &     44.7 &         NaN &         True &  False &           0 &         0 \\
 30 &   1.02 &             148.1 &      0.59 &  45.4 &     45.2 &     45.8 &         NaN &         True &  False &           0 &         0 \\
 31 &   0.68 &              39.8 &      0.44 &  45.0 &     44.6 &     45.0 &         NaN &         True &  False &           1 &         0 \\
 32 &   0.41 &              77.1 &      0.48 &  45.8 &     45.2 &     45.7 &         NaN &         True &  False &           1 &         0 \\
 33 &   1.68 &             132.1 &      0.64 &  45.0 &     45.1 &     45.5 &         NaN &         True &  False &           0 &         0 \\
 34 &   1.87 &              18.1 &      0.26 &  43.5 &     43.6 &     44.3 &         NaN &        False &  False &           0 &         0 \\
 35 &   1.29 &              69.6 &      0.41 &  44.7 &     44.6 &     45.4 &         NaN &        False &  False &           0 &         0 \\
 36 &   0.53 &             143.9 &      0.51 &  45.9 &     45.4 &     46.2 &         NaN &        False &  False &           0 &         0 \\
 37 &   0.88 &             110.7 &      0.58 &  45.4 &     45.2 &     45.7 &         NaN &         True &  False &           1 &         0 \\
 38 &   2.94 &              52.2 &      0.46 &  43.9 &     44.2 &     44.7 &         NaN &        False &  False &           0 &         0 \\
 39 &   1.04 &             108.3 &      0.61 &  45.3 &     45.1 &     45.5 &         NaN &         True &  False &           0 &         0 \\
 40 &   2.63 &             115.2 &      0.65 &  44.6 &     44.8 &     45.2 &         NaN &        False &  False &           0 &         0 \\
 41 &   1.44 &             106.6 &      0.60 &  45.0 &     45.0 &     45.3 &         NaN &         True &  False &           0 &         0 \\
 42 &   8.56 &             220.9 &      1.03 &  44.2 &     44.9 &     44.9 &         NaN &        False &  False &           0 &         0 \\
\bottomrule
\end{tabular}


==> M17_leaf_stats.tex <==
\begin{tabular}{rrrrrrlrrllrrr}
\toprule
ID & RA & decl. & PA & $\sigma_{major}$ & $\sigma_{minor}$ &  $R_{eff}$ &  $M_{obs}$ &  $M_{clip}$ &  $T_K$ &  $\sigma_{NH_3}$ &  $V_{LSR, NH_3}$ &  log($N_{para-NH_3}$) &  log($N_{H_2}$) \\& (deg) & (deg) & (deg) & ($\arcsec$) & ($\arcsec$) & (pc) & (M$_\odot$) & (M$_\odot$) & (K) & (km s$^{-1}$) & (km s$^{-1}$) & (cm$^{-2}$) & (cm$^{-2}$) \\\midrule
  0 &  274.7744 & -16.6161 &  172 &         18.1 &         11.5 &  0.28 $^{+0.14}_{-0.09}$ &   121.9 &          18.1 &  12.4 $\pm$ 2.8 &  0.32 $\pm$ 0.05 &          17.6 &            14.2 &             22.2 \\
  1 &  274.8064 & -16.5884 &  125 &         35.6 &         24.4 &  0.64 $^{+0.42}_{-0.19}$ &   664.3 &         229.8 &  15.1 $\pm$ 1.8 &  0.44 $\pm$ 0.04 &          18.9 &            14.1 &             22.2 \\
  2 &  274.8333 & -16.5475 &  191 &         18.3 &          6.7 &  0.21 $^{+0.11}_{-0.09}$ &    66.3 &          10.5 &  15.9 $\pm$ 1.8 &  0.34 $\pm$ 0.04 &          19.1 &            14.1 &             22.2 \\
  3 &  274.8293 & -16.5325 &  144 &         18.4 &         10.5 &  0.26 $^{+0.12}_{-0.09}$ &   109.3 &          41.9 &  18.1 $\pm$ 1.8 &  0.37 $\pm$ 0.04 &          19.3 &            14.2 &             22.3 \\
  4 &  274.8074 & -16.5044 &  123 &         35.9 &         23.8 &  0.63 $^{+0.45}_{-0.17}$ &  1480.8 &         878.3 &  19.5 $\pm$ 0.5 &  0.68 $\pm$ 0.01 &          18.4 &            14.7 &             22.3 \\
  5 &  274.7729 & -16.5110 &  156 &         20.3 &         13.8 &  0.33 $^{+0.09}_{-0.05}$ &   270.3 &          53.7 &  17.2 $\pm$ 0.8 &  0.53 $\pm$ 0.02 &          17.6 &            14.3 &             22.3 \\
  6 &  274.8011 & -16.3247 &  225 &         20.5 &         15.8 &  0.43 $^{+0.12}_{-0.07}$ &   317.6 &          92.4 &  16.5 $\pm$ 1.3 &  0.41 $\pm$ 0.03 &          21.9 &            14.2 &             22.2 \\
  7 &  274.8543 & -16.3014 &  161 &         20.7 &         11.6 &  0.34 $^{+0.12}_{-0.08}$ &   141.6 &          30.6 &  16.1 $\pm$ 1.7 &  0.23 $\pm$ 0.03 &          22.3 &            14.1 &             22.1 \\
  8 &  275.0490 & -16.2479 &  136 &         18.8 &         10.5 &  0.22 $^{+0.13}_{-0.13}$ &    53.0 &           8.5 &  27.6 $\pm$ 2.9 &  0.94 $\pm$ 0.09 &          19.7 &            13.7 &             22.5 \\
  9 &  275.0884 & -16.2424 &  212 &         27.9 &         10.1 &  0.33 $^{+0.19}_{-0.16}$ &   683.8 &         298.6 &  24.2 $\pm$ 0.3 &  1.28 $\pm$ 0.01 &          18.8 &            14.9 &             22.7 \\
 10 &  275.0293 & -16.2319 &  165 &         25.7 &         19.2 &   0.4 $^{+0.19}_{-0.32}$ &   215.5 &          67.8 &  27.8 $\pm$ 3.7 &  0.88 $\pm$ 0.11 &          21.7 &            13.8 &             22.4 \\
 11 &  275.0869 & -16.2116 &  133 &         27.4 &         22.6 &  0.49 $^{+0.26}_{-0.08}$ &  2634.3 &        2131.9 &  30.0 $\pm$ 0.3 &  1.52 $\pm$ 0.01 &          19.4 &            15.0 &             22.8 \\
 12 &  275.0469 & -16.1802 &   58 &         12.7 &         12.0 &  0.27 $^{+0.02}_{-0.04}$ &   253.6 &          95.5 &  24.8 $\pm$ 1.1 &  1.62 $\pm$ 0.05 &          20.0 &            14.6 &             22.6 \\
 13 &  275.0805 & -16.1622 &  203 &         10.7 &          9.2 &   0.2 $^{+0.01}_{-0.02}$ &    74.2 &          24.4 &  27.4 $\pm$ 2.0 &  0.47 $\pm$ 0.03 &          18.2 &            14.4 &             22.6 \\
 14 &  275.0363 & -16.1586 &   65 &         11.7 &          7.0 &  0.18 $^{+0.02}_{-0.04}$ &    44.6 &           5.2 &  25.4 $\pm$ 4.7 &  0.74 $\pm$ 0.12 &          17.2 &            13.9 &             22.4 \\
 15 &  275.0635 & -16.1364 &   74 &         43.2 &         16.0 &  0.55 $^{+0.51}_{-0.25}$ &   681.3 &         332.0 &  24.0 $\pm$ 1.0 &  0.88 $\pm$ 0.03 &          17.6 &            14.5 &             22.4 \\
 16 &  275.1484 & -16.0998 &  110 &         14.3 &          9.6 &  0.25 $^{+0.06}_{-0.02}$ &    79.1 &          26.4 &  28.0 $\pm$ 2.2 &  0.66 $\pm$ 0.04 &          19.3 &            14.3 &             22.0 \\
 17 &  275.1070 & -16.0935 &   89 &         18.8 &         14.1 &  0.36 $^{+0.11}_{-0.03}$ &   147.9 &          46.2 &  26.1 $\pm$ 2.2 &  0.63 $\pm$ 0.05 &          17.1 &            13.9 &             22.1 \\
 18 &  275.0655 & -16.0987 &   92 &         15.0 &          8.5 &  0.23 $^{+0.05}_{-0.04}$ &   102.0 &          18.6 &  24.5 $\pm$ 1.7 &  0.81 $\pm$ 0.05 &          17.3 &            13.8 &             22.2 \\
 19 &  275.0350 & -16.1007 &  224 &         15.2 &          7.8 &   0.17 $^{+0.1}_{-0.06}$ &    35.3 &           1.7 &  14.6 $\pm$ 4.0 &  0.91 $\pm$ 0.16 &          18.8 &            13.9 &             22.2 \\
 20 &  275.1407 & -16.0711 &   63 &         25.2 &         10.8 &   0.32 $^{+0.31}_{-0.1}$ &   132.5 &          44.1 &  26.0 $\pm$ 2.2 &  0.64 $\pm$ 0.05 &          17.4 &            14.0 &             22.1 \\
 21 &  275.0581 & -16.0814 &   71 &         16.9 &          8.3 &  0.23 $^{+0.13}_{-0.05}$ &    82.9 &          10.1 &  21.8 $\pm$ 2.0 &   0.6 $\pm$ 0.04 &          18.2 &            14.3 &             22.2 \\
 22 &  275.0761 & -16.0734 &  115 &         14.2 &          9.7 &  0.24 $^{+0.06}_{-0.03}$ &    70.0 &           8.1 &  22.7 $\pm$ 3.2 &  0.53 $\pm$ 0.07 &          17.4 &            14.1 &             22.2 \\
 23 &  275.0306 & -16.0751 &   72 &         13.4 &          8.6 &  0.19 $^{+0.05}_{-0.07}$ &    57.2 &          10.7 &  23.8 $\pm$ 3.8 &  0.55 $\pm$ 0.08 &          18.6 &            14.1 &             22.2 \\
 24 &  275.1040 & -16.0628 &  144 &         21.4 &         13.9 &   0.35 $^{+0.16}_{-0.1}$ &   125.5 &          28.1 &  21.0 $\pm$ 2.3 &  0.39 $\pm$ 0.04 &          19.3 &            14.1 &             22.2 \\
 25 &  275.0416 & -16.0511 &  115 &         29.8 &          9.9 &  0.26 $^{+0.23}_{-0.22}$ &   104.0 &          17.4 &  19.0 $\pm$ 3.0 &   0.7 $\pm$ 0.09 &          19.1 &            13.8 &             22.2 \\
 26 &  275.1101 & -16.0363 &   89 &         13.9 &          6.8 &  0.19 $^{+0.06}_{-0.05}$ &    39.6 &           2.0 &  25.9 $\pm$ 3.1 &  0.47 $\pm$ 0.05 &          18.9 &            13.8 &             22.2 \\
 27 &  275.0458 & -16.0286 &  211 &         16.5 &         11.8 &   0.24 $^{+0.1}_{-0.08}$ &    78.0 &          26.8 &  20.1 $\pm$ 3.4 &   0.65 $\pm$ 0.1 &          19.2 &            13.9 &             22.1 \\
 28 &  275.0279 & -16.0305 &   77 &         12.4 &          9.1 &  0.21 $^{+0.09}_{-0.03}$ &    60.6 &          10.8 &  19.3 $\pm$ 2.8 &  0.32 $\pm$ 0.05 &          21.6 &            14.0 &             22.1 \\
 29 &  275.1376 & -16.0251 &  118 &         16.3 &         10.2 &  0.27 $^{+0.08}_{-0.04}$ &   229.8 &         100.8 &  26.2 $\pm$ 0.8 &  0.86 $\pm$ 0.02 &          20.7 &            14.7 &             22.2 \\
 30 &  274.9847 & -16.0227 &  131 &         15.2 &         11.8 &  0.28 $^{+0.03}_{-0.05}$ &   103.9 &          28.7 &  20.0 $\pm$ 3.1 &  0.23 $\pm$ 0.04 &          19.7 &            14.1 &             22.1 \\
 31 &  275.1587 & -16.0225 &   89 &         12.3 &          5.6 &  0.16 $^{+0.07}_{-0.03}$ &    36.3 &           4.7 &  21.2 $\pm$ 1.2 &   0.4 $\pm$ 0.02 &          19.0 &            14.1 &             22.1 \\
 32 &  275.0543 & -16.0058 &  157 &         18.6 &         10.2 &  0.26 $^{+0.09}_{-0.15}$ &    69.4 &          15.6 &  18.7 $\pm$ 3.9 &  0.43 $\pm$ 0.08 &          19.6 &            13.8 &             22.1 \\
 33 &  275.1489 & -15.9936 &  148 &         19.2 &          7.8 &   0.23 $^{+0.1}_{-0.07}$ &   126.2 &          10.9 &  22.2 $\pm$ 0.6 &  0.94 $\pm$ 0.02 &          21.2 &            14.4 &             22.2 \\
 34 &  274.9853 & -15.9901 &   65 &         16.8 &         10.2 &  0.25 $^{+0.09}_{-0.13}$ &    80.1 &          24.5 &  17.6 $\pm$ 4.1 &   0.46 $\pm$ 0.1 &          20.3 &            14.0 &             22.1 \\
 35 &  275.1398 & -15.9835 &  105 &          9.3 &          6.7 &  0.16 $^{+0.0}_{--0.01}$ &    62.9 &           7.4 &  20.5 $\pm$ 0.4 &  0.43 $\pm$ 0.01 &          20.4 &            14.4 &             22.2 \\
 36 &  275.1584 & -15.9672 &   98 &         14.3 &         10.3 &  0.24 $^{+0.03}_{-0.03}$ &    93.2 &          17.6 &  22.6 $\pm$ 1.1 &  0.62 $\pm$ 0.03 &          21.5 &            14.2 &             22.1 \\
 37 &  275.1605 & -15.9448 &   93 &         15.4 &          5.4 &  0.16 $^{+0.09}_{-0.09}$ &    28.4 &           6.0 &  27.0 $\pm$ 2.4 &   0.6 $\pm$ 0.04 &          20.3 &            13.9 &             22.0 \\
\bottomrule
\end{tabular}


==> M17_leaf_stats_virial.tex <==
\begin{tabular}{rrrrrrrrllrr}
\toprule
 ID &  $\alpha_{vir}$ &  $M_{vir}$ &  $\sigma_{nt}$ & log$|\Omega_G|$ & log$\Omega_K$ & log$|\Omega_{Pw}|$ &  log$|\Omega_{Pt}|$ & on-filament & hub & $N_{proto}$ & Bad N(H$_2$) Pixels \\& & (M$_\odot$) & (km s$^{-1}$) & (erg) & (erg) & (erg) & (erg) & & & \\\midrule
  0 &   0.31 &              37.2 &      0.31 &  45.4 &     44.7 &     45.8 &         NaN &        False &  False &           0 &      0.00 \\
  1 &   0.21 &             141.0 &      0.43 &  46.5 &     45.7 &     46.9 &         NaN &        False &  False &           0 &      0.00 \\
  2 &   0.48 &              31.5 &      0.32 &  45.0 &     44.5 &     45.5 &         NaN &        False &  False &           2 &      0.00 \\
  3 &   0.43 &              46.5 &      0.35 &  45.4 &     44.8 &     45.8 &         NaN &        False &  False &           0 &      0.00 \\
  4 &   0.21 &             310.9 &      0.68 &  47.2 &     46.4 &     47.0 &         NaN &        False &   True &           3 &      0.00 \\
  5 &   0.39 &             104.3 &      0.53 &  46.1 &     45.4 &     46.2 &         NaN &        False &  False &           2 &      0.00 \\
  6 &   0.27 &              86.2 &      0.40 &  46.1 &     45.3 &     46.4 &         NaN &        False &  False &           1 &      0.00 \\
  7 &   0.23 &              32.4 &      0.21 &  45.5 &     44.6 &     46.0 &         NaN &        False &  False &           1 &      0.00 \\
  8 &   3.78 &             200.3 &      0.94 &  44.8 &     45.2 &     45.8 &        46.0 &        False &  False &           0 &      0.00 \\
  9 &   0.76 &             517.9 &      1.27 &  46.9 &     46.5 &     46.5 &        47.0 &        False &  False &           1 &      0.00 \\
 10 &   1.46 &             314.2 &      0.87 &  45.8 &     45.7 &     46.5 &        46.8 &        False &  False &           2 &      0.00 \\
 11 &   0.42 &            1103.0 &      1.52 &  47.9 &     47.3 &     47.2 &        47.4 &        False &   True &           1 &      0.59 \\
 12 &   2.69 &             681.6 &      1.61 &  46.1 &     46.3 &     46.2 &        46.6 &        False &  False &           0 &      0.00 \\
 13 &   0.77 &              57.3 &      0.45 &  45.1 &     44.8 &     45.8 &        45.5 &         True &  False &           1 &      0.00 \\
 14 &   2.37 &             105.6 &      0.74 &  44.8 &     44.9 &     45.4 &        45.6 &        False &  False &           0 &      0.00 \\
 15 &   0.64 &             433.8 &      0.87 &  46.6 &     46.2 &     46.9 &        47.1 &         True &  False &           8 &      0.00 \\
 16 &   1.55 &             122.3 &      0.65 &  45.1 &     45.1 &     45.5 &        45.8 &         True &  False &           1 &      0.00 \\
 17 &   1.07 &             157.7 &      0.62 &  45.5 &     45.3 &     46.1 &        46.4 &        False &  False &           1 &      0.00 \\
 18 &   1.54 &             157.3 &      0.80 &  45.4 &     45.3 &     45.6 &        45.9 &         True &  False &           1 &      0.00 \\
 19 &   3.98 &             140.4 &      0.90 &  44.6 &     45.0 &     45.2 &        45.4 &         True &  False &           0 &      0.00 \\
 20 &   1.12 &             148.2 &      0.63 &  45.4 &     45.3 &     45.9 &        46.2 &        False &  False &           0 &      0.00 \\
 21 &   1.08 &              89.7 &      0.59 &  45.2 &     45.0 &     45.5 &        45.5 &         True &  False &           0 &      0.00 \\
 22 &   1.13 &              78.9 &      0.52 &  45.0 &     44.9 &     45.6 &         NaN &         True &  False &           0 &      0.00 \\
 23 &   1.17 &              67.0 &      0.54 &  44.9 &     44.8 &     45.3 &         NaN &         True &  False &           0 &      0.00 \\
 24 &   0.55 &              69.5 &      0.37 &  45.4 &     44.9 &     46.0 &         NaN &         True &  False &           1 &      0.00 \\
 25 &   1.31 &             136.0 &      0.70 &  45.3 &     45.2 &     45.7 &         NaN &         True &  False &           0 &      0.00 \\
 26 &   1.33 &              52.5 &      0.46 &  44.6 &     44.6 &     45.2 &         NaN &        False &  False &           0 &      0.00 \\
 27 &   1.39 &             108.7 &      0.64 &  45.1 &     45.1 &     45.5 &         NaN &         True &  False &           0 &      0.00 \\
 28 &   0.52 &              31.3 &      0.30 &  45.0 &     44.5 &     45.4 &         NaN &         True &  False &           0 &      0.00 \\
 29 &   0.90 &             207.4 &      0.85 &  46.0 &     45.7 &     45.7 &         NaN &         True &  False &           0 &      0.00 \\
 30 &   0.29 &              29.9 &      0.21 &  45.3 &     44.6 &     45.7 &         NaN &        False &  False &           1 &      0.00 \\
 31 &   0.92 &              33.3 &      0.39 &  44.6 &     44.4 &     45.0 &         NaN &        False &  False &           0 &      0.00 \\
 32 &   0.86 &              59.8 &      0.42 &  45.0 &     44.7 &     45.6 &         NaN &         True &  False &           0 &      0.00 \\
 33 &   1.60 &             201.5 &      0.94 &  45.6 &     45.6 &     45.5 &         NaN &         True &  False &           0 &      0.00 \\
 34 &   0.79 &              63.3 &      0.45 &  45.1 &     44.8 &     45.5 &         NaN &        False &  False &           0 &      0.00 \\
 35 &   0.59 &              37.2 &      0.42 &  45.1 &     44.7 &     45.0 &         NaN &         True &  False &           0 &      0.00 \\
 36 &   1.07 &              99.4 &      0.61 &  45.3 &     45.1 &     45.5 &         NaN &         True &  False &           2 &      0.00 \\
 37 &   2.30 &              65.3 &      0.59 &  44.4 &     44.6 &     44.9 &         NaN &         True &  False &           0 &      0.00 \\
\bottomrule
\end{tabular}


==> MonR1_leaf_stats.tex <==
\begin{tabular}{rrrrrrlrrllrrr}
\toprule
ID & RA & decl. & PA & $\sigma_{major}$ & $\sigma_{minor}$ &  $R_{eff}$ &  $M_{obs}$ &  $M_{clip}$ &  $T_K$ &  $\sigma_{NH_3}$ &  $V_{LSR, NH_3}$ &  log($N_{para-NH_3}$) &  log($N_{H_2}$) \\& (deg) & (deg) & (deg) & ($\arcsec$) & ($\arcsec$) & (pc) & (M$_\odot$) & (M$_\odot$) & (K) & (km s$^{-1}$) & (km s$^{-1}$) & (cm$^{-2}$) & (cm$^{-2}$) \\\midrule
  0 &  98.1463 &  10.1702 &  193 &         27.5 &         16.0 &  0.22 $^{+0.13}_{-0.05}$ &  31.5 &          16.4 &  11.6 $\pm$ 0.7 &  0.19 $\pm$ 0.01 &           3.0 &            14.1 &             21.7 \\
  1 &  98.1130 &  10.1790 &  146 &         13.6 &         12.1 &  0.12 $^{+0.02}_{-0.01}$ &   5.0 &           1.1 &   9.6 $\pm$ 1.6 &  0.12 $\pm$ 0.01 &           2.8 &            13.8 &             21.5 \\
  2 &  98.1653 &  10.2836 &  103 &         15.0 &          6.3 &  0.08 $^{+0.03}_{-0.03}$ &   3.1 &           0.8 &  10.0 $\pm$ 2.6 &  0.21 $\pm$ 0.03 &           3.7 &            13.9 &             21.7 \\
  3 &  98.2036 &  10.2998 &  191 &         15.9 &         11.7 &  0.12 $^{+0.01}_{-0.03}$ &   5.8 &           1.5 &  11.9 $\pm$ 3.0 &  0.14 $\pm$ 0.03 &           4.0 &            13.7 &             21.7 \\
  4 &  98.2801 &  10.3043 &  222 &         14.6 &         10.6 &   0.1 $^{+0.01}_{-0.05}$ &   4.1 &           1.0 &  17.2 $\pm$ 4.1 &   0.46 $\pm$ 0.1 &           4.6 &            13.7 &             21.5 \\
  5 &  98.1659 &  10.3084 &  106 &         16.2 &          9.1 &   0.1 $^{+0.05}_{-0.05}$ &  11.1 &           2.2 &  11.8 $\pm$ 0.9 &  0.43 $\pm$ 0.02 &           3.2 &            14.1 &             22.0 \\
  6 &  98.0466 &  10.3127 &   65 &         13.9 &         10.6 &  0.11 $^{+0.03}_{-0.02}$ &   4.9 &           1.4 &  11.3 $\pm$ 3.2 &  0.13 $\pm$ 0.02 &           3.9 &            13.3 &             21.6 \\
  7 &  98.1325 &  10.3134 &  190 &         22.5 &         13.1 &  0.16 $^{+0.05}_{-0.04}$ &  25.4 &           7.0 &  10.9 $\pm$ 0.8 &   0.3 $\pm$ 0.01 &           4.0 &            14.2 &             22.0 \\
  8 &  98.1705 &  10.3265 &  127 &         16.6 &         10.0 &  0.11 $^{+0.04}_{-0.02}$ &  14.6 &           5.1 &  12.0 $\pm$ 0.8 &  0.46 $\pm$ 0.02 &           3.2 &            14.2 &             22.1 \\
  9 &  98.1923 &  10.3266 &   76 &         12.4 &          9.3 &  0.09 $^{+0.01}_{-0.01}$ &   4.2 &           1.4 &   9.9 $\pm$ 2.7 &  0.15 $\pm$ 0.02 &           5.8 &            13.9 &             21.8 \\
 10 &  98.2816 &  10.3361 &  137 &         19.2 &         14.0 &  0.15 $^{+0.06}_{-0.03}$ &   8.7 &           3.7 &  12.7 $\pm$ 2.5 &  0.22 $\pm$ 0.03 &           5.7 &            13.8 &             21.6 \\
 11 &  98.2637 &  10.3304 &   95 &         13.7 &          5.7 &  0.08 $^{+0.03}_{-0.04}$ &   1.9 &           0.5 &  13.9 $\pm$ 4.0 &  0.46 $\pm$ 0.11 &           5.5 &            14.3 &             21.6 \\
 12 &  98.1460 &  10.3341 &  189 &         21.0 &         17.2 &  0.18 $^{+0.05}_{-0.02}$ &  38.3 &           6.8 &  11.0 $\pm$ 0.9 &  0.49 $\pm$ 0.02 &           4.9 &            14.1 &             22.1 \\
 13 &  98.2529 &  10.3342 &  193 &         14.0 &          9.2 &  0.08 $^{+0.04}_{-0.03}$ &   3.0 &           0.5 &  14.4 $\pm$ 3.6 &  0.38 $\pm$ 0.08 &           5.2 &            14.0 &             21.7 \\
 14 &  98.0824 &  10.3539 &   79 &         23.4 &         15.0 &  0.17 $^{+0.08}_{-0.06}$ &  21.8 &           8.6 &  13.2 $\pm$ 2.0 &  0.37 $\pm$ 0.04 &           4.2 &            14.0 &             21.9 \\
 15 &  98.2299 &  10.3456 &   95 &         13.6 &          8.0 &  0.08 $^{+0.03}_{-0.04}$ &   2.9 &           0.3 &  14.0 $\pm$ 4.3 &   0.39 $\pm$ 0.1 &           5.3 &            14.3 &             21.7 \\
 16 &  98.1065 &  10.3618 &   94 &         23.3 &         18.0 &   0.16 $^{+0.1}_{-0.08}$ &  20.2 &           6.1 &  11.7 $\pm$ 2.8 &  0.37 $\pm$ 0.05 &           5.2 &            13.9 &             22.0 \\
 17 &  98.1789 &  10.3609 &   45 &         14.7 &          9.9 &  0.08 $^{+0.04}_{-0.06}$ &   3.3 &           0.2 &  14.6 $\pm$ 4.0 &  0.53 $\pm$ 0.11 &           3.8 &            14.0 &             21.8 \\
 18 &  98.1664 &  10.3775 &  108 &         26.1 &         19.2 &  0.19 $^{+0.08}_{-0.06}$ &  18.2 &           3.0 &  13.7 $\pm$ 2.7 &  0.38 $\pm$ 0.06 &           4.6 &            13.5 &             21.8 \\
 19 &  98.0911 &  10.3683 &   61 &         13.6 &          5.5 &  0.08 $^{+0.03}_{-0.02}$ &   4.9 &           0.3 &  12.5 $\pm$ 4.4 &   0.8 $\pm$ 0.17 &           4.8 &            14.1 &             22.0 \\
 20 &  98.0842 &  10.3892 &  175 &         11.6 &         11.1 &   0.1 $^{+0.02}_{-0.01}$ &   7.3 &           0.9 &  11.3 $\pm$ 3.9 &  0.41 $\pm$ 0.08 &           3.9 &            13.8 &             22.0 \\
 21 &  98.2783 &  10.4050 &  214 &         16.4 &         11.6 &  0.13 $^{+0.06}_{-0.02}$ &   8.1 &           2.0 &   9.9 $\pm$ 2.7 &  0.16 $\pm$ 0.02 &           5.7 &            13.7 &             21.7 \\
 22 &  98.2684 &  10.4338 &   79 &         13.0 &         10.9 &  0.11 $^{+0.01}_{-0.01}$ &   7.3 &           0.9 &  11.2 $\pm$ 2.0 &  0.12 $\pm$ 0.01 &           4.7 &            13.8 &             21.8 \\
 23 &  98.2325 &  10.4327 &  182 &          9.8 &          8.6 &  0.08 $^{+0.02}_{-0.02}$ &   2.6 &           0.1 &  10.4 $\pm$ 4.0 &  0.11 $\pm$ 0.03 &           5.4 &            14.1 &             21.8 \\
 24 &  98.0901 &  10.4340 &  221 &         13.0 &          5.7 &  0.08 $^{+0.04}_{-0.01}$ &   4.4 &           0.5 &  11.5 $\pm$ 4.1 &  0.45 $\pm$ 0.09 &           5.5 &            13.8 &             22.0 \\
 25 &  98.0668 &  10.4412 &  109 &         13.4 &          9.0 &   0.1 $^{+0.03}_{-0.03}$ &   5.4 &           0.4 &  13.4 $\pm$ 4.4 &  0.74 $\pm$ 0.15 &           5.6 &            13.9 &             21.9 \\
 26 &  98.0064 &  10.4718 &  169 &         11.9 &          8.3 &  0.09 $^{+0.01}_{-0.02}$ &   3.0 &           0.9 &  11.1 $\pm$ 3.1 &  0.22 $\pm$ 0.04 &           5.7 &            13.8 &             21.7 \\
 27 &  98.1381 &  10.4738 &  199 &         14.7 &          6.8 &  0.08 $^{+0.03}_{-0.05}$ &   3.9 &           0.2 &  13.3 $\pm$ 4.0 &  0.91 $\pm$ 0.17 &           4.6 &            14.3 &             22.0 \\
 28 &  98.1835 &  10.4983 &   89 &         35.2 &         21.2 &   0.23 $^{+0.13}_{-0.1}$ &  44.7 &          16.9 &   9.7 $\pm$ 1.2 &  0.23 $\pm$ 0.01 &           5.0 &            14.0 &             22.0 \\
 29 &  97.9987 &  10.4836 &  153 &         11.1 &          7.1 &  0.08 $^{+0.02}_{-0.02}$ &   3.1 &           0.3 &  14.4 $\pm$ 3.9 &  0.32 $\pm$ 0.08 &           5.6 &            13.7 &             21.7 \\
 30 &  98.1446 &  10.4947 &  219 &         18.0 &         10.7 &  0.12 $^{+0.05}_{-0.04}$ &  15.9 &           4.3 &  10.5 $\pm$ 1.2 &  0.27 $\pm$ 0.02 &           6.5 &            13.9 &             22.1 \\
 31 &  98.0548 &  10.4896 &  200 &         11.5 &          5.8 &  0.08 $^{+0.01}_{-0.02}$ &   2.7 &           0.2 &  11.1 $\pm$ 3.3 &  0.14 $\pm$ 0.03 &           6.3 &            13.8 &             21.7 \\
 32 &  98.0209 &  10.4940 &   68 &          8.8 &          7.7 &   0.08 $^{+-0.0}_{-0.0}$ &   2.2 &           0.4 &  10.0 $\pm$ 3.7 &  0.13 $\pm$ 0.02 &           6.2 &            13.2 &             21.7 \\
 33 &  98.2285 &  10.4957 &  159 &         11.4 &          8.5 &  0.08 $^{+0.03}_{-0.01}$ &   4.0 &           0.3 &  12.5 $\pm$ 4.0 &   0.47 $\pm$ 0.1 &           6.5 &            13.8 &             21.8 \\
 34 &  98.1558 &  10.5080 &  224 &         10.0 &          7.7 &    0.08 $^{+0.0}_{-0.0}$ &   6.8 &           1.4 &  10.3 $\pm$ 0.6 &  0.17 $\pm$ 0.01 &           6.4 &            14.2 &             22.1 \\
 35 &  98.1488 &  10.5244 &  112 &         24.5 &         14.0 &  0.17 $^{+0.11}_{-0.05}$ &  34.7 &          12.3 &   9.6 $\pm$ 0.8 &  0.27 $\pm$ 0.01 &           6.4 &            14.2 &             22.1 \\
 36 &  98.1240 &  10.5279 &  216 &         14.0 &         10.4 &   0.1 $^{+0.02}_{-0.02}$ &   6.9 &           0.9 &  12.5 $\pm$ 3.1 &  0.51 $\pm$ 0.08 &           5.5 &            13.5 &             22.0 \\
 37 &  98.2619 &  10.5496 &  176 &         40.3 &         19.7 &  0.22 $^{+0.16}_{-0.17}$ &  29.9 &          10.4 &  14.1 $\pm$ 3.0 &  0.49 $\pm$ 0.08 &           4.3 &            13.8 &             21.8 \\
 38 &  98.1646 &  10.5529 &   70 &         15.0 &          5.3 &  0.07 $^{+0.04}_{-0.03}$ &   3.4 &           0.2 &  12.9 $\pm$ 4.4 &  1.22 $\pm$ 0.24 &           5.8 &            14.4 &             21.9 \\
 39 &  98.1753 &  10.5613 &   63 &         20.1 &         14.9 &  0.14 $^{+0.06}_{-0.08}$ &  12.7 &           2.2 &  11.9 $\pm$ 4.1 &  1.19 $\pm$ 0.23 &           4.9 &            14.6 &             21.9 \\
 40 &  98.1388 &  10.5997 &   64 &         32.3 &         13.3 &   0.19 $^{+0.12}_{-0.1}$ &  20.7 &           6.4 &  11.4 $\pm$ 2.0 &  0.19 $\pm$ 0.02 &           6.8 &            13.9 &             21.8 \\
\bottomrule
\end{tabular}


==> MonR1_leaf_stats_virial.tex <==
\begin{tabular}{rrrrrrrrllrr}
\toprule
 ID &  $\alpha_{vir}$ &  $M_{vir}$ &  $\sigma_{nt}$ & log$|\Omega_G|$ & log$\Omega_K$ & log$|\Omega_{Pw}|$ &  log$|\Omega_{Pt}|$ & on-filament & hub & $N_{proto}$ & Bad N(H$_2$) Pixels \\& & (M$_\odot$) & (km s$^{-1}$) & (erg) & (erg) & (erg) & (erg) & & & \\\midrule
  0 &   0.47 &              14.8 &      0.18 &  44.4 &     43.8 &     44.6 &         NaN &         True &  False &           1 &         0 \\
  1 &   1.00 &               4.9 &      0.10 &  43.0 &     42.8 &     43.6 &         NaN &         True &  False &           0 &         0 \\
  2 &   1.85 &               5.7 &      0.20 &  42.8 &     42.8 &     43.3 &         NaN &         True &  False &           0 &         0 \\
  3 &   1.06 &               6.2 &      0.11 &  43.2 &     43.0 &     43.8 &         NaN &         True &  False &           0 &         0 \\
  4 &   6.16 &              25.0 &      0.45 &  42.9 &     43.5 &     43.4 &         NaN &        False &  False &           0 &         0 \\
  5 &   1.84 &              20.3 &      0.42 &  43.8 &     43.9 &     43.9 &         NaN &         True &  False &           1 &         0 \\
  6 &   1.09 &               5.3 &      0.11 &  43.1 &     42.9 &     43.5 &         NaN &        False &  False &           0 &         0 \\
  7 &   0.71 &              18.0 &      0.29 &  44.3 &     44.0 &     44.5 &         NaN &         True &  False &           1 &         0 \\
  8 &   1.84 &              27.0 &      0.46 &  44.0 &     44.0 &     44.1 &         NaN &         True &  False &           1 &         0 \\
  9 &   1.12 &               4.7 &      0.14 &  43.0 &     42.8 &     43.6 &         NaN &        False &  False &           0 &         0 \\
 10 &   1.35 &              11.8 &      0.21 &  43.4 &     43.4 &     44.0 &         NaN &         True &  False &           0 &         0 \\
 11 &   9.01 &              17.5 &      0.45 &  42.4 &     43.2 &     43.1 &         NaN &         True &  False &           0 &         0 \\
 12 &   1.18 &              45.1 &      0.48 &  44.6 &     44.5 &     44.7 &         NaN &         True &  False &           0 &         0 \\
 13 &   4.87 &              14.7 &      0.37 &  42.7 &     43.2 &     43.3 &         NaN &         True &  False &           0 &         0 \\
 14 &   1.23 &              26.9 &      0.36 &  44.2 &     44.1 &     44.4 &         NaN &         True &  False &           1 &         0 \\
 15 &   5.28 &              15.4 &      0.38 &  42.7 &     43.2 &     43.3 &         NaN &         True &  False &           0 &         0 \\
 16 &   1.28 &              25.9 &      0.36 &  44.1 &     44.0 &     44.4 &         NaN &         True &  False &           0 &         0 \\
 17 &   7.66 &              25.5 &      0.52 &  42.8 &     43.5 &     43.5 &         NaN &         True &  False &           0 &         0 \\
 18 &   1.78 &              32.3 &      0.37 &  44.0 &     44.0 &     44.5 &         NaN &         True &  False &           0 &         0 \\
 19 &   9.81 &              47.6 &      0.80 &  43.2 &     44.0 &     43.5 &         NaN &         True &  False &           0 &         0 \\
 20 &   2.64 &              19.4 &      0.41 &  43.4 &     43.7 &     43.8 &         NaN &         True &  False &           0 &         0 \\
 21 &   0.82 &               6.7 &      0.14 &  43.4 &     43.1 &     43.9 &         NaN &         True &  False &           0 &         0 \\
 22 &   0.72 &               5.2 &      0.09 &  43.4 &     43.0 &     43.8 &         NaN &         True &  False &           0 &         0 \\
 23 &   1.20 &               3.1 &      0.09 &  42.7 &     42.5 &     43.3 &         NaN &        False &  False &           0 &         0 \\
 24 &   3.81 &              16.7 &      0.45 &  43.1 &     43.5 &     43.4 &         NaN &         True &  False &           0 &         0 \\
 25 &   9.77 &              53.2 &      0.74 &  43.2 &     44.0 &     43.7 &         NaN &         True &  False &           0 &         0 \\
 26 &   2.19 &               6.6 &      0.21 &  42.7 &     42.9 &     43.4 &         NaN &        False &  False &           0 &         0 \\
 27 &  15.43 &              60.5 &      0.91 &  43.0 &     44.0 &     43.5 &         NaN &         True &  False &           0 &         0 \\
 28 &   0.40 &              18.0 &      0.22 &  44.6 &     44.0 &     44.9 &         NaN &         True &  False &           1 &         0 \\
 29 &   3.29 &              10.2 &      0.31 &  42.8 &     43.1 &     43.2 &         NaN &        False &  False &           0 &         0 \\
 30 &   0.72 &              11.5 &      0.26 &  44.0 &     43.7 &     44.2 &         NaN &         True &  False &           0 &         0 \\
 31 &   1.36 &               3.7 &      0.12 &  42.7 &     42.6 &     43.2 &         NaN &        False &  False &           0 &         0 \\
 32 &   1.50 &               3.2 &      0.10 &  42.5 &     42.5 &     43.2 &         NaN &         True &  False &           0 &         0 \\
 33 &   5.08 &              20.5 &      0.47 &  43.0 &     43.5 &     43.4 &         NaN &         True &  False &           0 &         0 \\
 34 &   0.68 &               4.6 &      0.16 &  43.5 &     43.1 &     43.7 &         NaN &         True &  False &           0 &         0 \\
 35 &   0.45 &              15.6 &      0.26 &  44.6 &     44.0 &     44.6 &         NaN &         True &  False &           0 &         0 \\
 36 &   4.10 &              28.4 &      0.50 &  43.4 &     43.8 &     43.9 &         NaN &         True &  False &           0 &         0 \\
 37 &   1.96 &              58.5 &      0.48 &  44.3 &     44.4 &     44.7 &         NaN &         True &  False &           0 &         0 \\
 38 &  29.94 &             102.0 &      1.22 &  42.9 &     44.2 &     43.4 &         NaN &         True &  False &           0 &         0 \\
 39 &  14.50 &             183.5 &      1.19 &  43.8 &     44.7 &     44.1 &         NaN &         True &  False &           0 &         0 \\
 40 &   0.62 &              12.9 &      0.18 &  44.1 &     43.6 &     44.5 &         NaN &         True &  False &           1 &         0 \\
\bottomrule
\end{tabular}


==> MonR2_leaf_stats.tex <==
\begin{tabular}{rrrrrrlrrllrrr}
\toprule
ID & RA & decl. & PA & $\sigma_{major}$ & $\sigma_{minor}$ &  $R_{eff}$ &  $M_{obs}$ &  $M_{clip}$ &  $T_K$ &  $\sigma_{NH_3}$ &  $V_{LSR, NH_3}$ &  log($N_{para-NH_3}$) &  log($N_{H_2}$) \\& (deg) & (deg) & (deg) & ($\arcsec$) & ($\arcsec$) & (pc) & (M$_\odot$) & (M$_\odot$) & (K) & (km s$^{-1}$) & (km s$^{-1}$) & (cm$^{-2}$) & (cm$^{-2}$) \\\midrule
  0 &  91.8054 & -6.4832 &  122 &         30.7 &         12.0 &  0.16 $^{+0.11}_{-0.07}$ &    6.4 &           1.9 &  12.3 $\pm$ 2.7 &  0.18 $\pm$ 0.03 &          10.0 &            13.8 &             21.4 \\
  1 &  91.7917 & -6.4735 &  190 &         31.1 &         13.9 &   0.13 $^{+0.12}_{-0.1}$ &    3.6 &           0.6 &  14.5 $\pm$ 4.2 &   0.42 $\pm$ 0.1 &          11.2 &            14.1 &             21.5 \\
  2 &  92.0198 & -6.4617 &  219 &         26.4 &         17.1 &   0.18 $^{+0.1}_{-0.06}$ &    8.9 &           3.2 &  13.7 $\pm$ 3.0 &  0.19 $\pm$ 0.03 &          10.5 &            13.3 &             21.5 \\
  3 &  91.9051 & -6.4493 &  191 &         32.1 &         19.4 &    0.2 $^{+0.14}_{-0.1}$ &    9.6 &           2.6 &  16.9 $\pm$ 3.9 &   0.53 $\pm$ 0.1 &           9.6 &            14.0 &             21.6 \\
  4 &  91.8010 & -6.4466 &  168 &         43.4 &         22.7 &   0.29 $^{+0.17}_{-0.2}$ &   26.8 &           9.3 &  12.1 $\pm$ 1.6 &   0.2 $\pm$ 0.02 &          11.9 &            13.9 &             21.5 \\
  5 &  91.9928 & -6.4526 &  192 &         17.0 &         13.2 &  0.13 $^{+0.06}_{-0.01}$ &    5.7 &           1.3 &  14.2 $\pm$ 2.5 &  0.16 $\pm$ 0.03 &          10.9 &            13.6 &             21.6 \\
  6 &  91.9640 & -6.4419 &  221 &         22.6 &         10.7 &  0.14 $^{+0.07}_{-0.06}$ &   14.0 &           3.1 &  15.5 $\pm$ 1.6 &  0.36 $\pm$ 0.03 &          10.8 &            13.7 &             21.9 \\
  7 &  92.0189 & -6.4322 &  183 &         14.9 &          9.8 &   0.1 $^{+0.05}_{-0.03}$ &    2.8 &           0.6 &  19.4 $\pm$ 2.7 &  0.33 $\pm$ 0.05 &          10.4 &            13.5 &             21.6 \\
  8 &  91.9949 & -6.4246 &  211 &         23.0 &         13.6 &  0.16 $^{+0.05}_{-0.06}$ &   12.8 &           5.4 &  16.7 $\pm$ 2.0 &  0.34 $\pm$ 0.04 &          11.0 &            13.5 &             21.7 \\
  9 &  92.0984 & -6.4198 &  165 &         27.5 &         11.4 &   0.13 $^{+0.09}_{-0.1}$ &    4.2 &           1.2 &  17.0 $\pm$ 3.0 &  0.28 $\pm$ 0.05 &           9.7 &            13.3 &             21.4 \\
 10 &  92.1238 & -6.4213 &  191 &         21.7 &          9.2 &  0.12 $^{+0.05}_{-0.05}$ &    2.9 &           1.0 &  15.7 $\pm$ 2.8 &   0.3 $\pm$ 0.05 &           9.4 &            13.2 &             21.3 \\
 11 &  92.2422 & -6.4156 &  168 &         14.3 &          9.6 &  0.11 $^{+0.04}_{-0.03}$ &    NaN &           NaN &  11.4 $\pm$ 2.1 &  0.12 $\pm$ 0.02 &           9.6 &            13.9 &              NaN \\
 12 &  92.1978 & -6.4067 &   67 &         24.1 &         11.9 &   0.13 $^{+0.1}_{-0.09}$ &    3.2 &           1.7 &  13.8 $\pm$ 3.8 &  0.17 $\pm$ 0.04 &           9.3 &            13.3 &             21.3 \\
 13 &  91.8567 & -6.4151 &  178 &         26.9 &         10.5 &  0.15 $^{+0.13}_{-0.05}$ &    7.6 &           1.7 &  13.9 $\pm$ 1.5 &  0.23 $\pm$ 0.03 &           9.6 &            14.0 &             21.6 \\
 14 &  92.0781 & -6.4106 &   54 &         17.5 &          8.5 &  0.09 $^{+0.04}_{-0.04}$ &    1.9 &           0.4 &  14.8 $\pm$ 3.9 &  0.24 $\pm$ 0.06 &          10.0 &            13.7 &             21.4 \\
 15 &  92.0269 & -6.4147 &  166 &         10.1 &          7.8 &  0.08 $^{+0.01}_{-0.01}$ &    2.7 &           0.4 &  15.5 $\pm$ 1.9 &  0.34 $\pm$ 0.04 &          10.6 &            13.6 &             21.6 \\
 16 &  91.9512 & -6.4166 &  193 &         12.1 &          6.2 &  0.08 $^{+0.03}_{-0.01}$ &    8.7 &           1.0 &  19.0 $\pm$ 0.8 &  0.34 $\pm$ 0.02 &          11.1 &            14.1 &             22.2 \\
 17 &  92.0430 & -6.4123 &  177 &         13.2 &          8.5 &   0.1 $^{+0.01}_{-0.01}$ &    4.1 &           0.8 &  15.0 $\pm$ 1.7 &  0.32 $\pm$ 0.03 &          10.4 &            13.7 &             21.5 \\
 18 &  91.9340 & -6.3985 &  166 &         37.6 &         29.1 &   0.28 $^{+0.15}_{-0.1}$ &  140.9 &          71.3 &  24.3 $\pm$ 0.7 &  0.59 $\pm$ 0.02 &          10.6 &            14.2 &             22.3 \\
 19 &  91.8941 & -6.4071 &  128 &         14.2 &         11.3 &   0.11 $^{+0.0}_{-0.02}$ &    7.8 &           1.5 &  20.4 $\pm$ 1.2 &  0.45 $\pm$ 0.03 &          10.5 &            13.9 &             21.9 \\
 20 &  92.1770 & -6.3956 &  157 &         38.7 &         14.8 &  0.19 $^{+0.25}_{-0.12}$ &    9.4 &           4.8 &  14.4 $\pm$ 3.4 &  0.34 $\pm$ 0.06 &           8.6 &            13.7 &             21.4 \\
 21 &  91.9629 & -6.3802 &  161 &         27.5 &         11.1 &  0.15 $^{+0.11}_{-0.05}$ &   27.7 &           9.3 &  23.0 $\pm$ 0.9 &  0.53 $\pm$ 0.02 &          10.7 &            14.0 &             22.2 \\
 22 &  91.9509 & -6.3704 &   45 &          9.5 &          7.0 &    0.07 $^{+0.0}_{-0.0}$ &    9.7 &           1.4 &  33.5 $\pm$ 1.5 &  0.69 $\pm$ 0.03 &           9.5 &            13.9 &             22.2 \\
 23 &  91.9328 & -6.3508 &  137 &         43.1 &         19.7 &   0.22 $^{+0.2}_{-0.16}$ &   59.6 &          29.2 &  19.2 $\pm$ 0.9 &  0.35 $\pm$ 0.02 &           9.5 &            14.0 &             22.1 \\
 24 &  91.8911 & -6.3581 &  152 &         10.2 &          9.3 &  0.08 $^{+0.01}_{-0.01}$ &    3.5 &           0.2 &  18.1 $\pm$ 2.3 &  0.26 $\pm$ 0.04 &           9.8 &            13.3 &             21.8 \\
 25 &  91.9795 & -6.3531 &  182 &         10.7 &          7.8 &    0.08 $^{+0.0}_{-0.0}$ &    3.2 &           0.9 &  22.2 $\pm$ 2.3 &  0.38 $\pm$ 0.04 &          10.4 &            13.5 &             21.8 \\
 26 &  91.9846 & -6.3364 &  159 &         15.9 &         12.7 &  0.11 $^{+0.04}_{-0.02}$ &    4.1 &           0.9 &  21.8 $\pm$ 3.5 &   0.3 $\pm$ 0.05 &          10.0 &            13.6 &             21.7 \\
 27 &  91.9182 & -6.3277 &   57 &         13.8 &          9.2 &  0.09 $^{+0.04}_{-0.02}$ &    3.0 &           0.4 &  13.4 $\pm$ 3.3 &  0.18 $\pm$ 0.04 &           9.4 &            14.0 &             21.8 \\
 28 &  92.0024 & -6.3232 &   82 &         12.1 &         10.8 &   0.1 $^{+0.02}_{-0.01}$ &    4.7 &           0.8 &  17.6 $\pm$ 2.5 &  0.32 $\pm$ 0.05 &           9.3 &            13.4 &             21.6 \\
 29 &  91.9747 & -6.3154 &  205 &         32.2 &         10.0 &  0.14 $^{+0.14}_{-0.09}$ &    5.0 &           1.2 &  21.8 $\pm$ 3.7 &  0.29 $\pm$ 0.06 &          10.3 &            13.4 &             21.6 \\
 30 &  91.9362 & -6.3123 &  119 &         25.2 &         14.0 &  0.14 $^{+0.08}_{-0.07}$ &    8.7 &           2.4 &  18.6 $\pm$ 3.5 &  0.39 $\pm$ 0.07 &           9.8 &            13.8 &             21.7 \\
 31 &  92.0036 & -6.3061 &  118 &         15.4 &         11.6 &  0.12 $^{+0.03}_{-0.02}$ &    3.8 &           1.1 &  18.3 $\pm$ 3.2 &  0.39 $\pm$ 0.07 &           9.5 &            13.6 &             21.5 \\
 32 &  92.0313 & -6.3038 &  157 &         15.2 &         12.3 &  0.13 $^{+0.03}_{-0.02}$ &    4.6 &           0.9 &  16.2 $\pm$ 2.2 &  0.19 $\pm$ 0.03 &           8.9 &            13.8 &             21.4 \\
 33 &  91.9090 & -6.2999 &  124 &         18.6 &         15.5 &  0.14 $^{+0.05}_{-0.07}$ &    5.5 &           1.4 &  15.1 $\pm$ 3.0 &  0.24 $\pm$ 0.05 &           9.6 &            13.9 &             21.5 \\
 34 &  92.1094 & -6.2932 &  174 &         14.0 &         10.5 &   0.1 $^{+0.03}_{-0.03}$ &    1.5 &           0.4 &  13.1 $\pm$ 3.3 &  0.32 $\pm$ 0.07 &           8.9 &            13.8 &             21.1 \\
 35 &  91.9046 & -6.2797 &  124 &         13.8 &          8.2 &  0.09 $^{+0.02}_{-0.02}$ &    2.2 &           0.4 &  13.4 $\pm$ 4.3 &  0.21 $\pm$ 0.05 &          10.1 &            14.0 &             21.5 \\
 36 &  91.9407 & -6.2652 &  147 &         13.9 &          8.9 &  0.08 $^{+0.06}_{-0.04}$ &    1.9 &           0.5 &  16.5 $\pm$ 3.7 &  0.45 $\pm$ 0.08 &          10.8 &            14.4 &             21.4 \\
 37 &  91.9304 & -6.2614 &  120 &          9.1 &          7.7 &    0.08 $^{+0.0}_{-0.0}$ &    1.4 &           0.2 &  18.7 $\pm$ 3.6 &   0.2 $\pm$ 0.04 &          10.4 &            13.7 &             21.4 \\
 38 &  91.9324 & -6.1787 &  187 &         24.8 &         19.5 &  0.22 $^{+0.04}_{-0.06}$ &   18.2 &           9.6 &  13.1 $\pm$ 1.6 &  0.22 $\pm$ 0.02 &          10.4 &            13.8 &             21.5 \\
 39 &  91.8388 & -6.1803 &   65 &         13.6 &          8.9 &   0.1 $^{+0.01}_{-0.01}$ &    2.0 &           0.3 &  11.7 $\pm$ 2.8 &  0.13 $\pm$ 0.02 &          10.9 &            13.6 &             21.3 \\
 40 &  91.8578 & -6.1582 &  132 &         32.3 &         13.6 &  0.21 $^{+0.12}_{-0.07}$ &   11.4 &           4.3 &  12.3 $\pm$ 1.8 &  0.15 $\pm$ 0.02 &          11.0 &            13.8 &             21.4 \\
 41 &  91.8922 & -6.1452 &  191 &         18.6 &         13.9 &  0.15 $^{+0.08}_{-0.04}$ &    5.2 &           1.4 &  12.9 $\pm$ 2.9 &  0.13 $\pm$ 0.02 &          10.7 &            13.7 &             21.4 \\
\bottomrule
\end{tabular}


==> MonR2_leaf_stats_virial.tex <==
\begin{tabular}{rrrrrrrrllrr}
\toprule
 ID &  $\alpha_{vir}$ &  $M_{vir}$ &  $\sigma_{nt}$ & log$|\Omega_G|$ & log$\Omega_K$ & log$|\Omega_{Pw}|$ &  log$|\Omega_{Pt}|$ & on-filament & hub & $N_{proto}$ & Bad N(H$_2$) Pixels \\& & (M$_\odot$) & (km s$^{-1}$) & (erg) & (erg) & (erg) & (erg) & & & \\\midrule
  0 &   1.62 &              10.4 &      0.17 &  43.1 &     43.1 &     43.6 &         NaN &         True &  False &           0 &         0 \\
  1 &   7.28 &              26.0 &      0.41 &  42.7 &     43.4 &     43.3 &         NaN &         True &  False &           0 &         0 \\
  2 &   1.46 &              13.0 &      0.17 &  43.4 &     43.3 &     43.8 &         NaN &        False &  False &           0 &         0 \\
  3 &   6.35 &              60.8 &      0.52 &  43.4 &     44.0 &     44.0 &         NaN &        False &  False &           0 &         0 \\
  4 &   0.77 &              20.6 &      0.19 &  44.1 &     43.8 &     44.5 &         NaN &         True &  False &           3 &         0 \\
  5 &   1.52 &               8.7 &      0.14 &  43.1 &     43.1 &     43.6 &         NaN &        False &  False &           0 &         0 \\
  6 &   1.57 &              21.9 &      0.35 &  43.9 &     43.9 &     43.8 &         NaN &         True &  False &           2 &         0 \\
  7 &   5.44 &              15.2 &      0.32 &  42.6 &     43.1 &     43.1 &         NaN &         True &  False &           0 &         0 \\
  8 &   1.91 &              24.5 &      0.33 &  43.7 &     43.8 &     43.9 &         NaN &         True &  False &           1 &         0 \\
  9 &   3.86 &              16.0 &      0.27 &  42.8 &     43.2 &     43.3 &         NaN &         True &  False &           0 &         0 \\
 10 &   5.32 &              15.2 &      0.28 &  42.5 &     43.1 &     43.1 &         NaN &         True &  False &           0 &         0 \\
 11 &    NaN &               4.9 &      0.09 &   NaN &      NaN &      NaN &         NaN &        False &  False &           0 &         0 \\
 12 &   2.65 &               8.4 &      0.14 &  42.6 &     42.8 &     43.2 &         NaN &         True &  False &           0 &         0 \\
 13 &   1.67 &              12.8 &      0.21 &  43.3 &     43.3 &     43.6 &         NaN &         True &  False &           1 &         0 \\
 14 &   4.58 &               8.8 &      0.23 &  42.3 &     42.8 &     42.9 &         NaN &         True &  False &           0 &         0 \\
 15 &   4.42 &              12.0 &      0.33 &  42.7 &     43.1 &     42.8 &         NaN &         True &  False &           0 &         0 \\
 16 &   1.44 &              12.6 &      0.33 &  43.7 &     43.7 &     43.4 &         NaN &         True &  False &           1 &         0 \\
 17 &   3.19 &              13.2 &      0.31 &  43.0 &     43.3 &     43.1 &         NaN &         True &  False &           1 &         0 \\
 18 &   0.77 &             108.1 &      0.58 &  45.6 &     45.2 &     45.2 &         NaN &        False &   True &           0 &         0 \\
 19 &   3.65 &              28.6 &      0.44 &  43.4 &     43.8 &     43.6 &         NaN &         True &  False &           0 &         0 \\
 20 &   2.86 &              27.0 &      0.33 &  43.4 &     43.6 &     43.7 &         NaN &         True &  False &           1 &         0 \\
 21 &   1.81 &              50.1 &      0.52 &  44.4 &     44.5 &     44.3 &         NaN &         True &  False &           0 &         0 \\
 22 &   4.01 &              38.8 &      0.68 &  43.8 &     44.2 &     43.4 &         NaN &         True &  False &           0 &         0 \\
 23 &   0.60 &              35.7 &      0.33 &  44.9 &     44.5 &     44.7 &         NaN &         True &  False &           4 &         0 \\
 24 &   2.74 &               9.5 &      0.24 &  42.9 &     43.1 &     43.2 &         NaN &         True &  False &           0 &         0 \\
 25 &   5.09 &              16.2 &      0.37 &  42.8 &     43.3 &     43.1 &         NaN &        False &  False &           0 &         0 \\
 26 &   4.10 &              16.6 &      0.29 &  42.9 &     43.3 &     43.4 &         NaN &        False &  False &           0 &         0 \\
 27 &   2.12 &               6.4 &      0.16 &  42.7 &     42.8 &     43.3 &         NaN &        False &  False &           1 &         0 \\
 28 &   3.16 &              14.8 &      0.30 &  43.0 &     43.3 &     43.2 &         NaN &         True &  False &           0 &         0 \\
 29 &   4.00 &              19.8 &      0.27 &  43.0 &     43.4 &     43.6 &         NaN &        False &  False &           0 &         0 \\
 30 &   3.16 &              27.6 &      0.38 &  43.4 &     43.7 &     43.7 &         NaN &         True &  False &           2 &         0 \\
 31 &   6.11 &              23.4 &      0.38 &  42.8 &     43.4 &     43.3 &         NaN &         True &  False &           0 &         0 \\
 32 &   2.27 &              10.3 &      0.16 &  42.9 &     43.1 &     43.4 &         NaN &         True &  False &           0 &         0 \\
 33 &   2.38 &              13.0 &      0.22 &  43.1 &     43.2 &     43.5 &         NaN &        False &  False &           0 &         0 \\
 34 &   8.53 &              12.5 &      0.30 &  42.1 &     42.8 &     42.7 &         NaN &        False &  False &           0 &         0 \\
 35 &   3.14 &               6.9 &      0.19 &  42.4 &     42.7 &     42.9 &         NaN &        False &  False &           0 &         0 \\
 36 &  10.03 &              19.0 &      0.44 &  42.4 &     43.2 &     42.7 &         NaN &         True &  False &           0 &         0 \\
 37 &   4.76 &               6.7 &      0.17 &  42.1 &     42.6 &     42.6 &         NaN &         True &  False &           0 &         0 \\
 38 &   0.98 &              17.9 &      0.20 &  43.9 &     43.7 &     44.1 &         NaN &         True &  False &           2 &         0 \\
 39 &   2.40 &               4.9 &      0.10 &  42.3 &     42.5 &     42.9 &         NaN &         True &  False &           0 &         0 \\
 40 &   1.04 &              11.9 &      0.13 &  43.5 &     43.3 &     43.9 &         NaN &         True &  False &           0 &         0 \\
 41 &   1.51 &               7.8 &      0.10 &  43.0 &     42.9 &     43.5 &         NaN &         True &  False &           0 &         0 \\
\bottomrule
\end{tabular}


==> NGC2264_leaf_stats.tex <==
\begin{tabular}{rrrrrrlrrllrrr}
\toprule
ID & RA & decl. & PA & $\sigma_{major}$ & $\sigma_{minor}$ &  $R_{eff}$ &  $M_{obs}$ &  $M_{clip}$ &  $T_K$ &  $\sigma_{NH_3}$ &  $V_{LSR, NH_3}$ &  log($N_{para-NH_3}$) &  log($N_{H_2}$) \\& (deg) & (deg) & (deg) & ($\arcsec$) & ($\arcsec$) & (pc) & (M$_\odot$) & (M$_\odot$) & (K) & (km s$^{-1}$) & (km s$^{-1}$) & (cm$^{-2}$) & (cm$^{-2}$) \\\midrule
  0 &  100.5318 &  9.1710 &   77 &         39.8 &         19.8 &  0.26 $^{+0.28}_{-0.11}$ &   30.6 &          13.1 &  11.0 $\pm$ 2.3 &  0.21 $\pm$ 0.03 &           7.8 &            14.0 &             21.6 \\
  1 &  100.5425 &  9.2038 &  190 &         17.8 &         13.8 &  0.13 $^{+0.04}_{-0.06}$ &    6.5 &           2.7 &   9.1 $\pm$ 4.1 &  0.19 $\pm$ 0.04 &           7.4 &            14.0 &             21.5 \\
  2 &  100.2946 &  9.3462 &  102 &         33.2 &         13.2 &    0.2 $^{+0.3}_{-0.08}$ &   14.4 &           4.1 &   9.7 $\pm$ 1.8 &  0.14 $\pm$ 0.01 &           4.4 &            14.0 &             21.6 \\
  3 &  100.3926 &  9.3385 &  118 &         10.5 &          7.9 &  0.08 $^{+0.02}_{-0.01}$ &    2.0 &           0.1 &  13.6 $\pm$ 3.0 &  0.47 $\pm$ 0.07 &           8.0 &            13.9 &             21.5 \\
  4 &  100.3810 &  9.3465 &  204 &         13.5 &          8.6 &  0.08 $^{+0.03}_{-0.06}$ &    2.4 &           0.2 &  13.9 $\pm$ 2.9 &  0.49 $\pm$ 0.07 &           8.2 &            13.6 &             21.6 \\
  5 &  100.3290 &  9.3533 &   94 &         13.3 &         11.2 &  0.11 $^{+0.03}_{-0.01}$ &    5.9 &           2.0 &  10.5 $\pm$ 2.7 &  0.13 $\pm$ 0.02 &           4.8 &            13.9 &             21.7 \\
  6 &  100.3637 &  9.3779 &   71 &         27.8 &         13.1 &  0.17 $^{+0.11}_{-0.05}$ &   20.7 &           6.9 &  13.6 $\pm$ 1.2 &  0.43 $\pm$ 0.03 &           8.1 &            13.9 &             21.7 \\
  7 &  100.3292 &  9.3721 &   88 &         13.2 &          8.9 &  0.09 $^{+0.03}_{-0.03}$ &    4.7 &           0.4 &  13.7 $\pm$ 3.0 &  0.38 $\pm$ 0.06 &           4.9 &            13.9 &             21.8 \\
  8 &  100.3474 &  9.3984 &  108 &         25.7 &         10.3 &   0.11 $^{+0.1}_{-0.08}$ &    7.6 &           2.3 &  14.3 $\pm$ 1.7 &  0.48 $\pm$ 0.04 &           7.7 &            13.8 &             21.8 \\
  9 &  100.3101 &  9.4110 &   60 &         42.2 &         17.0 &  0.23 $^{+0.19}_{-0.12}$ &   46.7 &          18.3 &  18.4 $\pm$ 1.8 &  0.58 $\pm$ 0.05 &           5.6 &            13.7 &             21.9 \\
 10 &  100.3362 &  9.4000 &  119 &         13.1 &          8.0 &  0.08 $^{+0.02}_{-0.06}$ &    4.5 &           0.6 &  17.7 $\pm$ 2.1 &  0.41 $\pm$ 0.05 &           7.6 &            13.5 &             21.8 \\
 11 &  100.2635 &  9.4329 &   62 &         15.6 &         13.7 &  0.13 $^{+0.05}_{-0.02}$ &    6.2 &           1.2 &  11.0 $\pm$ 3.3 &  0.35 $\pm$ 0.06 &           4.9 &            13.9 &             21.8 \\
 12 &  100.4601 &  9.4352 &  186 &         21.8 &         18.9 &  0.15 $^{+0.08}_{-0.09}$ &    4.2 &           1.2 &  14.3 $\pm$ 3.8 &  0.22 $\pm$ 0.05 &           7.5 &            13.7 &             21.2 \\
 13 &  100.3157 &  9.4484 &   97 &         24.2 &          9.5 &  0.13 $^{+0.08}_{-0.04}$ &   16.4 &           5.9 &  15.6 $\pm$ 0.7 &  0.38 $\pm$ 0.02 &           7.7 &            14.0 &             22.1 \\
 14 &  100.2811 &  9.4432 &   50 &         16.7 &          7.0 &  0.09 $^{+0.05}_{-0.02}$ &    5.7 &           0.7 &  16.5 $\pm$ 1.6 &  0.56 $\pm$ 0.05 &           6.2 &            14.0 &             22.0 \\
 15 &  100.3598 &  9.4732 &  108 &         38.9 &         20.5 &  0.19 $^{+0.18}_{-0.13}$ &   12.2 &           6.7 &  12.3 $\pm$ 3.3 &  0.43 $\pm$ 0.08 &           6.7 &            14.1 &             21.8 \\
 16 &  100.2989 &  9.4913 &  215 &         47.2 &         37.4 &  0.43 $^{+0.09}_{-0.08}$ &  492.7 &         322.3 &  18.8 $\pm$ 0.4 &  0.76 $\pm$ 0.01 &           7.3 &            14.5 &             22.2 \\
 17 &  100.2337 &  9.4803 &   48 &         12.4 &          6.7 &  0.08 $^{+0.02}_{-0.03}$ &    1.3 &           0.1 &  10.0 $\pm$ 5.0 &   1.0 $\pm$ 0.22 &           5.6 &            14.6 &             21.8 \\
 18 &  100.2793 &  9.5296 &  185 &         14.4 &         12.5 &  0.11 $^{+0.04}_{-0.02}$ &   11.5 &           0.8 &  15.3 $\pm$ 0.9 &  0.72 $\pm$ 0.03 &           6.5 &            14.2 &             22.2 \\
 19 &  100.1623 &  9.5459 &   75 &         27.6 &         11.9 &  0.16 $^{+0.08}_{-0.05}$ &   10.7 &           3.6 &  14.4 $\pm$ 3.3 &  0.53 $\pm$ 0.08 &           5.4 &            13.8 &             21.7 \\
 20 &  100.2798 &  9.5593 &   49 &         31.1 &         12.7 &  0.17 $^{+0.13}_{-0.07}$ &   76.8 &          28.3 &  15.7 $\pm$ 0.3 &  0.51 $\pm$ 0.01 &           6.1 &            14.6 &             22.3 \\
 21 &  100.2112 &  9.5783 &  121 &         21.0 &         20.7 &  0.19 $^{+0.02}_{-0.03}$ &   54.3 &          21.3 &  12.3 $\pm$ 0.6 &  0.47 $\pm$ 0.01 &           5.1 &            14.4 &             22.1 \\
 22 &  100.2646 &  9.5847 &  212 &         28.8 &         12.3 &  0.16 $^{+0.07}_{-0.08}$ &   84.1 &          24.7 &  16.0 $\pm$ 0.4 &  0.91 $\pm$ 0.02 &           5.3 &            14.6 &             22.3 \\
 23 &  100.2363 &  9.5936 &   51 &         15.9 &         11.5 &  0.12 $^{+0.02}_{-0.01}$ &   28.3 &           2.2 &  14.5 $\pm$ 0.3 &  0.49 $\pm$ 0.01 &           5.6 &            14.6 &             22.2 \\
 24 &  100.2841 &  9.5950 &  191 &         24.0 &         10.0 &   0.13 $^{+0.1}_{-0.05}$ &   45.0 &          10.8 &  16.6 $\pm$ 0.4 &  0.72 $\pm$ 0.02 &           5.1 &            14.5 &             22.2 \\
 25 &  100.1934 &  9.6285 &   78 &          9.8 &          7.8 &  0.07 $^{+0.01}_{-0.01}$ &    1.7 &           0.1 &  15.0 $\pm$ 3.8 &  0.32 $\pm$ 0.08 &           5.5 &            14.2 &             21.8 \\
 26 &  100.2361 &  9.6375 &   86 &         18.2 &         15.6 &  0.15 $^{+0.04}_{-0.02}$ &    9.8 &           3.5 &  13.3 $\pm$ 2.8 &  0.44 $\pm$ 0.06 &           5.5 &            13.7 &             21.9 \\
 27 &  100.3165 &  9.6474 &   66 &         36.0 &         14.8 &   0.21 $^{+0.27}_{-0.1}$ &   19.1 &           5.7 &  11.4 $\pm$ 2.0 &  0.24 $\pm$ 0.03 &           4.7 &            13.8 &             21.7 \\
 28 &  100.2896 &  9.6495 &  134 &         11.9 &          5.8 &  0.07 $^{+0.04}_{-0.01}$ &    2.0 &           0.1 &  15.7 $\pm$ 4.4 &  0.79 $\pm$ 0.17 &           5.5 &            14.1 &             21.8 \\
 29 &  100.3032 &  9.6809 &  188 &         14.5 &          6.4 &  0.08 $^{+0.04}_{-0.04}$ &    2.5 &           0.3 &  14.7 $\pm$ 3.8 &   0.57 $\pm$ 0.1 &           5.2 &            14.0 &             21.7 \\
 30 &  100.3173 &  9.6953 &   49 &         20.4 &         13.9 &  0.14 $^{+0.05}_{-0.04}$ &   10.3 &           2.2 &  12.8 $\pm$ 3.0 &   0.67 $\pm$ 0.1 &           5.8 &            14.0 &             21.6 \\
 31 &  100.3032 &  9.6913 &  198 &         11.5 &          7.5 &  0.08 $^{+0.01}_{-0.02}$ &    3.0 &           0.1 &   9.8 $\pm$ 4.3 &  0.31 $\pm$ 0.06 &           5.1 &            13.8 &             21.6 \\
 32 &  100.2961 &  9.7281 &   72 &         32.5 &         15.4 &  0.13 $^{+0.15}_{-0.09}$ &    7.3 &           1.5 &  12.2 $\pm$ 3.9 &  0.33 $\pm$ 0.07 &           5.0 &            13.8 &             21.6 \\
 33 &  100.3050 &  9.7449 &   93 &         22.1 &         10.5 &  0.12 $^{+0.06}_{-0.07}$ &    5.3 &           0.4 &  11.5 $\pm$ 4.4 &   0.48 $\pm$ 0.1 &           4.8 &            14.0 &             21.6 \\
 34 &  100.3208 &  9.7473 &  205 &         19.9 &          3.8 &  0.07 $^{+0.06}_{-0.03}$ &    1.6 &           0.3 &  12.2 $\pm$ 3.2 &  1.13 $\pm$ 0.17 &           5.6 &            14.5 &             21.5 \\
 35 &  100.1089 &  9.8339 &  181 &         38.6 &         19.3 &    0.19 $^{+0.2}_{-0.1}$ &    9.0 &           2.1 &  19.7 $\pm$ 3.7 &  0.35 $\pm$ 0.07 &          10.4 &            13.5 &             21.3 \\
 36 &  100.0504 &  9.8443 &   53 &         24.2 &          9.6 &    0.11 $^{+0.1}_{-0.1}$ &    2.3 &           0.5 &  16.1 $\pm$ 4.4 &  0.31 $\pm$ 0.08 &          10.1 &            13.7 &             21.2 \\
 37 &  100.1214 &  9.9082 &  100 &         18.3 &         10.1 &  0.11 $^{+0.06}_{-0.05}$ &    4.5 &           1.2 &  20.3 $\pm$ 3.1 &  0.36 $\pm$ 0.06 &          10.0 &            13.9 &             21.4 \\
 38 &  100.1130 &  9.9262 &  195 &         21.3 &          7.0 &   0.1 $^{+0.09}_{-0.03}$ &    2.1 &           0.3 &  18.0 $\pm$ 5.0 &  0.51 $\pm$ 0.13 &          10.0 &            14.0 &             21.3 \\
 39 &  100.2962 &  9.9336 &  211 &         15.2 &         14.2 &  0.15 $^{+0.01}_{-0.01}$ &   10.1 &           3.7 &  13.1 $\pm$ 1.5 &  0.28 $\pm$ 0.03 &           4.5 &            14.1 &             21.4 \\
 40 &  100.2746 &  9.9494 &  216 &         22.7 &         15.2 &  0.17 $^{+0.05}_{-0.04}$ &   11.0 &           3.0 &  10.3 $\pm$ 2.8 &  0.16 $\pm$ 0.02 &           4.7 &            13.9 &             21.4 \\
 41 &  100.0927 &  9.9416 &  158 &         16.9 &          6.1 &  0.09 $^{+0.05}_{-0.03}$ &    1.9 &           0.2 &  16.0 $\pm$ 4.3 &  0.88 $\pm$ 0.18 &           9.8 &            13.9 &             21.3 \\
\bottomrule
\end{tabular}


==> NGC2264_leaf_stats_virial.tex <==
\begin{tabular}{rrrrrrrrllrr}
\toprule
 ID &  $\alpha_{vir}$ &  $M_{vir}$ &  $\sigma_{nt}$ & log$|\Omega_G|$ & log$\Omega_K$ & log$|\Omega_{Pw}|$ &  log$|\Omega_{Pt}|$ & on-filament & hub & $N_{proto}$ & Bad N(H$_2$) Pixels \\& & (M$_\odot$) & (km s$^{-1}$) & (erg) & (erg) & (erg) & (erg) & & & \\\midrule
  0 &   0.60 &              18.5 &      0.20 &  44.3 &     43.9 &     44.4 &         NaN &         True &  False &           1 &         0 \\
  1 &   1.21 &               7.9 &      0.18 &  43.2 &     43.1 &     43.5 &         NaN &         True &  False &           1 &         0 \\
  2 &   0.63 &               9.1 &      0.12 &  43.7 &     43.3 &     44.1 &         NaN &         True &  False &           0 &         0 \\
  3 &   9.30 &              18.3 &      0.46 &  42.4 &     43.2 &     42.8 &         NaN &         True &  False &           0 &         0 \\
  4 &   8.44 &              20.3 &      0.48 &  42.6 &     43.3 &     42.9 &         NaN &         True &  False &           0 &         0 \\
  5 &   0.91 &               5.3 &      0.11 &  43.2 &     42.9 &     43.5 &         NaN &         True &  False &           0 &         0 \\
  6 &   1.80 &              37.2 &      0.43 &  44.1 &     44.2 &     44.1 &         NaN &         True &  False &           0 &         0 \\
  7 &   3.40 &              16.0 &      0.37 &  43.1 &     43.4 &     43.3 &         NaN &         True &  False &           0 &         0 \\
  8 &   3.74 &              28.2 &      0.47 &  43.4 &     43.8 &     43.6 &         NaN &         True &  False &           0 &         0 \\
  9 &   1.76 &              82.3 &      0.57 &  44.7 &     44.7 &     44.6 &         NaN &         True &  False &           0 &         0 \\
 10 &   3.72 &              16.8 &      0.40 &  43.1 &     43.5 &     43.2 &         NaN &         True &  False &           0 &         0 \\
 11 &   3.06 &              18.9 &      0.34 &  43.2 &     43.5 &     43.8 &         NaN &         True &  False &           0 &         0 \\
 12 &   3.19 &              13.5 &      0.21 &  42.8 &     43.1 &     43.5 &         NaN &        False &  False &           0 &         0 \\
 13 &   1.36 &              22.3 &      0.37 &  44.0 &     44.0 &     44.1 &         NaN &        False &  False &           1 &         0 \\
 14 &   5.64 &              32.1 &      0.55 &  43.2 &     43.8 &     43.6 &         NaN &        False &  False &           1 &         0 \\
 15 &   3.23 &              39.2 &      0.42 &  43.6 &     43.9 &     44.3 &         NaN &        False &  False &           0 &         0 \\
 16 &   0.51 &             253.6 &      0.76 &  46.5 &     46.0 &     45.8 &         NaN &        False &   True &           9 &         0 \\
 17 &  55.04 &              72.0 &      1.00 &  42.1 &     43.6 &     43.1 &         NaN &        False &  False &           0 &         0 \\
 18 &   4.97 &              57.3 &      0.71 &  43.8 &     44.3 &     44.0 &         NaN &        False &  False &           0 &         0 \\
 19 &   4.50 &              48.4 &      0.52 &  43.6 &     44.0 &     43.9 &         NaN &        False &  False &           0 &         0 \\
 20 &   0.65 &              49.8 &      0.51 &  45.2 &     44.9 &     44.6 &         NaN &         True &  False &           3 &         0 \\
 21 &   0.82 &              44.6 &      0.46 &  44.9 &     44.6 &     44.6 &         NaN &         True &  False &           6 &         0 \\
 22 &   1.57 &             132.0 &      0.90 &  45.4 &     45.3 &     44.6 &         NaN &         True &  False &           4 &         0 \\
 23 &   1.14 &              32.3 &      0.49 &  44.5 &     44.4 &     44.1 &         NaN &         True &  False &           0 &         0 \\
 24 &   1.54 &              69.4 &      0.72 &  44.9 &     44.9 &     44.2 &         NaN &         True &  False &           5 &         0 \\
 25 &   5.93 &               9.8 &      0.31 &  42.3 &     42.9 &     43.0 &         NaN &        False &  False &           0 &         0 \\
 26 &   3.38 &              33.1 &      0.43 &  43.5 &     43.8 &     44.1 &         NaN &        False &  False &           0 &         0 \\
 27 &   0.99 &              18.8 &      0.23 &  43.9 &     43.7 &     44.4 &         NaN &         True &  False &           0 &         0 \\
 28 &  22.14 &              45.0 &      0.79 &  42.5 &     43.6 &     43.0 &         NaN &         True &  False &           0 &         0 \\
 29 &  10.82 &              27.3 &      0.57 &  42.6 &     43.5 &     43.0 &         NaN &         True &  False &           0 &         0 \\
 30 &   6.32 &              65.1 &      0.67 &  43.6 &     44.2 &     43.7 &         NaN &         True &  False &           0 &         0 \\
 31 &   3.04 &               9.1 &      0.30 &  42.8 &     43.1 &     43.0 &         NaN &         True &  False &           0 &         0 \\
 32 &   2.47 &              17.9 &      0.32 &  43.3 &     43.5 &     43.6 &         NaN &         True &  False &           0 &         0 \\
 33 &   5.74 &              30.7 &      0.47 &  43.1 &     43.6 &     43.5 &         NaN &         True &  False &           0 &         0 \\
 34 &  53.20 &              87.4 &      1.12 &  42.3 &     43.8 &     42.7 &         NaN &        False &  False &           0 &         0 \\
 35 &   3.55 &              31.9 &      0.33 &  43.3 &     43.7 &     43.8 &         NaN &         True &  False &           1 &         0 \\
 36 &   6.65 &              15.0 &      0.30 &  42.4 &     43.0 &     43.0 &         NaN &         True &  False &           0 &         0 \\
 37 &   4.60 &              20.6 &      0.35 &  43.0 &     43.4 &     43.2 &         NaN &         True &  False &           0 &         0 \\
 38 &  14.00 &              28.9 &      0.50 &  42.3 &     43.3 &     43.0 &         NaN &         True &  False &           0 &         0 \\
 39 &   1.63 &              16.4 &      0.27 &  43.5 &     43.5 &     43.6 &         NaN &        False &  False &           2 &         0 \\
 40 &   0.80 &               8.8 &      0.14 &  43.6 &     43.3 &     43.8 &         NaN &        False &  False &           0 &         0 \\
 41 &  34.26 &              66.4 &      0.88 &  42.3 &     43.7 &     42.7 &         NaN &         True &  False &           1 &         0 \\
\bottomrule
\end{tabular}


==> NGC7538_leaf_stats.tex <==
\begin{tabular}{rrrrrrlrrllrrr}
\toprule
ID & RA & decl. & PA & $\sigma_{major}$ & $\sigma_{minor}$ &  $R_{eff}$ &  $M_{obs}$ &  $M_{clip}$ &  $T_K$ &  $\sigma_{NH_3}$ &  $V_{LSR, NH_3}$ &  log($N_{para-NH_3}$) &  log($N_{H_2}$) \\& (deg) & (deg) & (deg) & ($\arcsec$) & ($\arcsec$) & (pc) & (M$_\odot$) & (M$_\odot$) & (K) & (km s$^{-1}$) & (km s$^{-1}$) & (cm$^{-2}$) & (cm$^{-2}$) \\\midrule
  0 &  348.8620 &  61.1181 &  139 &         32.1 &         20.6 &  0.69 $^{+0.39}_{-0.33}$ &   285.6 &         193.5 &  23.4 $\pm$ 2.2 &  0.91 $\pm$ 0.07 &         -56.7 &            13.9 &             21.5 \\
  1 &  348.9680 &  61.1322 &  145 &         14.0 &         10.1 &   0.3 $^{+0.06}_{-0.09}$ &    21.7 &           3.6 &  14.3 $\pm$ 3.4 &  0.46 $\pm$ 0.09 &         -55.7 &            13.9 &             21.4 \\
  2 &  348.8169 &  61.1278 &  191 &         14.8 &          7.8 &  0.27 $^{+0.08}_{-0.18}$ &    22.2 &           4.9 &  12.7 $\pm$ 3.0 &  0.45 $\pm$ 0.08 &         -56.0 &            14.3 &             21.5 \\
  3 &  348.9377 &  61.1448 &  224 &         15.1 &         12.7 &  0.38 $^{+0.11}_{-0.04}$ &    43.6 &          17.3 &  18.0 $\pm$ 2.5 &  0.36 $\pm$ 0.05 &         -54.8 &            13.8 &             21.4 \\
  4 &  348.8210 &  61.1466 &  203 &         14.8 &          7.2 &  0.26 $^{+0.14}_{-0.23}$ &    17.4 &           2.6 &  11.9 $\pm$ 3.7 &  0.59 $\pm$ 0.12 &         -55.8 &            14.4 &             21.5 \\
  5 &  349.2294 &  61.2020 &  152 &         20.9 &          7.5 &  0.27 $^{+0.24}_{-0.21}$ &    20.9 &           2.1 &  15.9 $\pm$ 3.6 &   0.53 $\pm$ 0.1 &         -53.6 &            13.8 &             21.4 \\
  6 &  349.2145 &  61.2320 &   50 &         18.5 &         13.2 &  0.38 $^{+0.18}_{-0.14}$ &    40.2 &           6.7 &  16.2 $\pm$ 3.7 &  0.62 $\pm$ 0.11 &         -52.8 &            14.0 &             21.5 \\
  7 &  349.1750 &  61.2647 &   60 &         36.5 &         23.3 &  0.81 $^{+0.41}_{-0.46}$ &   280.3 &         120.9 &  16.8 $\pm$ 2.3 &  0.54 $\pm$ 0.06 &         -52.3 &            13.5 &             21.5 \\
  8 &  348.6059 &  61.2528 &  148 &         21.4 &          8.2 &  0.33 $^{+0.25}_{-0.12}$ &    36.6 &          14.7 &  16.4 $\pm$ 3.9 &  0.39 $\pm$ 0.08 &         -56.3 &            13.8 &             21.4 \\
  9 &  349.1789 &  61.3055 &   89 &         29.1 &         19.7 &   0.5 $^{+0.29}_{-0.35}$ &    85.1 &          29.5 &  15.5 $\pm$ 3.6 &  0.92 $\pm$ 0.15 &         -53.1 &            14.0 &             21.6 \\
 10 &  349.1047 &  61.3026 &  194 &         10.7 &          7.2 &  0.22 $^{+0.06}_{-0.06}$ &    24.6 &           4.5 &  16.0 $\pm$ 1.5 &  0.88 $\pm$ 0.06 &         -53.0 &            13.6 &             21.6 \\
 11 &  349.1310 &  61.3100 &  127 &         12.8 &          6.3 &  0.23 $^{+0.06}_{-0.07}$ &    25.5 &           4.1 &  16.4 $\pm$ 1.3 &  0.82 $\pm$ 0.05 &         -53.5 &            14.1 &             21.7 \\
 12 &  348.8187 &  61.3430 &  130 &         26.4 &         11.3 &  0.43 $^{+0.32}_{-0.23}$ &   152.8 &          39.7 &  14.1 $\pm$ 2.1 &  0.59 $\pm$ 0.06 &         -50.6 &            13.7 &             21.8 \\
 13 &  348.1818 &  61.3447 &   80 &         17.8 &         14.0 &  0.45 $^{+0.11}_{-0.08}$ &   101.2 &          32.7 &  14.9 $\pm$ 2.3 &  0.74 $\pm$ 0.08 &         -55.3 &            13.9 &             21.7 \\
 14 &  349.1694 &  61.3430 &  213 &         10.8 &          9.6 &  0.22 $^{+0.04}_{-0.17}$ &    15.9 &           1.3 &  20.4 $\pm$ 3.7 &  1.03 $\pm$ 0.15 &         -53.2 &            14.3 &             21.7 \\
 15 &  348.6798 &  61.3484 &  141 &         25.6 &         13.7 &  0.45 $^{+0.24}_{-0.22}$ &    73.7 &          17.6 &  17.5 $\pm$ 3.9 &   0.4 $\pm$ 0.08 &         -49.7 &            14.0 &             21.6 \\
 16 &  348.8180 &  61.3600 &  118 &         18.8 &         10.4 &  0.32 $^{+0.28}_{-0.18}$ &    85.0 &          17.6 &  13.5 $\pm$ 2.4 &  1.46 $\pm$ 0.15 &         -49.3 &            14.0 &             21.8 \\
 17 &  349.1407 &  61.3587 &  167 &         12.7 &          9.1 &  0.24 $^{+0.16}_{-0.09}$ &    36.7 &           7.4 &  19.8 $\pm$ 1.3 &  1.39 $\pm$ 0.07 &         -53.6 &            13.8 &             21.8 \\
 18 &  349.0876 &  61.3598 &  152 &         15.4 &         10.2 &  0.32 $^{+0.14}_{-0.11}$ &    79.5 &          24.4 &  14.6 $\pm$ 0.8 &  0.61 $\pm$ 0.03 &         -52.5 &            14.2 &             21.9 \\
 19 &  348.9793 &  61.3656 &  182 &         40.3 &         19.1 &    0.8 $^{+0.56}_{-0.3}$ &   571.1 &         353.7 &  17.4 $\pm$ 0.8 &  0.81 $\pm$ 0.03 &         -52.6 &            14.2 &             21.8 \\
 20 &  348.8967 &  61.3618 &  135 &         14.0 &          8.3 &   0.28 $^{+0.1}_{-0.07}$ &    51.8 &           4.8 &  14.0 $\pm$ 1.4 &  0.53 $\pm$ 0.04 &         -51.9 &            13.9 &             21.8 \\
 21 &  349.2577 &  61.3688 &   49 &         14.5 &          7.4 &  0.22 $^{+0.09}_{-0.16}$ &    15.8 &           1.0 &  15.4 $\pm$ 4.1 &   0.44 $\pm$ 0.1 &         -51.8 &            14.1 &             21.6 \\
 22 &  349.0553 &  61.3754 &  207 &         23.6 &         15.7 &  0.54 $^{+0.13}_{-0.11}$ &   424.0 &         179.6 &  15.5 $\pm$ 0.7 &   0.8 $\pm$ 0.03 &         -51.9 &            14.3 &             21.9 \\
 23 &  348.1828 &  61.3706 &  140 &         18.1 &          9.5 &   0.35 $^{+0.12}_{-0.1}$ &    77.8 &          15.0 &  14.0 $\pm$ 2.2 &  0.52 $\pm$ 0.06 &         -54.4 &            13.9 &             21.8 \\
 24 &  349.1334 &  61.3783 &  134 &         28.3 &         12.8 &  0.51 $^{+0.32}_{-0.17}$ &   260.5 &          82.8 &  15.9 $\pm$ 0.6 &  0.72 $\pm$ 0.02 &         -53.0 &            14.4 &             21.8 \\
 25 &  349.1650 &  61.3754 &   77 &         11.1 &          8.3 &  0.23 $^{+0.07}_{-0.05}$ &    51.7 &           7.0 &  18.4 $\pm$ 0.8 &  1.05 $\pm$ 0.04 &         -52.0 &            14.2 &             21.8 \\
 26 &  348.1158 &  61.3758 &  126 &         14.8 &          9.5 &  0.32 $^{+0.06}_{-0.04}$ &   127.2 &          23.3 &  15.3 $\pm$ 1.0 &  0.82 $\pm$ 0.04 &         -52.5 &            14.2 &             21.9 \\
 27 &  348.6142 &  61.3792 &   64 &         11.6 &          8.1 &  0.24 $^{+0.05}_{-0.04}$ &    26.4 &           5.8 &  13.8 $\pm$ 3.4 &  0.46 $\pm$ 0.08 &         -52.9 &            13.9 &             21.6 \\
 28 &  348.8573 &  61.3800 &  176 &         21.8 &          8.3 &  0.32 $^{+0.16}_{-0.19}$ &    47.4 &          10.6 &  14.9 $\pm$ 3.9 &  1.01 $\pm$ 0.19 &         -48.8 &            14.6 &             21.8 \\
 29 &  348.1475 &  61.3823 &  178 &         11.2 &          7.1 &  0.23 $^{+0.03}_{-0.05}$ &    65.3 &           8.8 &  15.5 $\pm$ 0.9 &  0.64 $\pm$ 0.03 &         -54.7 &            14.3 &             21.9 \\
 30 &  349.3561 &  61.3914 &  194 &         16.2 &          6.8 &  0.25 $^{+0.17}_{-0.16}$ &    19.6 &           4.0 &  14.5 $\pm$ 3.3 &  0.36 $\pm$ 0.07 &         -50.8 &            13.9 &             21.4 \\
 31 &  349.0111 &  61.4015 &   62 &         18.0 &         11.3 &    0.37 $^{+0.1}_{-0.1}$ &    72.6 &          13.9 &  14.1 $\pm$ 1.9 &  0.41 $\pm$ 0.04 &         -52.9 &            13.8 &             21.8 \\
 32 &  349.0676 &  61.4029 &   47 &         23.5 &          9.7 &  0.41 $^{+0.21}_{-0.15}$ &    69.4 &          18.7 &  14.9 $\pm$ 2.6 &  0.42 $\pm$ 0.06 &         -52.9 &            13.7 &             21.8 \\
 33 &  348.9744 &  61.4164 &   76 &         43.7 &          9.7 &  0.51 $^{+0.58}_{-0.28}$ &   163.2 &          63.2 &  14.0 $\pm$ 2.3 &  0.83 $\pm$ 0.08 &         -52.5 &            13.8 &             21.8 \\
 34 &  348.0187 &  61.4092 &  197 &         28.3 &         14.7 &  0.54 $^{+0.31}_{-0.18}$ &   160.4 &          33.0 &  15.8 $\pm$ 3.4 &   0.58 $\pm$ 0.1 &         -55.8 &            13.8 &             21.8 \\
 35 &  349.1990 &  61.4093 &  130 &          9.1 &          7.5 &   0.22 $^{+0.0}_{-0.02}$ &    25.6 &           1.9 &  12.9 $\pm$ 1.2 &  0.66 $\pm$ 0.04 &         -51.9 &            13.9 &             21.7 \\
 36 &  348.5659 &  61.4156 &  104 &         13.1 &         10.4 &  0.28 $^{+0.09}_{-0.12}$ &    33.4 &           4.2 &  10.8 $\pm$ 3.4 &  0.33 $\pm$ 0.07 &         -48.6 &            14.2 &             21.8 \\
 37 &  349.3035 &  61.4236 &   89 &         24.2 &          8.8 &  0.36 $^{+0.29}_{-0.14}$ &    37.2 &           6.6 &  16.3 $\pm$ 4.1 &  0.69 $\pm$ 0.14 &         -52.2 &            14.1 &             21.5 \\
 38 &  348.3604 &  61.4178 &  136 &         13.3 &          6.7 &  0.25 $^{+0.12}_{-0.04}$ &   156.6 &          27.7 &  20.1 $\pm$ 0.8 &  0.91 $\pm$ 0.03 &         -56.3 &            14.2 &             22.2 \\
 39 &  349.0301 &  61.4223 &  217 &         14.3 &         10.1 &  0.34 $^{+0.04}_{-0.04}$ &    45.1 &          13.8 &  17.4 $\pm$ 2.1 &  0.51 $\pm$ 0.05 &         -53.1 &            13.4 &             21.7 \\
 40 &  348.3346 &  61.4229 &  149 &         13.7 &         11.0 &  0.33 $^{+0.03}_{-0.05}$ &   279.1 &          86.9 &  17.6 $\pm$ 0.8 &  0.65 $\pm$ 0.02 &         -53.2 &            14.3 &             22.2 \\
 41 &  348.1103 &  61.4337 &  147 &         28.4 &         21.5 &  0.66 $^{+0.33}_{-0.25}$ &   275.4 &          68.2 &  15.3 $\pm$ 2.4 &   0.5 $\pm$ 0.06 &         -55.7 &            13.7 &             21.9 \\
 42 &  349.2358 &  61.4322 &  131 &         16.4 &         10.7 &   0.34 $^{+0.09}_{-0.1}$ &    46.0 &           8.5 &  15.6 $\pm$ 2.4 &  0.56 $\pm$ 0.06 &         -51.5 &            13.7 &             21.5 \\
 43 &  348.4427 &  61.4496 &  156 &         40.2 &         28.7 &  0.94 $^{+0.59}_{-0.64}$ &  3041.4 &        2208.1 &  26.9 $\pm$ 0.6 &  1.21 $\pm$ 0.02 &         -56.4 &            14.5 &             22.2 \\
 44 &  348.1571 &  61.4445 &  142 &         10.5 &          7.5 &  0.23 $^{+0.03}_{-0.01}$ &    34.6 &           2.8 &  12.0 $\pm$ 3.7 &  0.49 $\pm$ 0.09 &         -55.7 &            14.0 &             22.0 \\
 45 &  349.2767 &  61.4465 &   91 &         10.5 &          7.1 &  0.23 $^{+0.04}_{-0.01}$ &    17.1 &           2.1 &  13.5 $\pm$ 3.3 &  0.41 $\pm$ 0.07 &         -51.5 &            13.8 &             21.5 \\
 46 &  348.9484 &  61.4619 &   75 &         29.0 &         12.3 &  0.52 $^{+0.42}_{-0.22}$ &   173.1 &          94.9 &  15.4 $\pm$ 2.1 &  0.53 $\pm$ 0.06 &         -53.2 &            14.0 &             21.6 \\
 47 &  348.2268 &  61.4502 &  137 &         10.8 &          8.1 &  0.23 $^{+0.07}_{-0.06}$ &   105.2 &          13.3 &  20.1 $\pm$ 0.8 &  0.94 $\pm$ 0.03 &         -58.0 &            14.3 &             22.0 \\
 48 &  348.5225 &  61.4516 &  184 &         17.4 &          6.4 &  0.28 $^{+0.14}_{-0.09}$ &   130.5 &          28.9 &  23.0 $\pm$ 0.8 &  0.85 $\pm$ 0.03 &         -57.5 &            14.3 &             22.1 \\
 49 &  348.2411 &  61.4603 &  147 &         11.2 &          7.3 &  0.24 $^{+0.04}_{-0.05}$ &   126.9 &          13.5 &  21.2 $\pm$ 0.9 &   1.6 $\pm$ 0.05 &         -57.2 &            14.3 &             22.0 \\
 50 &  348.2969 &  61.4751 &  126 &         29.5 &         16.7 &   0.61 $^{+0.36}_{-0.3}$ &   392.6 &         196.3 &  19.2 $\pm$ 1.6 &  0.76 $\pm$ 0.05 &         -59.2 &            14.2 &             22.0 \\
 51 &  348.3725 &  61.4813 &   56 &         15.2 &         11.4 &   0.35 $^{+0.14}_{-0.1}$ &   104.8 &          33.1 &  29.3 $\pm$ 2.6 &  0.93 $\pm$ 0.07 &         -58.5 &            13.8 &             22.1 \\
 52 &  348.9557 &  61.4957 &   91 &         15.7 &         10.2 &  0.34 $^{+0.09}_{-0.06}$ &    73.3 &          16.9 &  14.0 $\pm$ 2.3 &  0.41 $\pm$ 0.05 &         -52.7 &            13.5 &             21.6 \\
 53 &  348.5167 &  61.5183 &  204 &         35.7 &         23.9 &  0.83 $^{+0.48}_{-0.33}$ &   463.8 &         280.0 &  21.1 $\pm$ 1.9 &  0.66 $\pm$ 0.05 &         -55.8 &            14.0 &             21.7 \\
 54 &  348.9695 &  61.5118 &   86 &         13.2 &          8.1 &  0.28 $^{+0.06}_{-0.06}$ &    46.7 &           8.4 &  13.7 $\pm$ 2.2 &  0.44 $\pm$ 0.05 &         -52.1 &            13.6 &             21.6 \\
 55 &  348.9835 &  61.5376 &  105 &         37.9 &         11.6 &  0.45 $^{+0.56}_{-0.38}$ &   123.1 &          30.7 &  14.8 $\pm$ 2.2 &  0.49 $\pm$ 0.06 &         -51.5 &            13.9 &             21.6 \\
 56 &  349.0687 &  61.5900 &   86 &         16.4 &         11.0 &  0.37 $^{+0.12}_{-0.04}$ &    98.4 &          35.8 &  15.6 $\pm$ 1.7 &  0.45 $\pm$ 0.04 &         -50.6 &            14.0 &             21.7 \\
 57 &  349.0372 &  61.6071 &   70 &         19.4 &         12.6 &   0.45 $^{+0.1}_{-0.07}$ &   172.9 &          66.9 &  20.4 $\pm$ 1.6 &  0.57 $\pm$ 0.04 &         -50.2 &            13.9 &             21.8 \\
 58 &  348.9210 &  61.6102 &  146 &         15.6 &         11.5 &  0.36 $^{+0.17}_{-0.09}$ &    55.2 &          12.6 &  14.2 $\pm$ 2.7 &  0.38 $\pm$ 0.06 &         -50.1 &            13.8 &             21.6 \\
 59 &  349.1925 &  61.6448 &   84 &         32.3 &         25.7 &   0.96 $^{+0.33}_{-0.2}$ &   621.0 &         366.8 &  15.6 $\pm$ 1.0 &  0.61 $\pm$ 0.03 &         -51.4 &            14.2 &             21.7 \\
 60 &  349.0568 &  61.6289 &  156 &         15.4 &         10.6 &  0.36 $^{+0.11}_{-0.05}$ &    76.8 &          30.2 &  18.8 $\pm$ 2.1 &  0.62 $\pm$ 0.06 &         -51.4 &            14.0 &             21.8 \\
 61 &  349.0081 &  61.6380 &  108 &         22.0 &         14.7 &  0.49 $^{+0.17}_{-0.08}$ &   144.0 &          50.6 &  13.1 $\pm$ 2.8 &  0.51 $\pm$ 0.06 &         -52.3 &            13.7 &             21.8 \\
 62 &  349.1215 &  61.6389 &  211 &         10.9 &          6.3 &  0.22 $^{+0.03}_{-0.03}$ &    21.3 &           3.2 &  18.1 $\pm$ 2.4 &  0.55 $\pm$ 0.06 &         -51.5 &            13.3 &             21.7 \\
 63 &  349.0942 &  61.6385 &  205 &         12.6 &          7.6 &  0.26 $^{+0.03}_{-0.05}$ &    35.3 &           6.0 &  15.3 $\pm$ 2.1 &  0.47 $\pm$ 0.05 &         -51.4 &            13.7 &             21.8 \\
 64 &  349.0450 &  61.6478 &  150 &         18.1 &         11.3 &   0.3 $^{+0.16}_{-0.17}$ &    39.2 &           7.3 &  18.6 $\pm$ 3.0 &  0.65 $\pm$ 0.09 &         -51.3 &            13.5 &             21.8 \\
 65 &  348.9884 &  61.6650 &   85 &         14.9 &          9.7 &  0.34 $^{+0.03}_{-0.02}$ &   101.5 &          33.8 &  15.9 $\pm$ 1.8 &  0.54 $\pm$ 0.05 &         -48.2 &            14.2 &             21.7 \\
 66 &  348.9845 &  61.6933 &   83 &         31.7 &         15.1 &  0.55 $^{+0.37}_{-0.23}$ &   186.4 &          67.5 &  12.7 $\pm$ 2.1 &  0.48 $\pm$ 0.05 &         -51.8 &            13.6 &             21.7 \\
 67 &  348.6898 &  61.7674 &  124 &         18.6 &          5.6 &   0.23 $^{+0.21}_{-0.1}$ &     6.2 &           0.4 &  10.0 $\pm$ 3.0 &   1.42 $\pm$ 0.3 &         -58.1 &            15.5 &             21.2 \\
 68 &  348.9339 &  61.7927 &   77 &         19.1 &         17.5 &  0.61 $^{+0.25}_{-0.08}$ &   416.1 &         247.8 &  20.8 $\pm$ 1.0 &  0.71 $\pm$ 0.03 &         -48.9 &            14.4 &             21.7 \\
 69 &  349.0691 &  61.7895 &  182 &         25.6 &          8.5 &  0.37 $^{+0.27}_{-0.25}$ &    71.6 &          22.2 &  15.2 $\pm$ 3.2 &  0.71 $\pm$ 0.11 &         -49.7 &            13.7 &             21.7 \\
 70 &  349.0520 &  61.8005 &  160 &         15.9 &          8.5 &  0.29 $^{+0.08}_{-0.11}$ &    53.0 &           9.9 &  15.1 $\pm$ 3.2 &   0.68 $\pm$ 0.1 &         -49.4 &            13.6 &             21.7 \\
 71 &  348.9485 &  61.8150 &  104 &         12.5 &          9.1 &  0.26 $^{+0.12}_{-0.06}$ &    32.1 &           2.2 &  13.7 $\pm$ 2.9 &   0.4 $\pm$ 0.06 &         -49.1 &            13.7 &             21.7 \\
 72 &  349.0657 &  61.8166 &  166 &         15.7 &          7.4 &   0.27 $^{+0.1}_{-0.09}$ &    34.3 &           2.3 &  11.8 $\pm$ 4.0 &  0.43 $\pm$ 0.11 &         -48.8 &            14.3 &             21.6 \\
\bottomrule
\end{tabular}


==> NGC7538_leaf_stats_virial.tex <==
\begin{tabular}{rrrrrrrrllrr}
\toprule
 ID &  $\alpha_{vir}$ &  $M_{vir}$ &  $\sigma_{nt}$ & log$|\Omega_G|$ & log$\Omega_K$ & log$|\Omega_{Pw}|$ &  log$|\Omega_{Pt}|$ & on-filament & hub & $N_{proto}$ & Bad N(H$_2$) Pixels \\& & (M$_\odot$) & (km s$^{-1}$) & (erg) & (erg) & (erg) & (erg) & & & \\\midrule
  0 &   2.03 &             578.3 &      0.90 &  45.8 &     45.9 &     45.8 &         NaN &        False &  False &           1 &      0.00 \\
  1 &   3.33 &              72.2 &      0.45 &  43.9 &     44.2 &     44.6 &         NaN &        False &  False &           0 &      0.00 \\
  2 &   2.70 &              59.8 &      0.44 &  44.0 &     44.2 &     44.5 &         NaN &        False &  False &           0 &      0.00 \\
  3 &   1.46 &              63.9 &      0.34 &  44.4 &     44.4 &     44.9 &         NaN &        False &  False &           0 &      0.00 \\
  4 &   5.38 &              93.5 &      0.59 &  43.8 &     44.3 &     44.4 &         NaN &        False &  False &           0 &      0.00 \\
  5 &   3.87 &              81.1 &      0.52 &  43.9 &     44.3 &     44.4 &         NaN &        False &  False &           0 &      0.00 \\
  6 &   3.76 &             151.0 &      0.61 &  44.3 &     44.7 &     44.9 &         NaN &        False &  False &           0 &      0.00 \\
  7 &   0.91 &             255.7 &      0.53 &  45.7 &     45.5 &     46.0 &         NaN &        False &  False &           2 &      0.00 \\
  8 &   1.71 &              62.5 &      0.38 &  44.3 &     44.3 &     44.7 &         NaN &        False &  False &           2 &      0.00 \\
  9 &   4.83 &             411.3 &      0.91 &  44.9 &     45.4 &     45.4 &         NaN &        False &  False &           0 &      0.00 \\
 10 &   6.65 &             163.9 &      0.87 &  44.2 &     44.8 &     44.3 &         NaN &        False &  False &           0 &      0.00 \\
 11 &   6.23 &             158.6 &      0.82 &  44.2 &     44.7 &     44.5 &         NaN &        False &  False &           0 &      0.00 \\
 12 &   1.01 &             155.0 &      0.58 &  45.4 &     45.3 &     45.4 &         NaN &         True &  False &           0 &      0.00 \\
 13 &   2.46 &             248.5 &      0.73 &  45.1 &     45.2 &     45.4 &         NaN &        False &  False &           1 &      0.00 \\
 14 &  14.19 &             225.1 &      1.03 &  43.8 &     44.7 &     44.5 &         NaN &         True &  False &           0 &      0.00 \\
 15 &   1.23 &              90.5 &      0.39 &  44.8 &     44.7 &     45.3 &         NaN &        False &  False &           0 &      0.00 \\
 16 &   7.60 &             646.0 &      1.46 &  45.1 &     45.7 &     45.0 &         NaN &         True &  False &           1 &      0.00 \\
 17 &  12.24 &             449.0 &      1.38 &  44.5 &     45.3 &     44.7 &         NaN &         True &  False &           1 &      0.00 \\
 18 &   1.58 &             125.6 &      0.60 &  45.0 &     45.0 &     45.1 &         NaN &         True &  False &           0 &      0.00 \\
 19 &   0.94 &             534.3 &      0.81 &  46.3 &     46.1 &     46.3 &         NaN &         True &  False &           4 &      0.00 \\
 20 &   1.62 &              83.7 &      0.53 &  44.7 &     44.7 &     44.8 &         NaN &         True &  False &           0 &      0.00 \\
 21 &   3.04 &              48.2 &      0.43 &  43.8 &     44.1 &     44.3 &         NaN &        False &  False &           0 &      0.00 \\
 22 &   0.83 &             350.3 &      0.80 &  46.2 &     45.9 &     45.8 &         NaN &         True &  False &           2 &      0.00 \\
 23 &   1.31 &             102.0 &      0.51 &  44.9 &     44.9 &     45.2 &         NaN &        False &  False &           0 &      0.00 \\
 24 &   1.02 &             265.8 &      0.71 &  45.8 &     45.6 &     45.7 &         NaN &         True &  False &           3 &      0.00 \\
 25 &   4.87 &             252.1 &      1.04 &  44.8 &     45.3 &     44.6 &         NaN &         True &  False &           1 &      0.00 \\
 26 &   1.67 &             212.9 &      0.82 &  45.4 &     45.4 &     45.1 &         NaN &        False &  False &           0 &      0.00 \\
 27 &   2.16 &              57.2 &      0.45 &  44.2 &     44.3 &     44.5 &         NaN &         True &  False &           2 &      0.00 \\
 28 &   6.76 &             320.3 &      1.00 &  44.6 &     45.2 &     45.0 &         NaN &         True &  False &           0 &      0.00 \\
 29 &   1.54 &             100.7 &      0.64 &  45.0 &     45.0 &     44.7 &         NaN &        False &  False &           0 &      0.00 \\
 30 &   2.11 &              41.3 &      0.35 &  43.9 &     44.0 &     44.4 &         NaN &         True &  False &           0 &      0.00 \\
 31 &   1.01 &              73.2 &      0.40 &  44.9 &     44.7 &     45.3 &         NaN &         True &  False &           0 &      0.00 \\
 32 &   1.23 &              85.5 &      0.41 &  44.8 &     44.7 &     45.4 &         NaN &        False &  False &           1 &      0.00 \\
 33 &   2.13 &             346.8 &      0.82 &  45.4 &     45.5 &     45.6 &         NaN &         True &  False &           3 &      0.00 \\
 34 &   1.19 &             191.5 &      0.57 &  45.4 &     45.3 &     45.7 &         NaN &         True &  False &           0 &      0.00 \\
 35 &   3.67 &              93.9 &      0.65 &  44.2 &     44.6 &     44.4 &         NaN &         True &  False &           0 &      0.00 \\
 36 &   1.10 &              36.6 &      0.32 &  44.3 &     44.1 &     44.9 &         NaN &         True &  False &           0 &      0.00 \\
 37 &   4.64 &             172.7 &      0.68 &  44.3 &     44.8 &     44.9 &         NaN &         True &  False &           1 &      0.00 \\
 38 &   1.33 &             208.1 &      0.90 &  45.7 &     45.6 &     45.1 &        46.2 &         True &  False &           0 &      0.00 \\
 39 &   2.18 &              98.5 &      0.50 &  44.5 &     44.6 &     45.0 &         NaN &        False &  False &           1 &      0.00 \\
 40 &   0.52 &             145.5 &      0.64 &  46.1 &     45.6 &     45.4 &         NaN &         True &  False &           4 &      0.00 \\
 41 &   0.66 &             181.1 &      0.49 &  45.8 &     45.4 &     46.1 &         NaN &         True &  False &           2 &      0.00 \\
 42 &   2.49 &             114.4 &      0.56 &  44.5 &     44.7 &     44.8 &         NaN &         True &  False &           0 &      0.00 \\
 43 &   0.45 &            1354.1 &      1.21 &  47.7 &     47.1 &     46.9 &        48.2 &        False &   True &           2 &      0.02 \\
 44 &   1.72 &              59.3 &      0.48 &  44.4 &     44.4 &     44.8 &         NaN &        False &  False &           0 &      0.00 \\
 45 &   2.53 &              43.3 &      0.40 &  43.8 &     44.0 &     44.3 &         NaN &         True &  False &           0 &      0.00 \\
 46 &   0.91 &             156.7 &      0.52 &  45.5 &     45.2 &     45.5 &        46.4 &         True &  False &           0 &      0.00 \\
 47 &   1.86 &             196.2 &      0.93 &  45.4 &     45.5 &     44.8 &         NaN &         True &  False &           1 &      0.00 \\
 48 &   1.55 &             202.9 &      0.84 &  45.5 &     45.5 &     45.1 &        46.4 &         True &  False &           0 &      0.00 \\
 49 &   4.68 &             593.9 &      1.60 &  45.5 &     46.0 &     44.9 &         NaN &         True &  False &           1 &      0.00 \\
 50 &   0.92 &             360.9 &      0.75 &  46.1 &     45.9 &     46.1 &        47.2 &         True &  False &           0 &      0.00 \\
 51 &   2.95 &             309.2 &      0.92 &  45.2 &     45.5 &     45.4 &        46.5 &        False &  False &           0 &      0.00 \\
 52 &   0.91 &              66.8 &      0.40 &  44.9 &     44.7 &     44.9 &         NaN &         True &  False &           1 &      0.00 \\
 53 &   0.83 &             383.0 &      0.65 &  46.1 &     45.8 &     46.2 &        47.2 &        False &  False &           2 &      0.00 \\
 54 &   1.30 &              60.6 &      0.43 &  44.6 &     44.5 &     44.7 &         NaN &         True &  False &           2 &      0.00 \\
 55 &   1.00 &             122.6 &      0.49 &  45.2 &     45.0 &     45.3 &         NaN &         True &  False &           4 &      0.00 \\
 56 &   0.89 &              87.6 &      0.44 &  45.1 &     44.9 &     45.2 &         NaN &         True &  False &           0 &      0.00 \\
 57 &   0.95 &             164.6 &      0.56 &  45.5 &     45.3 &     45.4 &         NaN &         True &  False &           1 &      0.00 \\
 58 &   1.16 &              64.2 &      0.37 &  44.6 &     44.5 &     45.0 &         NaN &        False &  False &           0 &      0.00 \\
 59 &   0.61 &             377.2 &      0.60 &  46.3 &     45.9 &     46.3 &         NaN &        False &  False &           4 &      0.00 \\
 60 &   1.92 &             147.4 &      0.61 &  44.9 &     45.0 &     45.2 &         NaN &         True &  False &           0 &      0.00 \\
 61 &   0.95 &             136.5 &      0.50 &  45.3 &     45.1 &     45.6 &         NaN &         True &  False &           1 &      0.00 \\
 62 &   3.39 &              72.3 &      0.54 &  44.0 &     44.4 &     44.4 &         NaN &         True &  False &           0 &      0.00 \\
 63 &   1.85 &              65.4 &      0.47 &  44.4 &     44.5 &     44.7 &         NaN &         True &  False &           0 &      0.00 \\
 64 &   3.38 &             132.5 &      0.64 &  44.4 &     44.7 &     44.9 &         NaN &         True &  False &           0 &      0.00 \\
 65 &   1.06 &             107.2 &      0.53 &  45.2 &     45.0 &     45.1 &         NaN &         True &  False &           1 &      0.00 \\
 66 &   0.74 &             137.2 &      0.47 &  45.5 &     45.2 &     45.6 &         NaN &         True &  False &           0 &      0.00 \\
 67 &  69.26 &             427.9 &      1.42 &  42.9 &     44.6 &     44.0 &         NaN &        False &  False &           0 &      0.00 \\
 68 &   0.78 &             322.7 &      0.70 &  46.2 &     45.8 &     45.7 &         NaN &        False &  False &           3 &      0.00 \\
 69 &   2.64 &             189.3 &      0.71 &  44.9 &     45.1 &     45.1 &         NaN &        False &  False &           0 &      0.00 \\
 70 &   2.58 &             136.4 &      0.67 &  44.7 &     44.9 &     44.8 &         NaN &        False &  False &           0 &      0.00 \\
 71 &   1.51 &              48.4 &      0.39 &  44.3 &     44.3 &     44.6 &         NaN &        False &  False &           0 &      0.00 \\
 72 &   1.63 &              56.0 &      0.43 &  44.4 &     44.4 &     44.6 &         NaN &        False &  False &           0 &      0.00 \\
\bottomrule
\end{tabular}


==> Rosette_leaf_stats.tex <==
\begin{tabular}{rrrrrrlrrllrrr}
\toprule
ID & RA & decl. & PA & $\sigma_{major}$ & $\sigma_{minor}$ &  $R_{eff}$ &  $M_{obs}$ &  $M_{clip}$ &  $T_K$ &  $\sigma_{NH_3}$ &  $V_{LSR, NH_3}$ &  log($N_{para-NH_3}$) &  log($N_{H_2}$) \\& (deg) & (deg) & (deg) & ($\arcsec$) & ($\arcsec$) & (pc) & (M$_\odot$) & (M$_\odot$) & (K) & (km s$^{-1}$) & (km s$^{-1}$) & (cm$^{-2}$) & (cm$^{-2}$) \\\midrule
  0 &  98.6014 &  4.0181 &   77 &         27.5 &         11.9 &  0.24 $^{+0.21}_{-0.11}$ &   25.2 &           5.1 &  16.5 $\pm$ 3.2 &  0.22 $\pm$ 0.04 &          16.0 &            13.3 &             21.6 \\
  1 &  98.3692 &  4.0146 &   77 &         28.4 &         13.0 &  0.27 $^{+0.12}_{-0.16}$ &   43.3 &          18.2 &  18.6 $\pm$ 3.3 &  0.57 $\pm$ 0.09 &          14.8 &            13.7 &             21.5 \\
  2 &  98.3335 &  4.0146 &  100 &         12.5 &          6.2 &  0.12 $^{+0.04}_{-0.05}$ &    4.7 &           0.5 &  18.6 $\pm$ 4.7 &  0.67 $\pm$ 0.15 &          14.8 &            13.8 &             21.5 \\
  3 &  98.6651 &  4.1077 &  120 &         15.2 &          6.0 &  0.13 $^{+0.04}_{-0.05}$ &    5.1 &           0.6 &  16.5 $\pm$ 3.7 &  0.58 $\pm$ 0.11 &          11.9 &            14.1 &             21.6 \\
  4 &  98.6565 &  4.1400 &   55 &         39.4 &         18.9 &  0.41 $^{+0.36}_{-0.15}$ &   88.8 &          33.8 &  13.1 $\pm$ 1.8 &  0.37 $\pm$ 0.04 &          11.3 &            13.9 &             21.7 \\
  5 &  98.6810 &  4.1273 &  225 &         12.2 &          6.8 &  0.12 $^{+0.02}_{-0.05}$ &    3.6 &           0.3 &  14.5 $\pm$ 3.3 &  0.34 $\pm$ 0.07 &          12.0 &            13.8 &             21.6 \\
  6 &  98.6171 &  4.1479 &  149 &         12.6 &          8.1 &  0.14 $^{+0.04}_{-0.01}$ &    7.4 &           1.1 &  13.2 $\pm$ 2.9 &  0.21 $\pm$ 0.04 &          11.3 &            13.6 &             21.7 \\
  7 &  98.6596 &  4.1695 &  199 &         28.8 &          9.7 &  0.22 $^{+0.21}_{-0.12}$ &   25.3 &           6.8 &  15.1 $\pm$ 3.0 &  0.35 $\pm$ 0.06 &          12.2 &            13.8 &             21.8 \\
  8 &  98.6047 &  4.1757 &   70 &         16.2 &         11.8 &   0.17 $^{+0.08}_{-0.1}$ &   10.0 &           1.4 &  15.1 $\pm$ 3.6 &  0.32 $\pm$ 0.07 &          11.6 &            13.9 &             21.6 \\
  9 &  98.6853 &  4.1758 &  208 &         23.4 &          9.7 &   0.2 $^{+0.11}_{-0.08}$ &   20.4 &           5.6 &  11.6 $\pm$ 1.5 &  0.25 $\pm$ 0.02 &          13.3 &            13.8 &             21.7 \\
 10 &  98.6590 &  4.2055 &  203 &         42.2 &         19.3 &  0.38 $^{+0.21}_{-0.23}$ &  127.6 &          59.1 &  16.9 $\pm$ 1.2 &  0.51 $\pm$ 0.03 &          12.7 &            14.0 &             21.7 \\
 11 &  98.5984 &  4.1971 &  218 &         22.5 &         11.7 &  0.21 $^{+0.13}_{-0.07}$ &   15.1 &           2.6 &  11.9 $\pm$ 3.1 &  0.26 $\pm$ 0.04 &          11.5 &            13.5 &             21.6 \\
 12 &  98.6119 &  4.2156 &  223 &         11.9 &          9.2 &  0.14 $^{+0.03}_{-0.02}$ &    6.7 &           0.8 &  14.6 $\pm$ 3.9 &   0.4 $\pm$ 0.08 &          12.0 &            13.6 &             21.7 \\
 13 &  98.6000 &  4.2256 &   97 &         19.8 &          8.4 &  0.15 $^{+0.08}_{-0.12}$ &    7.1 &           0.5 &  15.9 $\pm$ 4.1 &  0.49 $\pm$ 0.11 &          12.4 &            14.2 &             21.7 \\
 14 &  98.6076 &  4.2427 &   97 &         14.7 &         12.2 &  0.18 $^{+0.02}_{-0.04}$ &   14.4 &           2.4 &  15.4 $\pm$ 2.7 &  0.43 $\pm$ 0.07 &          13.3 &            13.6 &             21.7 \\
 15 &  98.5530 &  4.2608 &  137 &         16.6 &          9.5 &  0.16 $^{+0.06}_{-0.08}$ &   11.4 &           1.4 &  13.5 $\pm$ 4.0 &  0.96 $\pm$ 0.18 &          11.6 &            14.1 &             21.7 \\
 16 &  97.9372 &  4.2634 &  215 &         15.4 &         11.0 &  0.18 $^{+0.03}_{-0.06}$ &    9.2 &           1.7 &  10.8 $\pm$ 3.2 &  0.18 $\pm$ 0.03 &          12.7 &            13.4 &             21.5 \\
 17 &  98.5425 &  4.2862 &  132 &         33.0 &         10.9 &  0.26 $^{+0.21}_{-0.11}$ &   45.3 &           9.2 &  12.4 $\pm$ 2.3 &  0.48 $\pm$ 0.05 &          11.5 &            13.9 &             21.8 \\
 18 &  98.5733 &  4.2781 &  175 &         13.6 &          9.2 &  0.15 $^{+0.06}_{-0.02}$ &   12.5 &           1.8 &  11.7 $\pm$ 2.7 &  0.42 $\pm$ 0.05 &          12.7 &            13.6 &             21.8 \\
 19 &  97.9162 &  4.2793 &  122 &         10.8 &          7.8 &  0.13 $^{+0.03}_{-0.01}$ &    5.3 &           0.5 &  12.0 $\pm$ 3.3 &  0.33 $\pm$ 0.06 &          10.5 &            14.0 &             21.5 \\
 20 &  98.5982 &  4.2789 &  175 &         13.7 &          6.9 &  0.13 $^{+0.09}_{-0.02}$ &    5.7 &           0.8 &  11.1 $\pm$ 3.1 &  0.24 $\pm$ 0.04 &          12.9 &            13.8 &             21.7 \\
 21 &  98.6299 &  4.2977 &  195 &         31.9 &         15.0 &   0.27 $^{+0.27}_{-0.2}$ &   27.6 &           6.8 &  13.1 $\pm$ 3.4 &  0.39 $\pm$ 0.07 &          12.3 &            13.4 &             21.6 \\
 22 &  98.5736 &  4.2979 &  140 &         22.7 &         16.6 &   0.23 $^{+0.12}_{-0.2}$ &   33.5 &           4.1 &  11.2 $\pm$ 2.5 &  0.47 $\pm$ 0.06 &          11.1 &            13.8 &             21.8 \\
 23 &  98.5327 &  4.2998 &   94 &         13.5 &          5.5 &  0.11 $^{+0.05}_{-0.05}$ &    6.5 &           0.4 &  15.4 $\pm$ 3.6 &   0.3 $\pm$ 0.06 &          15.7 &            13.2 &             21.8 \\
 24 &  98.5284 &  4.3195 &   83 &         22.8 &         10.6 &  0.21 $^{+0.13}_{-0.05}$ &   27.6 &           6.4 &  13.9 $\pm$ 2.6 &  0.36 $\pm$ 0.06 &          15.8 &            13.8 &             21.8 \\
 25 &  97.9643 &  4.3181 &  224 &         21.4 &         14.9 &  0.27 $^{+0.06}_{-0.08}$ &   39.4 &          17.5 &  17.1 $\pm$ 2.8 &  0.44 $\pm$ 0.07 &          13.7 &            13.9 &             21.5 \\
 26 &  97.9869 &  4.3179 &  196 &         15.9 &         13.4 &   0.2 $^{+0.12}_{-0.07}$ &   13.6 &           4.0 &  12.3 $\pm$ 3.0 &  0.26 $\pm$ 0.05 &          13.2 &            14.2 &             21.5 \\
 27 &  98.5672 &  4.3157 &  209 &         11.8 &          6.7 &  0.11 $^{+0.03}_{-0.03}$ &   10.3 &           0.9 &  18.8 $\pm$ 2.2 &  0.56 $\pm$ 0.06 &           9.9 &            13.8 &             21.8 \\
 28 &  98.5608 &  4.3425 &   86 &         33.2 &         13.9 &  0.29 $^{+0.16}_{-0.13}$ &   70.6 &          22.4 &  16.4 $\pm$ 2.2 &  0.42 $\pm$ 0.05 &          10.8 &            13.7 &             21.8 \\
 29 &  98.5358 &  4.3558 &   99 &         32.4 &         14.9 &  0.33 $^{+0.14}_{-0.14}$ &   76.1 &          25.0 &  11.5 $\pm$ 1.5 &  0.32 $\pm$ 0.03 &          12.5 &            14.1 &             21.8 \\
 30 &  97.8343 &  4.3663 &  195 &         15.1 &         10.8 &  0.17 $^{+0.07}_{-0.03}$ &    8.9 &           3.4 &  19.4 $\pm$ 2.9 &  0.39 $\pm$ 0.06 &          18.5 &            13.5 &             21.4 \\
 31 &  98.5562 &  4.3783 &  213 &         14.9 &         13.2 &   0.2 $^{+0.04}_{-0.03}$ &   31.0 &          11.1 &  13.9 $\pm$ 2.3 &  0.45 $\pm$ 0.05 &          11.4 &            13.8 &             21.8 \\
 32 &  98.5737 &  4.3807 &  133 &         15.5 &          9.0 &  0.13 $^{+0.07}_{-0.08}$ &    7.9 &           1.5 &  21.5 $\pm$ 4.0 &  0.85 $\pm$ 0.14 &          11.5 &            13.6 &             21.7 \\
 33 &  98.5358 &  4.4427 &  123 &         18.6 &         12.8 &  0.23 $^{+0.05}_{-0.06}$ &   28.4 &           7.4 &  18.6 $\pm$ 2.6 &  0.45 $\pm$ 0.06 &          15.0 &            13.7 &             21.6 \\
 34 &  98.5404 &  4.4689 &  122 &         12.7 &         10.3 &   0.15 $^{+0.04}_{-0.1}$ &    8.5 &           1.4 &  16.5 $\pm$ 3.4 &  0.41 $\pm$ 0.07 &          15.8 &            13.6 &             21.5 \\
 35 &  98.2447 &  4.4683 &  208 &         15.0 &          9.4 &  0.16 $^{+0.04}_{-0.08}$ &    9.4 &           3.4 &  13.1 $\pm$ 3.2 &  0.28 $\pm$ 0.05 &          16.5 &            14.0 &             21.3 \\
 36 &  98.4988 &  4.4907 &  209 &         26.5 &         12.9 &   0.24 $^{+0.2}_{-0.18}$ &   16.0 &           5.3 &  14.1 $\pm$ 2.9 &  0.39 $\pm$ 0.06 &          15.9 &            13.5 &             21.5 \\
 37 &  98.5237 &  4.4961 &   54 &         17.1 &          8.4 &  0.15 $^{+0.06}_{-0.05}$ &    5.9 &           0.8 &  14.3 $\pm$ 4.0 &   0.54 $\pm$ 0.1 &          15.9 &            14.1 &             21.5 \\
 38 &  98.4709 &  4.5113 &  133 &         12.6 &          9.0 &  0.14 $^{+0.03}_{-0.04}$ &    5.0 &           0.9 &  14.7 $\pm$ 3.2 &  0.34 $\pm$ 0.06 &          15.9 &            13.4 &             21.4 \\
 39 &  98.4115 &  4.5303 &  107 &         30.2 &         22.3 &  0.37 $^{+0.23}_{-0.13}$ &   41.2 &          13.5 &  13.9 $\pm$ 2.2 &  0.48 $\pm$ 0.06 &          13.6 &            13.9 &             21.3 \\
 40 &  98.5069 &  4.5350 &  214 &         13.7 &          8.8 &  0.14 $^{+0.04}_{-0.04}$ &    5.1 &           0.6 &  13.8 $\pm$ 3.6 &  0.18 $\pm$ 0.04 &          15.5 &            13.8 &             21.4 \\
 41 &  98.6522 &  4.5898 &  155 &         11.8 &          8.1 &  0.13 $^{+0.03}_{-0.04}$ &    4.4 &           1.3 &  15.0 $\pm$ 4.0 &   0.45 $\pm$ 0.1 &          14.7 &            13.9 &             21.3 \\
 42 &  98.2916 &  4.6352 &  222 &         10.9 &         10.9 &  0.15 $^{+0.01}_{-0.03}$ &    6.0 &           2.5 &  21.0 $\pm$ 3.7 &    0.6 $\pm$ 0.1 &          20.3 &            13.9 &             21.1 \\
 43 &  98.4631 &  4.6427 &  218 &         11.5 &         10.6 &   0.15 $^{+0.0}_{-0.01}$ &    5.2 &           0.7 &  15.7 $\pm$ 3.6 &  0.19 $\pm$ 0.04 &          12.5 &            13.8 &             21.3 \\
 44 &  98.3478 &  4.6767 &   60 &         13.9 &         11.1 &  0.14 $^{+0.03}_{-0.11}$ &    3.3 &           1.0 &  20.7 $\pm$ 3.9 &  0.43 $\pm$ 0.08 &           9.9 &            13.4 &             21.1 \\
 45 &  98.3595 &  4.7624 &   48 &         53.1 &         14.2 &  0.38 $^{+0.37}_{-0.24}$ &   37.2 &          18.2 &  16.1 $\pm$ 2.2 &  0.37 $\pm$ 0.05 &          10.5 &            13.9 &             21.2 \\
 46 &  98.2988 &  4.7686 &  104 &         13.9 &         10.9 &  0.17 $^{+0.04}_{-0.04}$ &    7.2 &           3.2 &  17.5 $\pm$ 3.4 &  0.49 $\pm$ 0.08 &          11.3 &            14.1 &             21.1 \\
 47 &  98.4009 &  4.8288 &  163 &         10.6 &          8.5 &  0.13 $^{+-0.0}_{-0.01}$ &    3.9 &           1.5 &  19.4 $\pm$ 3.4 &  0.48 $\pm$ 0.08 &          10.4 &            13.6 &             21.0 \\
\bottomrule
\end{tabular}


==> Rosette_leaf_stats_virial.tex <==
\begin{tabular}{rrrrrrrrllrr}
\toprule
 ID &  $\alpha_{vir}$ &  $M_{vir}$ &  $\sigma_{nt}$ & log$|\Omega_G|$ & log$\Omega_K$ & log$|\Omega_{Pw}|$ &  log$|\Omega_{Pt}|$ & on-filament & hub & $N_{proto}$ & Bad N(H$_2$) Pixels \\& & (M$_\odot$) & (km s$^{-1}$) & (erg) & (erg) & (erg) & (erg) & & & \\\midrule
  0 &   0.86 &              21.7 &      0.20 &  44.1 &     43.9 &     44.2 &         NaN &         True &  False &           0 &         0 \\
  1 &   2.21 &              95.6 &      0.56 &  44.5 &     44.7 &     44.4 &         NaN &         True &  False &           3 &         0 \\
  2 &  11.64 &              55.2 &      0.67 &  43.0 &     43.9 &     43.2 &         NaN &        False &  False &           2 &         0 \\
  3 &   8.76 &              44.7 &      0.57 &  43.0 &     43.8 &     43.4 &         NaN &         True &  False &           0 &         0 \\
  4 &   0.76 &              67.1 &      0.36 &  45.0 &     44.7 &     45.0 &         NaN &         True &  False &           1 &         0 \\
  5 &   4.80 &              17.5 &      0.33 &  42.8 &     43.2 &     43.3 &         NaN &        False &  False &           0 &         0 \\
  6 &   1.53 &              11.4 &      0.20 &  43.3 &     43.3 &     43.6 &         NaN &         True &  False &           0 &         0 \\
  7 &   1.36 &              34.3 &      0.34 &  44.2 &     44.1 &     44.3 &         NaN &         True &  False &           1 &         0 \\
  8 &   2.43 &              24.2 &      0.31 &  43.5 &     43.7 &     43.9 &         NaN &        False &  False &           0 &         0 \\
  9 &   0.89 &              18.1 &      0.24 &  44.0 &     43.8 &     44.1 &         NaN &         True &  False &           2 &         0 \\
 10 &   0.86 &             109.7 &      0.50 &  45.3 &     45.1 &     45.0 &         NaN &         True &  False &           0 &         0 \\
 11 &   1.37 &              20.8 &      0.25 &  43.7 &     43.7 &     44.1 &         NaN &        False &  False &           0 &         0 \\
 12 &   3.91 &              26.2 &      0.39 &  43.2 &     43.6 &     43.6 &         NaN &        False &  False &           0 &         0 \\
 13 &   5.47 &              38.9 &      0.48 &  43.2 &     43.8 &     43.7 &         NaN &        False &  False &           0 &         0 \\
 14 &   2.73 &              39.4 &      0.42 &  43.8 &     44.0 &     44.0 &         NaN &        False &  False &           0 &         0 \\
 15 &  12.45 &             141.9 &      0.96 &  43.6 &     44.5 &     43.8 &         NaN &         True &  False &           0 &         0 \\
 16 &   1.23 &              11.3 &      0.17 &  43.4 &     43.3 &     43.8 &         NaN &         True &  False &           1 &         0 \\
 17 &   1.43 &              64.8 &      0.47 &  44.6 &     44.6 &     44.5 &         NaN &         True &  False &           1 &         0 \\
 18 &   2.39 &              29.9 &      0.41 &  43.7 &     43.9 &     43.8 &         NaN &         True &  False &           0 &         0 \\
 19 &   3.47 &              18.6 &      0.33 &  43.0 &     43.4 &     43.4 &         NaN &         True &  False &           0 &         0 \\
 20 &   1.96 &              11.1 &      0.23 &  43.1 &     43.2 &     43.6 &         NaN &         True &  False &           0 &         0 \\
 21 &   1.80 &              49.6 &      0.39 &  44.2 &     44.2 &     44.4 &         NaN &         True &  False &           0 &         0 \\
 22 &   1.67 &              56.1 &      0.47 &  44.4 &     44.4 &     44.4 &         NaN &         True &  False &           2 &         0 \\
 23 &   2.18 &              14.2 &      0.29 &  43.3 &     43.4 &     43.5 &         NaN &         True &  False &           0 &         0 \\
 24 &   1.23 &              34.0 &      0.35 &  44.3 &     44.1 &     44.3 &         NaN &         True &  False &           3 &         0 \\
 25 &   1.59 &              62.6 &      0.44 &  44.5 &     44.5 &     44.3 &         NaN &         True &  False &           1 &         0 \\
 26 &   1.40 &              19.1 &      0.25 &  43.7 &     43.6 &     43.9 &         NaN &         True &  False &           1 &         0 \\
 27 &   3.73 &              38.3 &      0.55 &  43.7 &     44.1 &     43.5 &         NaN &         True &  False &           2 &         0 \\
 28 &   0.88 &              61.9 &      0.41 &  44.9 &     44.7 &     44.8 &         NaN &         True &  False &           3 &         0 \\
 29 &   0.55 &              42.0 &      0.31 &  44.9 &     44.5 &     44.9 &         NaN &         True &  False &           4 &         0 \\
 30 &   3.75 &              33.3 &      0.37 &  43.4 &     43.7 &     43.6 &         NaN &         True &  False &           2 &         0 \\
 31 &   1.44 &              44.8 &      0.44 &  44.4 &     44.4 &     44.2 &         NaN &        False &  False &           3 &         0 \\
 32 &  12.14 &              95.8 &      0.84 &  43.4 &     44.3 &     43.6 &         NaN &         True &  False &           0 &         0 \\
 33 &   1.91 &              54.3 &      0.44 &  44.3 &     44.3 &     44.2 &         NaN &         True &  False &           1 &         0 \\
 34 &   3.76 &              31.9 &      0.40 &  43.4 &     43.7 &     43.6 &         NaN &         True &  False &           0 &         0 \\
 35 &   1.85 &              17.5 &      0.26 &  43.5 &     43.5 &     43.5 &         NaN &         True &  False &           0 &         0 \\
 36 &   2.75 &              44.1 &      0.38 &  43.7 &     44.0 &     44.1 &         NaN &         True &  False &           0 &         0 \\
 37 &   7.77 &              46.1 &      0.54 &  43.1 &     43.8 &     43.5 &         NaN &         True &  False &           0 &         0 \\
 38 &   4.20 &              21.0 &      0.33 &  43.0 &     43.4 &     43.4 &         NaN &         True &  False &           0 &         0 \\
 39 &   2.32 &              95.6 &      0.48 &  44.4 &     44.5 &     44.6 &         NaN &        False &  False &           0 &         0 \\
 40 &   1.92 &               9.8 &      0.16 &  43.0 &     43.1 &     43.4 &         NaN &         True &  False &           0 &         0 \\
 41 &   6.94 &              30.2 &      0.44 &  42.9 &     43.5 &     43.2 &         NaN &         True &  False &           0 &         0 \\
 42 &  10.26 &              61.3 &      0.59 &  43.1 &     43.9 &     43.2 &         NaN &        False &  False &           1 &         0 \\
 43 &   2.34 &              12.1 &      0.17 &  42.9 &     43.1 &     43.4 &         NaN &         True &  False &           0 &         0 \\
 44 &   9.91 &              33.0 &      0.42 &  42.6 &     43.4 &     43.1 &         NaN &        False &  False &           0 &         0 \\
 45 &   1.79 &              66.8 &      0.36 &  44.3 &     44.3 &     44.5 &         NaN &         True &  False &           1 &         0 \\
 46 &   6.43 &              46.0 &      0.48 &  43.2 &     43.8 &     43.3 &         NaN &         True &  False &           0 &         0 \\
 47 &   9.36 &              36.3 &      0.47 &  42.8 &     43.5 &     42.9 &         NaN &        False &  False &           1 &         0 \\
\bottomrule
\end{tabular}


==> W3_leaf_stats.tex <==
\begin{tabular}{rrrrrrlrrllrrr}
\toprule
ID & RA & decl. & PA & $\sigma_{major}$ & $\sigma_{minor}$ &  $R_{eff}$ &  $M_{obs}$ &  $M_{clip}$ &  $T_K$ &  $\sigma_{NH_3}$ &  $V_{LSR, NH_3}$ &  log($N_{para-NH_3}$) &  log($N_{H_2}$) \\& (deg) & (deg) & (deg) & ($\arcsec$) & ($\arcsec$) & (pc) & (M$_\odot$) & (M$_\odot$) & (K) & (km s$^{-1}$) & (km s$^{-1}$) & (cm$^{-2}$) & (cm$^{-2}$) \\\midrule
  0 &  36.5415 &  61.0964 &  185 &         16.1 &          7.6 &  0.18 $^{+0.14}_{-0.14}$ &    7.1 &           1.1 &  12.3 $\pm$ 4.1 &  0.19 $\pm$ 0.05 &         -49.2 &            13.6 &             21.2 \\
  1 &  36.4968 &  61.1103 &  213 &         26.0 &          9.4 &  0.33 $^{+0.21}_{-0.13}$ &   26.5 &           7.0 &  12.0 $\pm$ 2.8 &  0.25 $\pm$ 0.04 &         -49.7 &            13.7 &             21.3 \\
  2 &  36.4520 &  61.1305 &  200 &         14.4 &         12.4 &  0.28 $^{+0.05}_{-0.01}$ &   25.2 &           6.7 &  11.0 $\pm$ 3.1 &  0.31 $\pm$ 0.05 &         -50.2 &            13.7 &             21.3 \\
  3 &  36.3429 &  61.1377 &  104 &         22.2 &          9.6 &  0.25 $^{+0.17}_{-0.13}$ &   17.4 &           5.0 &  14.2 $\pm$ 4.1 &  0.58 $\pm$ 0.12 &         -47.5 &            13.9 &             21.4 \\
  4 &  36.4152 &  61.1731 &  150 &         16.8 &         12.0 &   0.3 $^{+0.05}_{-0.05}$ &   26.2 &           8.1 &  12.5 $\pm$ 2.4 &  0.59 $\pm$ 0.07 &         -48.0 &            13.8 &             21.4 \\
  5 &  36.4070 &  61.2240 &  101 &         55.6 &         29.5 &  0.79 $^{+0.67}_{-0.31}$ &  295.6 &         149.7 &  12.5 $\pm$ 1.5 &  0.39 $\pm$ 0.03 &         -47.8 &            14.0 &             21.4 \\
  6 &  36.3754 &  61.1927 &  137 &         15.3 &          6.2 &  0.17 $^{+0.11}_{-0.08}$ &    8.1 &           1.2 &  15.0 $\pm$ 3.2 &  0.75 $\pm$ 0.12 &         -48.7 &            13.9 &             21.4 \\
  7 &  36.3567 &  61.2493 &   97 &         25.0 &         18.2 &  0.44 $^{+0.24}_{-0.14}$ &   81.9 &          31.3 &  12.1 $\pm$ 1.8 &  0.36 $\pm$ 0.04 &         -48.7 &            13.9 &             21.4 \\
  8 &  36.3695 &  61.2742 &  214 &         15.7 &         11.8 &   0.24 $^{+0.12}_{-0.1}$ &   24.9 &           4.7 &  14.9 $\pm$ 2.8 &   0.73 $\pm$ 0.1 &         -48.3 &            14.0 &             21.4 \\
  9 &  36.3028 &  61.3043 &  137 &         24.1 &         13.6 &  0.36 $^{+0.14}_{-0.09}$ &   40.1 &           9.2 &  12.4 $\pm$ 2.9 &  0.24 $\pm$ 0.04 &         -47.2 &            13.8 &             21.4 \\
 10 &  36.3714 &  61.3075 &   56 &         12.6 &         11.2 &  0.23 $^{+0.06}_{-0.09}$ &   14.3 &           3.7 &  13.3 $\pm$ 3.4 &  0.35 $\pm$ 0.07 &         -47.4 &            13.9 &             21.4 \\
 11 &  36.4519 &  61.3472 &  162 &         16.3 &         10.2 &  0.26 $^{+0.08}_{-0.07}$ &   21.4 &           6.5 &  19.0 $\pm$ 3.1 &  0.42 $\pm$ 0.07 &         -50.6 &            13.9 &             21.3 \\
 12 &  37.0143 &  61.3707 &  140 &         14.8 &          7.9 &  0.22 $^{+0.06}_{-0.05}$ &   25.4 &           4.5 &  14.8 $\pm$ 3.1 &  0.95 $\pm$ 0.12 &         -48.5 &            14.0 &             21.6 \\
 13 &  37.0152 &  61.4164 &  101 &         18.5 &         10.7 &  0.26 $^{+0.08}_{-0.12}$ &   74.0 &           7.7 &  15.7 $\pm$ 1.0 &   0.9 $\pm$ 0.04 &         -47.7 &            14.3 &             21.7 \\
 14 &  36.9407 &  61.4235 &  129 &         10.5 &          7.0 &  0.16 $^{+0.02}_{-0.03}$ &    9.5 &           1.8 &  16.0 $\pm$ 3.7 &   0.53 $\pm$ 0.1 &         -48.2 &            14.3 &             21.7 \\
 15 &  37.0146 &  61.4554 &   96 &         31.2 &         12.7 &   0.39 $^{+0.3}_{-0.15}$ &  333.6 &          83.4 &  16.0 $\pm$ 0.4 &  0.65 $\pm$ 0.01 &         -48.6 &            14.4 &             21.8 \\
 16 &  37.1458 &  61.4572 &  177 &         15.2 &          9.7 &  0.23 $^{+0.09}_{-0.06}$ &   15.7 &           5.3 &  23.2 $\pm$ 3.6 &  0.25 $\pm$ 0.05 &         -46.6 &            13.1 &             21.6 \\
 17 &  37.0260 &  61.4890 &  131 &         35.7 &         12.0 &    0.4 $^{+0.29}_{-0.2}$ &  374.8 &          80.6 &  16.1 $\pm$ 0.4 &  0.66 $\pm$ 0.01 &         -48.4 &            14.4 &             21.8 \\
 18 &  36.6832 &  61.4956 &  151 &         22.7 &         15.6 &   0.41 $^{+0.2}_{-0.08}$ &   66.4 &          29.1 &  12.2 $\pm$ 1.9 &   0.4 $\pm$ 0.04 &         -47.5 &            13.9 &             21.5 \\
 19 &  36.7455 &  61.4983 &  178 &         25.2 &         17.5 &  0.45 $^{+0.17}_{-0.11}$ &   97.3 &          37.0 &  13.3 $\pm$ 2.1 &  0.58 $\pm$ 0.06 &         -47.5 &            13.9 &             21.5 \\
 20 &  36.9543 &  61.5194 &  117 &         17.2 &          8.7 &   0.2 $^{+0.08}_{-0.16}$ &   12.6 &           1.7 &  17.4 $\pm$ 4.1 &  0.63 $\pm$ 0.13 &         -50.1 &            14.2 &             21.7 \\
 21 &  36.6824 &  61.5405 &  111 &         28.9 &         18.2 &  0.44 $^{+0.15}_{-0.15}$ &   60.2 &          19.0 &  13.3 $\pm$ 3.0 &  0.34 $\pm$ 0.06 &         -47.6 &            13.6 &             21.5 \\
 22 &  37.1072 &  61.5351 &  101 &         20.9 &         10.7 &  0.29 $^{+0.16}_{-0.09}$ &   61.6 &          12.3 &  18.8 $\pm$ 1.4 &  0.68 $\pm$ 0.04 &         -49.9 &            13.9 &             21.6 \\
 23 &  36.9769 &  61.5363 &  207 &         15.4 &          7.2 &  0.17 $^{+0.08}_{-0.07}$ &    9.9 &           0.4 &  17.2 $\pm$ 3.6 &  0.26 $\pm$ 0.06 &         -50.3 &            13.9 &             21.7 \\
 24 &  37.2483 &  61.5560 &  152 &         15.2 &         11.7 &  0.29 $^{+0.06}_{-0.05}$ &   24.0 &          10.5 &  19.9 $\pm$ 2.4 &  0.43 $\pm$ 0.05 &         -51.3 &            13.9 &             21.2 \\
 25 &  36.8599 &  61.5586 &   91 &         14.1 &          9.9 &   0.2 $^{+0.04}_{-0.11}$ &   14.2 &           2.2 &  15.6 $\pm$ 3.1 &  0.44 $\pm$ 0.07 &         -49.6 &            13.9 &             21.6 \\
 26 &  36.8319 &  61.5727 &  199 &         19.5 &         10.9 &   0.29 $^{+0.09}_{-0.1}$ &   29.4 &           5.6 &  15.9 $\pm$ 3.0 &  0.45 $\pm$ 0.07 &         -49.6 &            13.6 &             21.5 \\
 27 &  36.7580 &  61.5883 &  184 &         31.0 &         13.2 &   0.33 $^{+0.27}_{-0.2}$ &   33.4 &           6.9 &  13.3 $\pm$ 3.5 &  0.27 $\pm$ 0.05 &         -47.0 &            13.7 &             21.5 \\
 28 &  36.8128 &  61.5898 &   63 &         10.8 &          8.1 &  0.18 $^{+0.01}_{-0.07}$ &   10.7 &           1.2 &  16.1 $\pm$ 3.8 &   0.2 $\pm$ 0.05 &         -49.4 &            13.6 &             21.5 \\
 29 &  36.7663 &  61.6091 &  145 &         16.6 &          5.2 &  0.17 $^{+0.12}_{-0.07}$ &   10.4 &           1.4 &  14.3 $\pm$ 4.0 &  0.36 $\pm$ 0.08 &         -49.6 &            14.0 &             21.5 \\
 30 &  36.6247 &  61.6225 &   90 &         14.5 &          8.8 &  0.22 $^{+0.05}_{-0.09}$ &   12.5 &           1.6 &  11.7 $\pm$ 3.2 &  0.35 $\pm$ 0.06 &         -46.0 &            13.9 &             21.4 \\
 31 &  36.6671 &  61.6776 &   64 &         28.5 &         13.4 &  0.36 $^{+0.23}_{-0.21}$ &   47.3 &          15.0 &  15.8 $\pm$ 3.3 &  0.54 $\pm$ 0.09 &         -46.9 &            13.4 &             21.4 \\
 32 &  36.7546 &  61.8260 &  119 &         20.8 &         13.3 &   0.3 $^{+0.15}_{-0.16}$ &   34.7 &           7.7 &  17.5 $\pm$ 3.0 &   0.7 $\pm$ 0.09 &         -47.7 &            14.1 &             21.5 \\
 33 &  36.0531 &  61.8251 &   93 &         13.9 &         11.2 &  0.26 $^{+0.06}_{-0.05}$ &   13.3 &           5.0 &  11.9 $\pm$ 2.5 &  0.22 $\pm$ 0.03 &         -43.8 &            13.9 &             21.2 \\
 34 &  36.7332 &  61.8404 &  162 &         14.1 &          7.2 &  0.18 $^{+0.06}_{-0.05}$ &   14.9 &           3.5 &  17.0 $\pm$ 2.9 &  0.85 $\pm$ 0.12 &         -47.9 &            14.0 &             21.5 \\
 35 &  35.8751 &  61.8562 &  221 &         20.8 &         12.6 &  0.36 $^{+0.12}_{-0.09}$ &   37.6 &          16.6 &  15.4 $\pm$ 1.9 &   0.3 $\pm$ 0.04 &         -43.0 &            13.8 &             21.3 \\
 36 &  36.7611 &  61.8690 &   67 &         22.1 &         15.5 &  0.38 $^{+0.06}_{-0.04}$ &  273.1 &         105.3 &  28.5 $\pm$ 0.8 &  1.13 $\pm$ 0.03 &         -46.7 &            14.3 &             21.6 \\
 37 &  35.9743 &  61.8680 &  210 &         15.1 &         10.5 &  0.25 $^{+0.04}_{-0.07}$ &   18.4 &           4.4 &  13.2 $\pm$ 2.9 &   0.3 $\pm$ 0.05 &         -41.9 &            13.8 &             21.3 \\
 38 &  36.7951 &  61.8824 &  149 &         21.1 &         10.6 &  0.28 $^{+0.19}_{-0.09}$ &  108.6 &          32.7 &  24.0 $\pm$ 0.9 &   1.0 $\pm$ 0.03 &         -48.6 &            14.3 &             21.6 \\
 39 &  35.8095 &  61.8925 &   83 &         15.3 &          8.9 &   0.2 $^{+0.08}_{-0.16}$ &    8.2 &           1.9 &  14.7 $\pm$ 4.2 &  0.25 $\pm$ 0.06 &         -42.9 &            13.8 &             21.3 \\
 40 &  36.7496 &  61.9087 &   78 &         27.2 &          9.9 &  0.33 $^{+0.24}_{-0.12}$ &   64.4 &          21.0 &  19.3 $\pm$ 1.6 &  0.46 $\pm$ 0.04 &         -45.1 &            13.9 &             21.6 \\
 41 &  34.5379 &  61.9100 &  189 &         29.4 &         20.8 &  0.55 $^{+0.27}_{-0.18}$ &  123.0 &          71.4 &  12.8 $\pm$ 1.2 &  0.33 $\pm$ 0.02 &         -41.9 &            14.3 &             21.3 \\
 42 &  35.8087 &  61.9139 &  225 &         13.3 &          9.8 &  0.24 $^{+0.03}_{-0.02}$ &   16.5 &           2.6 &  14.0 $\pm$ 1.9 &  0.34 $\pm$ 0.04 &         -43.5 &            14.1 &             21.4 \\
 43 &  34.6511 &  61.9054 &  203 &         13.2 &          5.7 &  0.17 $^{+0.07}_{-0.04}$ &   19.8 &           3.9 &  12.1 $\pm$ 0.6 &  0.31 $\pm$ 0.01 &         -43.2 &            14.4 &             21.3 \\
 44 &  34.6179 &  61.9053 &  153 &         10.5 &          7.3 &  0.17 $^{+0.01}_{-0.03}$ &   21.1 &           4.4 &  12.5 $\pm$ 0.6 &  0.33 $\pm$ 0.01 &         -43.0 &            14.3 &             21.3 \\
 45 &  36.8435 &  61.9302 &  169 &         25.0 &         20.2 &  0.39 $^{+0.18}_{-0.26}$ &   61.4 &          17.1 &  20.5 $\pm$ 3.1 &  0.47 $\pm$ 0.07 &         -48.5 &            13.6 &             21.5 \\
 46 &  36.3685 &  61.9374 &   73 &         25.1 &         13.7 &  0.39 $^{+0.19}_{-0.13}$ &   57.3 &          28.4 &  18.3 $\pm$ 2.0 &  0.32 $\pm$ 0.04 &         -43.1 &            13.8 &             21.3 \\
 47 &  35.8053 &  61.9307 &   62 &         12.0 &          9.6 &   0.2 $^{+0.04}_{-0.07}$ &   17.0 &           2.5 &  14.4 $\pm$ 2.6 &  0.75 $\pm$ 0.09 &         -42.9 &            14.3 &             21.4 \\
 48 &  35.8327 &  61.9406 &  141 &         15.6 &          8.7 &  0.24 $^{+0.05}_{-0.03}$ &   24.9 &           4.3 &  13.5 $\pm$ 1.9 &  0.34 $\pm$ 0.04 &         -42.1 &            14.2 &             21.4 \\
 49 &  36.8202 &  61.9505 &  100 &         18.7 &         16.8 &   0.3 $^{+0.11}_{-0.24}$ &   38.2 &           9.2 &  19.9 $\pm$ 3.2 &   0.68 $\pm$ 0.1 &         -48.1 &            14.0 &             21.5 \\
 50 &  35.7930 &  61.9571 &   77 &         14.6 &         10.5 &  0.27 $^{+0.07}_{-0.04}$ &   22.6 &           4.1 &  12.0 $\pm$ 1.8 &  0.35 $\pm$ 0.04 &         -43.6 &            14.3 &             21.4 \\
 51 &  36.7123 &  61.9662 &  142 &         14.5 &         11.1 &   0.28 $^{+0.1}_{-0.03}$ &   34.9 &          16.9 &  23.2 $\pm$ 2.8 &  0.62 $\pm$ 0.07 &         -44.2 &            13.7 &             21.5 \\
 52 &  36.4833 &  61.9684 &  143 &         12.2 &          9.0 &  0.22 $^{+0.05}_{-0.02}$ &   13.0 &           3.8 &  20.3 $\pm$ 2.8 &  0.55 $\pm$ 0.07 &         -37.5 &            13.9 &             21.3 \\
 53 &  36.7786 &  61.9715 &   81 &         12.6 &          5.8 &  0.17 $^{+0.11}_{-0.05}$ &    9.4 &           1.0 &  16.7 $\pm$ 3.5 &  0.27 $\pm$ 0.05 &         -46.9 &            13.7 &             21.4 \\
 54 &  35.7822 &  61.9754 &   88 &         12.2 &          9.7 &  0.23 $^{+0.06}_{-0.02}$ &   20.6 &           3.2 &  14.9 $\pm$ 2.2 &  0.31 $\pm$ 0.04 &         -43.3 &            13.9 &             21.4 \\
 55 &  35.7194 &  61.9775 &  139 &         10.4 &          9.0 &    0.2 $^{+0.0}_{-0.01}$ &   11.7 &           2.1 &  15.6 $\pm$ 2.7 &  0.23 $\pm$ 0.04 &         -43.4 &            13.7 &             21.3 \\
 56 &  35.6635 &  61.9823 &   48 &         11.9 &          7.6 &  0.19 $^{+0.02}_{-0.05}$ &   10.3 &           1.0 &  12.7 $\pm$ 3.2 &   0.3 $\pm$ 0.06 &         -42.3 &            14.1 &             21.3 \\
 57 &  35.9207 &  61.9880 &  175 &         11.7 &          8.6 &   0.2 $^{+0.04}_{-0.04}$ &   11.6 &           1.1 &  15.5 $\pm$ 3.1 &  0.21 $\pm$ 0.04 &         -40.5 &            14.0 &             21.3 \\
 58 &  35.7525 &  61.9911 &  184 &         16.9 &         13.9 &  0.35 $^{+0.06}_{-0.04}$ &   45.2 &          14.3 &  12.4 $\pm$ 1.6 &  0.36 $\pm$ 0.03 &         -43.6 &            14.2 &             21.3 \\
 59 &  35.5528 &  62.0052 &   59 &         15.1 &         11.8 &  0.29 $^{+0.02}_{-0.05}$ &   21.8 &           5.5 &  12.9 $\pm$ 2.1 &  0.22 $\pm$ 0.03 &         -42.9 &            14.1 &             21.3 \\
 60 &  35.8011 &  62.0093 &   45 &         11.1 &          6.0 &  0.17 $^{+0.03}_{-0.07}$ &    7.4 &           1.1 &  18.1 $\pm$ 3.7 &  0.22 $\pm$ 0.04 &         -43.1 &            14.2 &             21.3 \\
 61 &  35.4334 &  62.0133 &  183 &         22.8 &         13.7 &  0.43 $^{+0.15}_{-0.11}$ &   61.5 &          31.3 &  13.2 $\pm$ 1.1 &  0.23 $\pm$ 0.02 &         -43.7 &            14.2 &             21.2 \\
 62 &  35.3379 &  62.0289 &   68 &         21.3 &         13.8 &  0.33 $^{+0.11}_{-0.14}$ &   34.4 &           9.5 &  14.9 $\pm$ 2.2 &  0.23 $\pm$ 0.03 &         -43.3 &            13.8 &             21.2 \\
 63 &  35.3035 &  62.0257 &  172 &         14.1 &          5.3 &  0.16 $^{+0.06}_{-0.07}$ &    7.4 &           0.6 &  11.7 $\pm$ 3.5 &  0.36 $\pm$ 0.07 &         -43.9 &            13.7 &             21.2 \\
 64 &  36.5114 &  62.0431 &   82 &         10.4 &          8.6 &  0.18 $^{+0.02}_{-0.05}$ &    9.1 &           2.2 &  19.8 $\pm$ 3.9 &   0.58 $\pm$ 0.1 &         -38.3 &            14.0 &             21.5 \\
 65 &  36.1253 &  62.0582 &  199 &         17.4 &         10.8 &  0.29 $^{+0.16}_{-0.08}$ &   23.5 &          10.7 &  16.2 $\pm$ 2.5 &  0.41 $\pm$ 0.05 &         -39.7 &            14.2 &             21.3 \\
 66 &  36.5332 &  62.0660 &  141 &         28.8 &         10.3 &  0.29 $^{+0.25}_{-0.22}$ &   27.0 &           6.0 &  17.6 $\pm$ 3.1 &  0.62 $\pm$ 0.09 &         -39.0 &            14.0 &             21.5 \\
 67 &  36.4711 &  62.0714 &  196 &         21.4 &         16.8 &   0.48 $^{+0.13}_{-0.1}$ &  147.7 &          94.3 &  22.0 $\pm$ 1.1 &  0.71 $\pm$ 0.03 &         -38.7 &            14.2 &             21.5 \\
 68 &  36.0825 &  62.0695 &  188 &         13.0 &          7.6 &   0.2 $^{+0.07}_{-0.05}$ &    7.2 &           2.4 &  15.7 $\pm$ 2.8 &  0.22 $\pm$ 0.04 &         -40.4 &            14.0 &             21.3 \\
 69 &  36.6070 &  62.0885 &  121 &         50.3 &         18.6 &  0.65 $^{+0.44}_{-0.33}$ &  194.5 &         110.3 &  19.8 $\pm$ 2.2 &  0.65 $\pm$ 0.06 &         -39.3 &            13.7 &             21.5 \\
 70 &  36.0297 &  62.0763 &  119 &         12.2 &         10.7 &  0.24 $^{+0.03}_{-0.03}$ &   11.0 &           4.6 &  15.1 $\pm$ 2.6 &  0.26 $\pm$ 0.04 &         -41.0 &            13.8 &             21.2 \\
 71 &  36.2424 &  62.0819 &  152 &         28.3 &         12.3 &  0.39 $^{+0.32}_{-0.14}$ &   62.1 &          27.3 &  15.3 $\pm$ 1.5 &  0.39 $\pm$ 0.03 &         -39.6 &            14.0 &             21.4 \\
 72 &  36.2950 &  62.0867 &  179 &         16.7 &         12.8 &  0.26 $^{+0.07}_{-0.13}$ &   23.1 &           4.9 &  17.4 $\pm$ 2.5 &  0.43 $\pm$ 0.06 &         -40.0 &            13.5 &             21.5 \\
 73 &  36.4663 &  62.1018 &   79 &         23.5 &         16.4 &  0.36 $^{+0.19}_{-0.13}$ &   44.3 &          20.9 &  27.4 $\pm$ 4.5 &  0.75 $\pm$ 0.11 &         -38.6 &            13.9 &             21.5 \\
 74 &  36.3712 &  62.0998 &  155 &         18.2 &         16.5 &  0.39 $^{+0.08}_{-0.12}$ &  276.9 &         237.4 &  36.0 $\pm$ 1.2 &  1.11 $\pm$ 0.03 &         -42.5 &            14.2 &             21.5 \\
 75 &  36.3907 &  62.1127 &   56 &         11.5 &          5.8 &  0.16 $^{+0.06}_{-0.04}$ &   18.5 &           9.5 &  34.6 $\pm$ 3.3 &  0.64 $\pm$ 0.06 &         -45.9 &            13.6 &             21.5 \\
 76 &  36.4645 &  62.1372 &   75 &         14.1 &          9.7 &  0.25 $^{+0.06}_{-0.06}$ &   21.3 &           7.7 &  16.6 $\pm$ 2.3 &  0.34 $\pm$ 0.04 &         -38.1 &            14.2 &             21.5 \\
 77 &  36.5105 &  62.1454 &   90 &         25.7 &         21.1 &   0.48 $^{+0.23}_{-0.2}$ &  111.7 &          48.2 &  20.5 $\pm$ 2.4 &  0.61 $\pm$ 0.06 &         -39.7 &            13.9 &             21.5 \\
 78 &  36.6952 &  62.1448 &  170 &         10.9 &          6.5 &  0.17 $^{+0.02}_{-0.01}$ &    7.6 &           0.7 &  16.4 $\pm$ 2.8 &  0.57 $\pm$ 0.08 &         -38.4 &            13.9 &             21.3 \\
 79 &  36.4921 &  62.1713 &  200 &         18.9 &         11.0 &   0.26 $^{+0.1}_{-0.17}$ &   24.6 &           5.2 &  16.8 $\pm$ 3.1 &  0.52 $\pm$ 0.08 &         -41.7 &            14.2 &             21.5 \\
 80 &  36.5694 &  62.1907 &  134 &         24.7 &         11.8 &  0.29 $^{+0.19}_{-0.22}$ &   31.8 &           9.3 &  19.1 $\pm$ 2.9 &  0.57 $\pm$ 0.08 &         -40.7 &            13.6 &             21.4 \\
 81 &  36.5571 &  62.2009 &  138 &         14.8 &          8.2 &   0.19 $^{+0.1}_{-0.07}$ &   15.6 &           1.6 &  18.1 $\pm$ 4.8 &   0.93 $\pm$ 0.2 &         -41.3 &            13.9 &             21.4 \\
 82 &  36.5664 &  62.2188 &  157 &         21.8 &          7.9 &  0.23 $^{+0.19}_{-0.15}$ &   17.2 &           2.9 &  15.3 $\pm$ 3.5 &   0.62 $\pm$ 0.1 &         -42.0 &            14.2 &             21.3 \\
 83 &  36.6769 &  62.2462 &   89 &         13.6 &          9.5 &    0.2 $^{+0.1}_{-0.06}$ &    7.2 &           0.6 &  17.6 $\pm$ 3.6 &  0.38 $\pm$ 0.07 &         -43.0 &            14.1 &             21.2 \\
\bottomrule
\end{tabular}


==> W3_leaf_stats_virial.tex <==
\begin{tabular}{rrrrrrrrllrr}
\toprule
 ID &  $\alpha_{vir}$ &  $M_{vir}$ &  $\sigma_{nt}$ & log$|\Omega_G|$ & log$\Omega_K$ & log$|\Omega_{Pw}|$ &  log$|\Omega_{Pt}|$ & on-filament & hub & $N_{proto}$ & Bad N(H$_2$) Pixels \\& & (M$_\odot$) & (km s$^{-1}$) & (erg) & (erg) & (erg) & (erg) & & & \\\midrule
  0 &   1.77 &              12.6 &      0.18 &  43.2 &     43.2 &     43.4 &         NaN &         True &  False &           0 &      0.00 \\
  1 &   1.19 &              31.5 &      0.24 &  44.0 &     43.9 &     44.3 &         NaN &         True &  False &           0 &      0.00 \\
  2 &   1.39 &              35.0 &      0.31 &  44.1 &     44.0 &     44.1 &         NaN &         True &  False &           0 &      0.00 \\
  3 &   5.13 &              89.2 &      0.57 &  43.8 &     44.3 &     44.0 &         NaN &         True &  False &           0 &      0.00 \\
  4 &   4.15 &             108.9 &      0.59 &  44.1 &     44.5 &     44.3 &         NaN &        False &  False &           1 &      0.00 \\
  5 &   0.48 &             141.1 &      0.38 &  45.8 &     45.2 &     45.6 &         NaN &        False &   True &           6 &      0.00 \\
  6 &  11.61 &              94.2 &      0.74 &  43.3 &     44.2 &     43.5 &         NaN &        False &  False &           0 &      0.00 \\
  7 &   0.83 &              68.1 &      0.35 &  44.9 &     44.6 &     44.8 &         NaN &        False &  False &           1 &      0.00 \\
  8 &   5.25 &             130.9 &      0.73 &  44.1 &     44.6 &     44.0 &         NaN &        False &  False &           1 &      0.00 \\
  9 &   0.80 &              32.0 &      0.23 &  44.4 &     44.1 &     44.5 &         NaN &        False &  False &           3 &      0.00 \\
 10 &   2.37 &              33.9 &      0.34 &  43.7 &     43.8 &     43.9 &         NaN &        False &  False &           0 &      0.00 \\
 11 &   2.68 &              57.4 &      0.41 &  44.0 &     44.2 &     44.0 &         NaN &        False &  False &           2 &      0.00 \\
 12 &   7.61 &             193.8 &      0.94 &  44.2 &     44.9 &     44.0 &         NaN &         True &  False &           0 &      0.00 \\
 13 &   2.82 &             208.5 &      0.90 &  45.0 &     45.3 &     44.4 &         NaN &         True &  False &           0 &      0.00 \\
 14 &   5.23 &              49.6 &      0.53 &  43.5 &     44.0 &     43.8 &         NaN &         True &  False &           0 &      0.00 \\
 15 &   0.51 &             169.4 &      0.65 &  46.2 &     45.7 &     45.0 &         NaN &        False &   True &           4 &      0.00 \\
 16 &   1.86 &              29.2 &      0.23 &  43.7 &     43.8 &     44.2 &         NaN &         True &  False &           1 &      0.00 \\
 17 &   0.48 &             181.2 &      0.66 &  46.3 &     45.7 &     45.0 &         NaN &        False &   True &           9 &      0.00 \\
 18 &   1.15 &              76.1 &      0.39 &  44.7 &     44.6 &     44.8 &         NaN &        False &  False &           1 &      0.00 \\
 19 &   1.62 &             157.2 &      0.57 &  45.0 &     45.0 &     44.9 &         NaN &        False &  False &           1 &      0.00 \\
 20 &   6.62 &              83.7 &      0.63 &  43.6 &     44.2 &     44.1 &         NaN &        False &  False &           0 &      0.00 \\
 21 &   1.07 &              64.2 &      0.33 &  44.6 &     44.5 &     44.8 &         NaN &        False &  False &           0 &      0.00 \\
 22 &   2.28 &             140.8 &      0.68 &  44.8 &     45.0 &     44.5 &         NaN &         True &  False &           0 &      0.00 \\
 23 &   1.87 &              18.4 &      0.24 &  43.5 &     43.5 &     43.8 &         NaN &        False &  False &           1 &      0.00 \\
 24 &   2.79 &              66.8 &      0.42 &  44.0 &     44.3 &     44.1 &         NaN &         True &  False &           1 &      0.00 \\
 25 &   3.16 &              44.8 &      0.43 &  43.7 &     44.0 &     43.9 &         NaN &         True &  False &           2 &      0.00 \\
 26 &   2.31 &              67.9 &      0.44 &  44.2 &     44.3 &     44.4 &         NaN &         True &  False &           1 &      0.00 \\
 27 &   1.02 &              34.0 &      0.26 &  44.2 &     44.0 &     44.5 &         NaN &         True &  False &           1 &      0.00 \\
 28 &   1.41 &              15.0 &      0.18 &  43.5 &     43.5 &     43.7 &         NaN &         True &  False &           0 &      0.00 \\
 29 &   2.53 &              26.3 &      0.35 &  43.5 &     43.7 &     43.6 &         NaN &         True &  False &           0 &      0.00 \\
 30 &   2.57 &              32.0 &      0.34 &  43.6 &     43.8 &     43.8 &         NaN &         True &  False &           0 &      0.00 \\
 31 &   2.35 &             111.3 &      0.53 &  44.5 &     44.7 &     44.5 &         NaN &        False &  False &           0 &      0.00 \\
 32 &   4.42 &             153.4 &      0.70 &  44.3 &     44.8 &     44.4 &        45.7 &        False &  False &           0 &      0.00 \\
 33 &   1.53 &              20.4 &      0.20 &  43.5 &     43.5 &     43.9 &         NaN &         True &  False &           0 &      0.00 \\
 34 &   8.72 &             129.7 &      0.85 &  43.8 &     44.5 &     43.8 &        46.1 &        False &  False &           0 &      0.00 \\
 35 &   1.20 &              45.3 &      0.29 &  44.3 &     44.2 &     44.4 &         NaN &         True &  False &           2 &      0.00 \\
 36 &   1.78 &             486.9 &      1.13 &  46.0 &     46.0 &     44.8 &        46.6 &        False &  False &           0 &      0.08 \\
 37 &   1.70 &              31.2 &      0.29 &  43.8 &     43.9 &     44.0 &         NaN &         True &  False &           0 &      0.00 \\
 38 &   2.53 &             274.3 &      0.99 &  45.3 &     45.5 &     44.3 &         NaN &        False &  False &           3 &      0.00 \\
 39 &   2.41 &              19.8 &      0.23 &  43.2 &     43.4 &     43.7 &         NaN &         True &  False &           0 &      0.00 \\
 40 &   1.28 &              82.2 &      0.45 &  44.8 &     44.7 &     44.6 &        45.8 &         True &  False &           1 &      0.00 \\
 41 &   0.61 &              74.6 &      0.32 &  45.1 &     44.7 &     45.0 &         NaN &         True &  False &           2 &      0.00 \\
 42 &   2.09 &              34.5 &      0.33 &  43.8 &     43.9 &     43.9 &         NaN &         True &  False &           0 &      0.00 \\
 43 &   1.03 &              20.3 &      0.30 &  44.1 &     43.9 &     43.4 &         NaN &         True &  False &           0 &      0.00 \\
 44 &   1.15 &              24.2 &      0.32 &  44.1 &     44.0 &     43.5 &         NaN &         True &  False &           0 &      0.00 \\
 45 &   1.66 &             101.7 &      0.46 &  44.7 &     44.7 &     44.7 &         NaN &         True &  False &           0 &      0.00 \\
 46 &   0.98 &              56.0 &      0.30 &  44.6 &     44.4 &     44.5 &         NaN &         True &  False &           4 &      0.00 \\
 47 &   6.53 &             111.0 &      0.74 &  43.9 &     44.5 &     43.7 &         NaN &         True &  False &           0 &      0.00 \\
 48 &   1.38 &              34.2 &      0.33 &  44.1 &     44.1 &     43.9 &         NaN &         True &  False &           1 &      0.00 \\
 49 &   3.88 &             148.4 &      0.67 &  44.4 &     44.8 &     44.4 &         NaN &         True &  False &           0 &      0.00 \\
 50 &   1.75 &              39.5 &      0.34 &  44.0 &     44.0 &     44.1 &         NaN &         True &  False &           0 &      0.00 \\
 51 &   3.43 &             119.8 &      0.61 &  44.3 &     44.7 &     44.3 &         NaN &         True &  False &           2 &      0.00 \\
 52 &   5.80 &              75.4 &      0.54 &  43.6 &     44.2 &     43.8 &         NaN &        False &  False &           0 &      0.00 \\
 53 &   2.06 &              19.5 &      0.26 &  43.4 &     43.5 &     43.6 &         NaN &         True &  False &           0 &      0.00 \\
 54 &   1.42 &              29.1 &      0.29 &  44.0 &     43.9 &     43.9 &         NaN &         True &  False &           2 &      0.00 \\
 55 &   1.58 &              18.4 &      0.21 &  43.5 &     43.5 &     43.7 &         NaN &         True &  False &           0 &      0.00 \\
 56 &   2.17 &              22.4 &      0.29 &  43.5 &     43.6 &     43.6 &         NaN &         True &  False &           0 &      0.00 \\
 57 &   1.51 &              17.6 &      0.19 &  43.5 &     43.5 &     43.7 &         NaN &        False &  False &           0 &      0.00 \\
 58 &   1.19 &              53.8 &      0.35 &  44.5 &     44.4 &     44.4 &         NaN &         True &  False &           1 &      0.00 \\
 59 &   1.10 &              23.9 &      0.21 &  43.9 &     43.8 &     44.1 &         NaN &         True &  False &           0 &      0.00 \\
 60 &   2.21 &              16.4 &      0.20 &  43.2 &     43.4 &     43.4 &         NaN &         True &  False &           0 &      0.00 \\
 61 &   0.61 &              37.5 &      0.22 &  44.7 &     44.2 &     44.6 &         NaN &         True &  False &           1 &      0.00 \\
 62 &   0.87 &              30.0 &      0.21 &  44.3 &     44.0 &     44.3 &         NaN &         True &  False &           0 &      0.00 \\
 63 &   3.29 &              24.3 &      0.35 &  43.2 &     43.6 &     43.3 &         NaN &         True &  False &           0 &      0.00 \\
 64 &   7.32 &              67.0 &      0.57 &  43.4 &     44.0 &     43.7 &         NaN &        False &  False &           0 &      0.00 \\
 65 &   2.46 &              57.9 &      0.40 &  44.0 &     44.2 &     44.1 &         NaN &        False &  False &           1 &      0.00 \\
 66 &   4.46 &             120.4 &      0.62 &  44.1 &     44.6 &     44.3 &        45.9 &        False &  False &           0 &      0.00 \\
 67 &   1.73 &             254.9 &      0.70 &  45.4 &     45.4 &     45.0 &        47.0 &        False &  False &           1 &      0.00 \\
 68 &   2.46 &              17.7 &      0.20 &  43.1 &     43.3 &     43.6 &         NaN &        False &  False &           0 &      0.00 \\
 69 &   1.52 &             296.4 &      0.65 &  45.5 &     45.5 &     45.4 &        46.9 &         True &  False &           3 &      0.00 \\
 70 &   2.29 &              25.2 &      0.25 &  43.4 &     43.6 &     43.8 &         NaN &        False &  False &           0 &      0.00 \\
 71 &   1.15 &              71.3 &      0.38 &  44.7 &     44.6 &     44.6 &         NaN &        False &  False &           3 &      0.00 \\
 72 &   2.52 &              58.2 &      0.42 &  44.0 &     44.2 &     44.2 &         NaN &        False &  False &           0 &      0.00 \\
 73 &   4.84 &             214.6 &      0.74 &  44.4 &     44.9 &     44.7 &        46.2 &         True &  False &           0 &      0.00 \\
 74 &   1.74 &             483.0 &      1.10 &  46.0 &     46.0 &     44.7 &        46.8 &        False &  False &           3 &      0.14 \\
 75 &   4.12 &              76.3 &      0.63 &  44.0 &     44.5 &     43.6 &         NaN &        False &  False &           0 &      0.00 \\
 76 &   1.83 &              39.0 &      0.33 &  44.0 &     44.0 &     44.2 &        45.8 &         True &  False &           0 &      0.00 \\
 77 &   1.73 &             193.1 &      0.60 &  45.1 &     45.2 &     45.0 &        46.4 &         True &  False &           2 &      0.00 \\
 78 &   7.84 &              59.6 &      0.56 &  43.2 &     43.9 &     43.5 &         NaN &         True &  False &           0 &      0.00 \\
 79 &   3.19 &              78.4 &      0.51 &  44.1 &     44.4 &     44.2 &        45.7 &         True &  False &           0 &      0.00 \\
 80 &   3.28 &             104.3 &      0.56 &  44.2 &     44.6 &     44.2 &         NaN &         True &  False &           0 &      0.00 \\
 81 &  10.63 &             165.9 &      0.93 &  43.8 &     44.6 &     43.7 &         NaN &         True &  False &           0 &      0.00 \\
 82 &   5.46 &              93.7 &      0.62 &  43.8 &     44.3 &     43.9 &         NaN &         True &  False &           0 &      0.00 \\
 83 &   5.19 &              37.2 &      0.37 &  43.1 &     43.6 &     43.6 &         NaN &         True &  False &           0 &      0.00 \\
\bottomrule
\end{tabular}


==> W48_leaf_stats.tex <==
\begin{tabular}{rrrrrrlrrllrrr}
\toprule
ID & RA & decl. & PA & $\sigma_{major}$ & $\sigma_{minor}$ &  $R_{eff}$ &  $M_{obs}$ &  $M_{clip}$ &  $T_K$ &  $\sigma_{NH_3}$ &  $V_{LSR, NH_3}$ &  log($N_{para-NH_3}$) &  log($N_{H_2}$) \\& (deg) & (deg) & (deg) & ($\arcsec$) & ($\arcsec$) & (pc) & (M$_\odot$) & (M$_\odot$) & (K) & (km s$^{-1}$) & (km s$^{-1}$) & (cm$^{-2}$) & (cm$^{-2}$) \\\midrule
  0 &  284.7530 &  0.9409 &   64 &         16.5 &          9.5 &    0.35 $^{+0.07}_{-0.2}$ &   126.4 &          23.8 &  12.6 $\pm$ 2.9 &  0.28 $\pm$ 0.05 &          47.6 &            14.3 &             21.9 \\
  1 &  284.8809 &  0.9637 &  109 &         20.4 &         11.5 &   0.34 $^{+0.21}_{-0.26}$ &    96.6 &          14.5 &  13.5 $\pm$ 2.9 &   0.66 $\pm$ 0.1 &          45.4 &            13.8 &             22.0 \\
  2 &  284.7698 &  0.9709 &  194 &         18.5 &         11.3 &   0.46 $^{+0.19}_{-0.19}$ &   120.3 &          22.5 &  13.8 $\pm$ 2.1 &  0.33 $\pm$ 0.04 &          47.1 &            14.2 &             21.9 \\
  3 &  284.9213 &  0.9851 &  147 &         30.3 &         14.9 &   0.68 $^{+0.51}_{-0.16}$ &  1000.5 &         374.7 &  14.8 $\pm$ 0.3 &  0.66 $\pm$ 0.01 &          45.6 &            14.7 &             22.0 \\
  4 &  285.0465 &  0.9835 &   71 &         11.9 &          9.0 &   0.31 $^{+0.03}_{-0.02}$ &    80.1 &          10.2 &  13.5 $\pm$ 0.7 &  0.37 $\pm$ 0.02 &          43.2 &            14.4 &             21.9 \\
  5 &  285.0422 &  0.9984 &   91 &         11.5 &          6.8 &   0.24 $^{+0.08}_{-0.04}$ &    59.9 &           5.0 &  14.0 $\pm$ 1.1 &  0.63 $\pm$ 0.04 &          42.9 &            14.2 &             21.9 \\
  6 &  284.9416 &  1.0159 &  186 &         30.8 &         24.9 &   0.85 $^{+0.36}_{-0.18}$ &  1888.7 &         942.6 &  16.2 $\pm$ 0.4 &  0.67 $\pm$ 0.01 &          46.0 &            14.6 &             22.0 \\
  7 &  285.0214 &  1.0089 &  201 &         12.3 &          9.1 &    0.29 $^{+0.1}_{-0.06}$ &    56.1 &          16.7 &  16.3 $\pm$ 2.7 &   0.5 $\pm$ 0.07 &          41.1 &            13.3 &             21.9 \\
  8 &  284.8016 &  1.0532 &  167 &         25.6 &         11.4 &   0.55 $^{+0.43}_{-0.18}$ &   182.7 &          45.4 &  13.2 $\pm$ 1.9 &  0.33 $\pm$ 0.04 &          46.1 &            14.1 &             21.9 \\
  9 &  284.8671 &  1.0730 &   54 &         40.1 &         23.0 &   0.96 $^{+0.78}_{-0.45}$ &   778.4 &         281.5 &  13.0 $\pm$ 1.4 &  0.38 $\pm$ 0.03 &          41.8 &            14.1 &             21.9 \\
 10 &  284.8538 &  1.1006 &  222 &         10.9 &          7.5 &   0.24 $^{+0.06}_{-0.07}$ &    45.4 &           2.4 &  12.9 $\pm$ 3.7 &  0.49 $\pm$ 0.09 &          41.8 &            13.8 &             21.9 \\
 11 &  285.1903 &  1.1140 &  155 &         18.9 &         12.4 &   0.43 $^{+0.26}_{-0.18}$ &   153.0 &          18.0 &  12.3 $\pm$ 3.0 &  0.31 $\pm$ 0.06 &          37.0 &            13.9 &             21.9 \\
 12 &  284.8044 &  1.1276 &  206 &         16.0 &         14.5 &   0.44 $^{+0.16}_{-0.24}$ &   130.6 &          20.1 &  10.5 $\pm$ 2.7 &  0.24 $\pm$ 0.04 &          41.8 &            14.0 &             21.9 \\
 13 &  285.3979 &  1.1357 &  123 &         24.5 &         10.9 &   0.48 $^{+0.36}_{-0.17}$ &   166.6 &          51.5 &  14.3 $\pm$ 2.1 &  0.27 $\pm$ 0.04 &          42.1 &            13.7 &             21.9 \\
 14 &  285.3207 &  1.1310 &  119 &         20.2 &          9.5 &   0.35 $^{+0.22}_{-0.18}$ &    95.5 &          11.3 &  14.8 $\pm$ 2.9 &  0.65 $\pm$ 0.09 &          42.5 &            13.8 &             21.9 \\
 15 &  284.8362 &  1.1283 &  223 &         14.2 &         10.4 &   0.38 $^{+0.08}_{-0.03}$ &   174.6 &          40.6 &  12.1 $\pm$ 0.8 &  0.42 $\pm$ 0.02 &          41.6 &            14.3 &             21.9 \\
 16 &  285.2771 &  1.1536 &  224 &         37.9 &         21.9 &   0.87 $^{+0.39}_{-0.36}$ &   556.6 &         145.9 &  12.9 $\pm$ 1.4 &  0.27 $\pm$ 0.02 &          37.7 &            13.9 &             22.0 \\
 17 &  285.4633 &  1.1433 &   61 &         22.0 &         10.5 &   0.47 $^{+0.18}_{-0.15}$ &   158.7 &          33.0 &  13.5 $\pm$ 1.8 &  0.38 $\pm$ 0.04 &          43.7 &            13.9 &             21.8 \\
 18 &  284.8249 &  1.1388 &   88 &         10.0 &          8.2 &    0.27 $^{+0.0}_{-0.03}$ &    69.3 &           8.2 &  11.2 $\pm$ 1.0 &  0.33 $\pm$ 0.02 &          41.4 &            14.3 &             21.9 \\
 19 &  285.4410 &  1.1420 &  159 &         14.1 &          9.7 &   0.34 $^{+0.14}_{-0.11}$ &    62.9 &           7.9 &  12.4 $\pm$ 3.4 &  0.41 $\pm$ 0.07 &          43.6 &            14.0 &             21.8 \\
 20 &  285.3290 &  1.1483 &  205 &         16.0 &         15.1 &   0.43 $^{+0.12}_{-0.15}$ &   150.7 &          31.0 &  15.3 $\pm$ 2.6 &   0.6 $\pm$ 0.08 &          41.7 &            13.3 &             22.0 \\
 21 &  285.2546 &  1.1445 &  187 &         12.6 &         10.0 &    0.35 $^{+0.0}_{-0.06}$ &    71.7 &          11.6 &  11.8 $\pm$ 1.9 &  0.22 $\pm$ 0.03 &          38.3 &            13.8 &             21.9 \\
 22 &  284.8349 &  1.1628 &   94 &         25.4 &         16.6 &   0.67 $^{+0.27}_{-0.16}$ &   568.9 &         151.2 &  13.3 $\pm$ 1.2 &  0.48 $\pm$ 0.03 &          41.2 &            14.3 &             21.9 \\
 23 &  285.5849 &  1.1580 &  205 &         12.7 &         10.5 &   0.37 $^{+0.06}_{-0.02}$ &    51.9 &          10.1 &  10.3 $\pm$ 1.8 &  0.18 $\pm$ 0.02 &          38.6 &            14.2 &             21.4 \\
 24 &  285.4203 &  1.1711 &  173 &         12.5 &          8.3 &   0.29 $^{+0.12}_{-0.03}$ &    63.9 &          11.7 &  13.9 $\pm$ 2.2 &  1.11 $\pm$ 0.11 &          42.2 &            14.4 &             21.9 \\
 25 &  285.3549 &  1.1718 &  162 &         19.9 &         12.7 &   0.48 $^{+0.13}_{-0.11}$ &   285.4 &          71.9 &  14.8 $\pm$ 0.8 &  1.01 $\pm$ 0.04 &          41.3 &            14.5 &             22.0 \\
 26 &  285.3010 &  1.1760 &   62 &         17.3 &         13.5 &   0.46 $^{+0.14}_{-0.12}$ &   206.5 &          50.7 &  17.7 $\pm$ 2.0 &  0.39 $\pm$ 0.04 &          38.1 &            13.7 &             22.0 \\
 27 &  285.4056 &  1.1737 &  143 &         15.8 &          5.6 &   0.24 $^{+0.16}_{-0.09}$ &    50.8 &           2.6 &  15.4 $\pm$ 2.4 &  1.36 $\pm$ 0.14 &          41.7 &            13.6 &             21.9 \\
 28 &  285.4546 &  1.1762 &   60 &         12.1 &          9.5 &   0.33 $^{+0.03}_{-0.01}$ &   109.5 &          37.4 &  17.1 $\pm$ 0.7 &  0.39 $\pm$ 0.02 &          42.7 &            14.3 &             21.9 \\
 29 &  285.2489 &  1.1906 &  141 &         42.4 &         17.8 &   0.87 $^{+0.53}_{-0.33}$ &  1058.2 &         467.0 &  13.7 $\pm$ 0.9 &  0.81 $\pm$ 0.04 &          36.1 &            14.4 &             22.0 \\
 30 &  285.3356 &  1.1845 &  123 &         18.6 &         13.0 &   0.46 $^{+0.18}_{-0.09}$ &   278.2 &          49.3 &  14.6 $\pm$ 0.8 &  0.38 $\pm$ 0.02 &          41.4 &            14.2 &             22.0 \\
 31 &  285.1315 &  1.1853 &  176 &         22.4 &         12.3 &   0.49 $^{+0.26}_{-0.12}$ &   195.9 &          41.4 &  16.7 $\pm$ 2.7 &  0.59 $\pm$ 0.08 &          38.2 &            13.8 &             21.9 \\
 32 &  284.4067 &  1.1835 &  109 &         14.4 &          6.4 &   0.28 $^{+0.08}_{-0.09}$ &    53.3 &           3.1 &  16.1 $\pm$ 3.2 &  0.23 $\pm$ 0.04 &          46.7 &            13.8 &             21.9 \\
 33 &  285.3905 &  1.1846 &  204 &         13.2 &          7.7 &    0.3 $^{+0.09}_{-0.05}$ &   121.8 &          23.4 &  14.4 $\pm$ 0.5 &  0.38 $\pm$ 0.01 &          41.9 &            14.3 &             22.0 \\
 34 &  285.3705 &  1.1882 &  185 &         17.6 &         10.8 &    0.43 $^{+0.1}_{-0.06}$ &   312.9 &          90.0 &  14.7 $\pm$ 0.5 &  0.49 $\pm$ 0.01 &          41.6 &            14.4 &             22.0 \\
 35 &  285.1567 &  1.1863 &  175 &         16.8 &          8.1 &   0.31 $^{+0.14}_{-0.19}$ &    63.7 &           5.0 &  15.6 $\pm$ 3.1 &  0.43 $\pm$ 0.07 &          38.6 &            13.8 &             21.9 \\
 36 &  285.4499 &  1.1909 &   86 &         10.7 &          8.4 &   0.29 $^{+0.01}_{-0.02}$ &    82.2 &          17.5 &  20.9 $\pm$ 0.9 &  0.38 $\pm$ 0.02 &          42.7 &            14.3 &             21.9 \\
 37 &  285.4214 &  1.1969 &  159 &         31.6 &         15.2 &   0.68 $^{+0.31}_{-0.22}$ &   475.1 &         122.8 &  15.0 $\pm$ 0.7 &  0.43 $\pm$ 0.02 &          40.0 &            14.2 &             21.9 \\
 38 &  285.2161 &  1.1924 &  169 &         18.4 &         11.0 &   0.43 $^{+0.15}_{-0.08}$ &   172.8 &          32.8 &  15.3 $\pm$ 1.7 &  0.25 $\pm$ 0.03 &          39.1 &            13.9 &             21.9 \\
 39 &  284.4195 &  1.1954 &  188 &         13.8 &          6.5 &   0.27 $^{+0.11}_{-0.11}$ &    64.1 &           6.4 &  16.3 $\pm$ 3.3 &   0.59 $\pm$ 0.1 &          46.8 &            13.9 &             22.0 \\
 40 &  285.3170 &  1.2074 &  185 &         24.7 &         16.1 &   0.64 $^{+0.28}_{-0.23}$ &   712.4 &         313.8 &  16.9 $\pm$ 0.7 &  0.76 $\pm$ 0.02 &          41.5 &            14.5 &             22.0 \\
 41 &  285.3434 &  1.2036 &  167 &         13.8 &          8.2 &   0.31 $^{+0.04}_{-0.09}$ &   113.1 &          10.1 &  14.5 $\pm$ 1.0 &  0.49 $\pm$ 0.03 &          41.2 &            14.2 &             22.0 \\
 42 &  284.4387 &  1.2080 &  153 &         19.4 &         12.4 &     0.4 $^{+0.32}_{-0.2}$ &   137.3 &          18.7 &  14.5 $\pm$ 2.1 &  0.43 $\pm$ 0.05 &          47.6 &            14.0 &             22.0 \\
 43 &  284.4575 &  1.2148 &   61 &         16.4 &         11.7 &   0.35 $^{+0.17}_{-0.21}$ &   109.4 &          20.1 &  13.2 $\pm$ 2.7 &  0.92 $\pm$ 0.12 &          46.9 &            14.1 &             22.0 \\
 44 &  285.4257 &  1.2243 &  193 &         32.4 &         17.4 &    0.85 $^{+0.3}_{-0.35}$ &  1719.3 &        1226.3 &  23.4 $\pm$ 0.6 &  0.77 $\pm$ 0.02 &          42.7 &            14.7 &             21.9 \\
 45 &  285.2580 &  1.2245 &  223 &         25.7 &         14.2 &   0.56 $^{+0.27}_{-0.18}$ &   470.3 &         163.5 &  14.3 $\pm$ 1.1 &  0.59 $\pm$ 0.03 &          40.9 &            14.1 &             21.9 \\
 46 &  284.3109 &  1.2269 &  199 &         15.2 &         12.3 &   0.45 $^{+0.08}_{-0.03}$ &   163.4 &          43.1 &  11.3 $\pm$ 1.4 &  0.19 $\pm$ 0.02 &          11.6 &            14.0 &             22.0 \\
 47 &  285.4533 &  1.2264 &  156 &          9.1 &          7.8 &  0.25 $^{+-0.01}_{-0.01}$ &    93.2 &          31.1 &  30.0 $\pm$ 2.3 &   1.0 $\pm$ 0.06 &          44.0 &            14.0 &             21.9 \\
 48 &  284.4150 &  1.2401 &  145 &         27.5 &         17.4 &    0.6 $^{+0.26}_{-0.24}$ &   438.5 &         100.4 &  14.8 $\pm$ 2.4 &  0.86 $\pm$ 0.09 &          45.2 &            13.6 &             22.0 \\
 49 &  285.4763 &  1.2349 &  167 &         17.1 &          7.5 &   0.31 $^{+0.12}_{-0.15}$ &    55.8 &          11.8 &  18.6 $\pm$ 2.8 &  0.57 $\pm$ 0.08 &          42.7 &            13.9 &             21.8 \\
 50 &  285.3914 &  1.2429 &  205 &         17.7 &         11.7 &    0.42 $^{+0.12}_{-0.1}$ &   112.9 &          24.9 &  20.4 $\pm$ 2.2 &  0.54 $\pm$ 0.06 &          43.0 &            13.5 &             21.9 \\
 51 &  285.2790 &  1.2405 &  168 &         16.3 &          9.6 &   0.34 $^{+0.16}_{-0.08}$ &    99.1 &          13.7 &  16.0 $\pm$ 3.1 &  1.36 $\pm$ 0.17 &          39.6 &            14.4 &             21.9 \\
 52 &  285.3126 &  1.2493 &  210 &         12.1 &          8.7 &   0.27 $^{+0.12}_{-0.03}$ &    76.5 &           7.8 &  14.3 $\pm$ 2.3 &  0.83 $\pm$ 0.09 &          36.5 &            13.5 &             21.9 \\
 53 &  285.2771 &  1.2525 &  141 &         12.8 &          9.1 &   0.31 $^{+0.07}_{-0.06}$ &    76.3 &          13.8 &  16.5 $\pm$ 2.1 &  0.53 $\pm$ 0.06 &          40.6 &            13.6 &             21.9 \\
 54 &  285.3161 &  1.2638 &  124 &         18.7 &         13.7 &    0.48 $^{+0.18}_{-0.1}$ &   348.6 &          91.9 &  14.8 $\pm$ 1.6 &  0.85 $\pm$ 0.06 &          36.7 &            13.8 &             21.9 \\
 55 &  284.3729 &  1.2631 &   75 &         12.4 &          8.9 &   0.31 $^{+0.04}_{-0.02}$ &   100.6 &           5.7 &  15.0 $\pm$ 2.7 &  0.36 $\pm$ 0.05 &          46.2 &            13.7 &             22.0 \\
 56 &  284.4186 &  1.2734 &  115 &         22.1 &         14.7 &   0.53 $^{+0.14}_{-0.12}$ &   390.4 &          65.6 &  13.4 $\pm$ 2.2 &  0.84 $\pm$ 0.08 &          43.5 &            13.6 &             22.0 \\
 57 &  284.2771 &  1.2796 &  174 &         50.1 &         18.3 &    1.0 $^{+0.98}_{-0.51}$ &  1095.0 &         454.6 &  16.2 $\pm$ 1.5 &  0.45 $\pm$ 0.04 &          46.2 &            14.0 &             22.0 \\
 58 &  285.3412 &  1.2877 &   99 &         22.3 &          7.9 &   0.31 $^{+0.37}_{-0.28}$ &    61.3 &          12.9 &  14.3 $\pm$ 3.9 &  1.06 $\pm$ 0.21 &          42.1 &            14.6 &             21.9 \\
 59 &  284.3859 &  1.2889 &   61 &         25.9 &         16.8 &   0.59 $^{+0.46}_{-0.16}$ &   384.6 &          58.8 &  13.1 $\pm$ 1.8 &  0.59 $\pm$ 0.05 &          44.3 &            14.1 &             22.0 \\
 60 &  284.3256 &  1.2931 &   47 &         24.6 &         15.1 &     0.6 $^{+0.37}_{-0.1}$ &   428.4 &          69.6 &  12.5 $\pm$ 2.4 &  0.53 $\pm$ 0.06 &          45.3 &            13.9 &             22.0 \\
 61 &  284.3615 &  1.2926 &  225 &         14.8 &          6.2 &    0.28 $^{+0.16}_{-0.1}$ &    79.4 &           6.2 &  14.9 $\pm$ 3.1 &   0.58 $\pm$ 0.1 &          43.2 &            13.9 &             22.0 \\
 62 &  284.1749 &  1.2925 &   97 &         15.1 &          6.2 &   0.27 $^{+0.17}_{-0.11}$ &    47.4 &           4.1 &  16.4 $\pm$ 3.1 &  0.84 $\pm$ 0.12 &          40.8 &            14.1 &             22.0 \\
 63 &  284.3504 &  1.3022 &  176 &         13.0 &          9.6 &   0.31 $^{+0.03}_{-0.15}$ &    99.2 &          14.2 &  12.3 $\pm$ 3.4 &  0.77 $\pm$ 0.11 &          44.3 &            14.0 &             22.0 \\
 64 &  284.2068 &  1.3114 &  211 &         44.6 &         12.6 &   0.67 $^{+0.55}_{-0.43}$ &   726.8 &         266.6 &  15.4 $\pm$ 0.5 &  0.54 $\pm$ 0.01 &          44.6 &            14.5 &             22.0 \\
 65 &  284.2929 &  1.3132 &  191 &         20.0 &         18.9 &    0.6 $^{+0.27}_{-0.16}$ &   372.8 &          78.6 &  12.6 $\pm$ 1.9 &  0.44 $\pm$ 0.04 &          47.1 &            14.1 &             22.0 \\
 66 &  285.5802 &  1.3111 &  224 &         16.8 &          6.6 &    0.3 $^{+0.14}_{-0.11}$ &    47.7 &           8.5 &  22.0 $\pm$ 2.7 &  0.41 $\pm$ 0.05 &          40.7 &            14.0 &             21.5 \\
 67 &  284.2398 &  1.3149 &   88 &         16.8 &         13.1 &   0.46 $^{+0.07}_{-0.04}$ &   308.4 &          63.6 &  14.5 $\pm$ 0.4 &  0.59 $\pm$ 0.01 &          45.3 &            14.7 &             22.0 \\
 68 &  284.1739 &  1.3171 &  122 &          9.6 &          8.6 &   0.25 $^{+0.05}_{-0.03}$ &    40.9 &           3.9 &  18.8 $\pm$ 3.8 &   0.8 $\pm$ 0.14 &          41.8 &            13.5 &             22.0 \\
 69 &  285.5585 &  1.3447 &   45 &         45.9 &         15.1 &   0.77 $^{+0.63}_{-0.48}$ &   547.5 &         237.2 &  18.4 $\pm$ 1.4 &  0.45 $\pm$ 0.03 &          42.2 &            14.0 &             21.6 \\
 70 &  284.2817 &  1.3348 &  146 &         19.5 &         14.2 &   0.51 $^{+0.37}_{-0.18}$ &   240.8 &          34.1 &  14.1 $\pm$ 2.1 &  0.48 $\pm$ 0.06 &          46.8 &            14.1 &             22.0 \\
 71 &  285.4941 &  1.3584 &   47 &         12.4 &          7.3 &   0.28 $^{+0.07}_{-0.08}$ &    41.2 &           9.2 &  16.2 $\pm$ 3.3 &  0.32 $\pm$ 0.06 &          42.2 &            13.8 &             21.6 \\
 72 &  284.1919 &  1.3637 &  109 &         21.5 &          6.5 &   0.33 $^{+0.26}_{-0.12}$ &   132.6 &          11.1 &  16.2 $\pm$ 0.7 &  0.73 $\pm$ 0.03 &          42.4 &            14.3 &             22.0 \\
 73 &  285.5307 &  1.3632 &  218 &         11.1 &          7.4 &   0.26 $^{+0.08}_{-0.06}$ &    58.1 &           6.3 &  16.2 $\pm$ 1.3 &  0.31 $\pm$ 0.03 &          43.4 &            14.0 &             21.6 \\
 74 &  285.5112 &  1.3690 &  181 &         19.0 &         11.1 &   0.46 $^{+0.15}_{-0.08}$ &   195.8 &          48.5 &  14.2 $\pm$ 0.8 &  0.31 $\pm$ 0.02 &          43.7 &            14.1 &             21.6 \\
 75 &  284.2259 &  1.3757 &  137 &         15.6 &          7.4 &    0.32 $^{+0.1}_{-0.08}$ &   117.3 &          13.5 &  13.3 $\pm$ 2.7 &  0.47 $\pm$ 0.07 &          47.8 &            13.9 &             22.0 \\
 76 &  284.1989 &  1.3917 &  204 &         31.7 &         19.6 &   0.75 $^{+0.28}_{-0.27}$ &   937.5 &         295.5 &  15.1 $\pm$ 0.5 &  0.74 $\pm$ 0.02 &          41.7 &            14.6 &             22.0 \\
 77 &  284.2040 &  1.4298 &   75 &          9.9 &          7.9 &   0.27 $^{+-0.0}_{-0.05}$ &    45.0 &           3.7 &  13.8 $\pm$ 3.1 &  0.55 $\pm$ 0.09 &          41.4 &            14.1 &             22.0 \\
 78 &  284.6071 &  1.5266 &   66 &         35.0 &         16.5 &   0.79 $^{+0.35}_{-0.22}$ &   430.2 &         104.4 &  11.7 $\pm$ 1.4 &  0.26 $\pm$ 0.02 &          35.7 &            14.1 &             21.9 \\
 79 &  284.5908 &  1.5147 &   48 &         12.5 &          6.4 &   0.24 $^{+0.08}_{-0.09}$ &    38.2 &           2.6 &  11.9 $\pm$ 2.4 &  0.14 $\pm$ 0.02 &          34.8 &            13.9 &             21.9 \\
 80 &  284.5755 &  1.5473 &  208 &         32.4 &         25.3 &   0.86 $^{+0.36}_{-0.34}$ &   812.2 &         279.7 &  13.0 $\pm$ 1.4 &  0.41 $\pm$ 0.03 &          32.7 &            14.1 &             22.0 \\
 81 &  284.5425 &  1.5360 &   94 &         15.7 &          9.6 &   0.34 $^{+0.12}_{-0.21}$ &    67.0 &           5.2 &  10.6 $\pm$ 3.2 &   0.2 $\pm$ 0.04 &          32.0 &            13.9 &             22.0 \\
 82 &  284.5441 &  1.5694 &  208 &         28.9 &         17.0 &   0.68 $^{+0.22}_{-0.33}$ &   536.0 &         138.8 &  19.9 $\pm$ 2.1 &   0.5 $\pm$ 0.05 &          35.0 &            13.6 &             22.1 \\
 83 &  284.6235 &  1.5801 &   84 &         11.5 &          9.9 &   0.31 $^{+0.05}_{-0.03}$ &    81.8 &           9.3 &  14.5 $\pm$ 2.9 &  0.27 $\pm$ 0.05 &          34.2 &            13.7 &             22.0 \\
 84 &  284.6107 &  1.6049 &   99 &         29.6 &         20.2 &    0.8 $^{+0.31}_{-0.16}$ &   649.3 &         243.7 &  14.0 $\pm$ 1.8 &  0.46 $\pm$ 0.04 &          31.6 &            14.0 &             22.1 \\
 85 &  284.5700 &  1.5962 &  157 &         17.3 &         11.4 &    0.4 $^{+0.24}_{-0.06}$ &   149.9 &          21.2 &  13.0 $\pm$ 2.9 &  0.42 $\pm$ 0.07 &          32.0 &            13.6 &             22.1 \\
 86 &  284.4820 &  1.6022 &   52 &         21.5 &         16.1 &   0.46 $^{+0.26}_{-0.27}$ &   138.6 &          10.4 &  24.6 $\pm$ 4.0 &  0.77 $\pm$ 0.11 &          34.4 &            13.8 &             22.1 \\
 87 &  284.5391 &  1.6197 &  134 &         33.6 &         29.2 &   0.99 $^{+0.49}_{-0.34}$ &  4451.6 &        2672.0 &  20.1 $\pm$ 0.3 &  1.43 $\pm$ 0.01 &          33.2 &            14.9 &             22.2 \\
 88 &  284.4939 &  1.6315 &   99 &         20.2 &          8.6 &   0.31 $^{+0.15}_{-0.23}$ &    62.8 &           9.1 &  11.3 $\pm$ 4.2 &  0.75 $\pm$ 0.12 &          33.4 &            14.1 &             22.1 \\
 89 &  284.5149 &  1.6483 &  151 &         20.0 &         12.5 &   0.51 $^{+0.07}_{-0.16}$ &   235.2 &          54.6 &  15.3 $\pm$ 1.7 &  0.53 $\pm$ 0.05 &          31.9 &            14.1 &             22.1 \\
 90 &  284.5529 &  1.6751 &  223 &         35.7 &         15.1 &   0.71 $^{+0.47}_{-0.25}$ &  1939.1 &        1027.7 &  22.2 $\pm$ 0.3 &  0.97 $\pm$ 0.01 &          33.8 &            14.9 &             22.2 \\
 91 &  284.5859 &  1.6797 &   59 &         32.6 &         12.3 &    0.6 $^{+0.46}_{-0.23}$ &   613.3 &         250.1 &  13.1 $\pm$ 0.6 &  0.39 $\pm$ 0.01 &          35.7 &            14.4 &             22.1 \\
 92 &  284.5187 &  1.6695 &  119 &         13.5 &          9.4 &   0.35 $^{+0.08}_{-0.04}$ &   102.1 &          20.1 &  13.9 $\pm$ 1.6 &   0.4 $\pm$ 0.04 &          33.2 &            13.9 &             22.1 \\
 93 &  284.6399 &  1.6874 &   95 &         26.8 &         19.4 &    0.66 $^{+0.3}_{-0.17}$ &   466.4 &         156.9 &  11.6 $\pm$ 1.4 &  0.32 $\pm$ 0.03 &          36.5 &            14.2 &             22.0 \\
 94 &  284.6094 &  1.6806 &  199 &         18.8 &          9.8 &    0.41 $^{+0.19}_{-0.1}$ &   149.5 &          24.6 &  10.3 $\pm$ 1.4 &  0.25 $\pm$ 0.02 &          35.1 &            14.2 &             22.1 \\
 95 &  284.6564 &  1.6999 &  131 &         14.5 &          9.6 &    0.27 $^{+0.19}_{-0.2}$ &    68.8 &           6.2 &  12.7 $\pm$ 2.8 &  0.33 $\pm$ 0.05 &          36.4 &            14.0 &             22.0 \\
 96 &  284.5964 &  1.7045 &   85 &         12.1 &          8.8 &    0.3 $^{+0.04}_{-0.06}$ &    82.1 &           8.1 &  15.9 $\pm$ 3.3 &  0.41 $\pm$ 0.07 &          36.3 &            13.7 &             22.1 \\
 97 &  284.6133 &  1.7210 &  180 &         23.8 &         18.5 &   0.66 $^{+0.29}_{-0.15}$ &   414.6 &         102.1 &  12.2 $\pm$ 1.7 &  0.35 $\pm$ 0.04 &          37.1 &            14.1 &             22.1 \\
 98 &  284.6143 &  1.7476 &  126 &         14.3 &          7.2 &    0.3 $^{+0.14}_{-0.07}$ &    80.2 &           5.3 &  13.0 $\pm$ 1.3 &  0.18 $\pm$ 0.02 &          38.2 &            14.1 &             22.0 \\
 99 &  284.6256 &  1.7783 &  223 &         31.4 &         11.2 &   0.46 $^{+0.49}_{-0.41}$ &   231.9 &          50.2 &  13.7 $\pm$ 2.7 &  0.71 $\pm$ 0.09 &          37.9 &            13.8 &             21.9 \\
\bottomrule
\end{tabular}


==> W48_leaf_stats_virial.tex <==
\begin{tabular}{rrrrrrrrllrr}
\toprule
 ID &  $\alpha_{vir}$ &  $M_{vir}$ &  $\sigma_{nt}$ & log$|\Omega_G|$ & log$\Omega_K$ & log$|\Omega_{Pw}|$ &  log$|\Omega_{Pt}|$ & on-filament & hub & $N_{proto}$ & Bad N(H$_2$) Pixels \\& & (M$_\odot$) & (km s$^{-1}$) & (erg) & (erg) & (erg) & (erg) & & & \\\midrule
  0 &   0.30 &              37.8 &      0.27 &  45.4 &     44.6 &     45.6 &         NaN &         True &  False &           0 &      0.00 \\
  1 &   1.57 &             152.1 &      0.66 &  45.2 &     45.1 &     45.6 &         NaN &         True &  False &           0 &      0.00 \\
  2 &   0.53 &              63.7 &      0.32 &  45.2 &     44.7 &     45.9 &         NaN &        False &  False &           0 &      0.00 \\
  3 &   0.30 &             300.0 &      0.65 &  46.9 &     46.2 &     46.6 &         NaN &         True &  False &           3 &      0.00 \\
  4 &   0.66 &              52.5 &      0.36 &  45.0 &     44.6 &     45.4 &         NaN &         True &  False &           0 &      0.00 \\
  5 &   1.64 &              98.0 &      0.62 &  44.9 &     44.9 &     45.1 &         NaN &         True &  False &           0 &      0.00 \\
  6 &   0.21 &             393.4 &      0.67 &  47.3 &     46.5 &     46.8 &         NaN &        False &   True &           8 &      0.00 \\
  7 &   1.42 &              79.5 &      0.49 &  44.7 &     44.7 &     45.4 &         NaN &         True &  False &           1 &      0.00 \\
  8 &   0.43 &              77.9 &      0.32 &  45.5 &     44.9 &     46.1 &         NaN &        False &  False &           2 &      0.00 \\
  9 &   0.21 &             161.6 &      0.37 &  46.5 &     45.6 &     46.9 &         NaN &         True &  False &           2 &      0.00 \\
 10 &   1.38 &              62.6 &      0.49 &  44.6 &     44.6 &     45.1 &         NaN &         True &  False &           0 &      0.00 \\
 11 &   0.35 &              53.0 &      0.30 &  45.4 &     44.8 &     45.8 &         NaN &        False &  False &           0 &      0.00 \\
 12 &   0.28 &              35.9 &      0.23 &  45.3 &     44.5 &     45.9 &         NaN &        False &  False &           0 &      0.00 \\
 13 &   0.32 &              52.8 &      0.26 &  45.5 &     44.8 &     46.0 &         NaN &        False &  False &           1 &      0.00 \\
 14 &   1.63 &             155.4 &      0.65 &  45.1 &     45.1 &     45.6 &         NaN &        False &  False &           0 &      0.00 \\
 15 &   0.43 &              75.0 &      0.41 &  45.6 &     45.0 &     45.7 &         NaN &         True &  False &           1 &      0.00 \\
 16 &   0.16 &              89.0 &      0.25 &  46.3 &     45.3 &     46.8 &         NaN &        False &  False &           2 &      0.00 \\
 17 &   0.52 &              82.1 &      0.38 &  45.4 &     45.0 &     45.9 &         NaN &         True &  False &           1 &      0.00 \\
 18 &   0.51 &              35.6 &      0.32 &  45.0 &     44.5 &     45.3 &         NaN &         True &  False &           0 &      0.00 \\
 19 &   1.05 &              66.1 &      0.41 &  44.8 &     44.6 &     45.5 &         NaN &        False &  False &           0 &      0.00 \\
 20 &   1.09 &             164.2 &      0.59 &  45.4 &     45.3 &     45.9 &         NaN &        False &  False &           0 &      0.00 \\
 21 &   0.38 &              27.6 &      0.21 &  44.9 &     44.3 &     45.6 &         NaN &        False &  False &           0 &      0.00 \\
 22 &   0.30 &             171.6 &      0.48 &  46.4 &     45.7 &     46.4 &         NaN &         True &  False &           1 &      0.00 \\
 23 &   0.42 &              21.9 &      0.17 &  44.6 &     44.0 &     45.1 &         NaN &        False &  False &           0 &      0.00 \\
 24 &   5.38 &             343.6 &      1.11 &  44.9 &     45.4 &     45.4 &         NaN &        False &  False &           0 &      0.00 \\
 25 &   1.66 &             474.4 &      1.01 &  45.9 &     46.0 &     46.1 &         NaN &        False &  False &           1 &      0.00 \\
 26 &   0.42 &              87.5 &      0.38 &  45.7 &     45.1 &     46.0 &         NaN &        False &  False &           0 &      0.00 \\
 27 &   8.35 &             424.3 &      1.36 &  44.7 &     45.5 &     45.1 &         NaN &        False &  False &           0 &      0.00 \\
 28 &   0.58 &              63.2 &      0.38 &  45.3 &     44.8 &     45.5 &         NaN &         True &  False &           0 &      0.00 \\
 29 &   0.53 &             564.9 &      0.81 &  46.8 &     46.3 &     46.8 &         NaN &        False &  False &           5 &      0.00 \\
 30 &   0.29 &              80.0 &      0.37 &  45.9 &     45.2 &     46.1 &         NaN &        False &  False &           0 &      0.00 \\
 31 &   0.94 &             183.7 &      0.58 &  45.6 &     45.4 &     46.0 &         NaN &        False &  False &           0 &      0.00 \\
 32 &   0.51 &              27.0 &      0.22 &  44.7 &     44.2 &     45.3 &         NaN &         True &  False &           0 &      0.00 \\
 33 &   0.43 &              52.3 &      0.37 &  45.4 &     44.8 &     45.5 &         NaN &        False &  False &           0 &      0.00 \\
 34 &   0.36 &             113.2 &      0.48 &  46.1 &     45.4 &     45.9 &         NaN &        False &  False &           1 &      0.00 \\
 35 &   1.04 &              66.3 &      0.42 &  44.8 &     44.6 &     45.4 &         NaN &        False &  False &           0 &      0.00 \\
 36 &   0.69 &              56.4 &      0.37 &  45.1 &     44.7 &     45.3 &         NaN &         True &  False &           0 &      0.00 \\
 37 &   0.30 &             143.4 &      0.42 &  46.2 &     45.5 &     46.5 &         NaN &        False &  False &           0 &      0.00 \\
 38 &   0.25 &              42.7 &      0.23 &  45.6 &     44.7 &     45.9 &         NaN &        False &  False &           0 &      0.00 \\
 39 &   1.55 &              99.2 &      0.58 &  44.9 &     44.9 &     45.3 &         NaN &         True &  False &           0 &      0.00 \\
 40 &   0.52 &             371.7 &      0.75 &  46.6 &     46.1 &     46.5 &         NaN &        False &  False &           6 &      0.00 \\
 41 &   0.73 &              82.2 &      0.48 &  45.3 &     45.0 &     45.6 &         NaN &        False &  False &           0 &      0.00 \\
 42 &   0.61 &              84.1 &      0.42 &  45.4 &     45.0 &     45.8 &         NaN &         True &  False &           0 &      0.00 \\
 43 &   2.59 &             283.2 &      0.91 &  45.2 &     45.5 &     45.6 &         NaN &         True &  False &           0 &      0.00 \\
 44 &   0.31 &             531.4 &      0.77 &  47.3 &     46.5 &     46.8 &         NaN &        False &   True &           4 &      0.01 \\
 45 &   0.44 &             208.5 &      0.59 &  46.3 &     45.7 &     46.3 &         NaN &        False &  False &           1 &      0.00 \\
 46 &   0.18 &              29.9 &      0.18 &  45.5 &     44.5 &     46.0 &         NaN &        False &  False &           1 &      0.00 \\
 47 &   2.71 &             252.9 &      0.99 &  45.3 &     45.5 &     45.1 &         NaN &         True &  False &           0 &      0.00 \\
 48 &   1.00 &             439.6 &      0.86 &  46.2 &     46.0 &     46.4 &         NaN &         True &  False &           0 &      0.00 \\
 49 &   1.98 &             110.4 &      0.56 &  44.7 &     44.8 &     45.4 &         NaN &         True &  False &           0 &      0.00 \\
 50 &   1.21 &             136.5 &      0.53 &  45.2 &     45.1 &     45.9 &         NaN &        False &  False &           0 &      0.00 \\
 51 &   6.05 &             599.3 &      1.36 &  45.2 &     45.8 &     45.6 &         NaN &        False &  False &           0 &      0.00 \\
 52 &   2.43 &             185.6 &      0.83 &  45.0 &     45.2 &     45.3 &         NaN &        False &  False &           0 &      0.00 \\
 53 &   1.27 &              97.1 &      0.52 &  45.0 &     44.9 &     45.5 &         NaN &        False &  False &           0 &      0.00 \\
 54 &   0.98 &             342.8 &      0.85 &  46.1 &     45.9 &     46.0 &         NaN &        False &  False &           0 &      0.00 \\
 55 &   0.50 &              50.6 &      0.35 &  45.2 &     44.7 &     45.6 &         NaN &         True &  False &           0 &      0.00 \\
 56 &   0.93 &             364.4 &      0.84 &  46.2 &     45.9 &     46.3 &         NaN &         True &  False &           0 &      0.00 \\
 57 &   0.21 &             233.2 &      0.44 &  46.8 &     45.9 &     47.1 &         NaN &         True &  False &           3 &      0.00 \\
 58 &   5.42 &             331.9 &      1.06 &  44.8 &     45.3 &     45.4 &         NaN &        False &  False &           0 &      0.00 \\
 59 &   0.56 &             215.7 &      0.59 &  46.1 &     45.7 &     46.4 &         NaN &         True &  False &           2 &      0.00 \\
 60 &   0.42 &             178.9 &      0.53 &  46.2 &     45.6 &     46.4 &         NaN &         True &  False &           0 &      0.00 \\
 61 &   1.26 &             100.3 &      0.58 &  45.1 &     45.0 &     45.4 &         NaN &         True &  False &           0 &      0.00 \\
 62 &   4.04 &             191.7 &      0.84 &  44.6 &     45.0 &     45.3 &         NaN &        False &  False &           0 &      0.00 \\
 63 &   1.85 &             183.4 &      0.76 &  45.2 &     45.3 &     45.6 &         NaN &         True &  False &           0 &      0.00 \\
 64 &   0.29 &             209.5 &      0.53 &  46.6 &     45.9 &     46.5 &         NaN &         True &  False &           1 &      0.00 \\
 65 &   0.35 &             129.7 &      0.43 &  46.1 &     45.4 &     46.4 &         NaN &         True &  False &           1 &      0.00 \\
 66 &   1.36 &              64.9 &      0.40 &  44.6 &     44.5 &     45.0 &         NaN &         True &  False &           0 &      0.00 \\
 67 &   0.54 &             167.0 &      0.58 &  46.0 &     45.6 &     46.1 &         NaN &         True &  False &           1 &      0.00 \\
 68 &   4.00 &             163.3 &      0.80 &  44.5 &     44.9 &     45.2 &         NaN &        False &  False &           0 &      0.00 \\
 69 &   0.34 &             187.9 &      0.44 &  46.3 &     45.6 &     46.3 &         NaN &         True &  False &           3 &      0.00 \\
 70 &   0.54 &             130.5 &      0.48 &  45.8 &     45.3 &     46.2 &         NaN &         True &  False &           0 &      0.00 \\
 71 &   0.94 &              38.7 &      0.30 &  44.5 &     44.3 &     45.0 &         NaN &         True &  False &           0 &      0.00 \\
 72 &   1.36 &             180.9 &      0.73 &  45.4 &     45.4 &     45.6 &         NaN &         True &  False &           0 &      0.00 \\
 73 &   0.61 &              35.4 &      0.30 &  44.8 &     44.4 &     44.9 &         NaN &         True &  False &           0 &      0.00 \\
 74 &   0.30 &              59.3 &      0.30 &  45.6 &     44.9 &     45.7 &         NaN &         True &  False &           2 &      0.00 \\
 75 &   0.67 &              78.5 &      0.46 &  45.3 &     45.0 &     45.6 &         NaN &         True &  False &           0 &      0.00 \\
 76 &   0.44 &             409.6 &      0.73 &  46.8 &     46.2 &     46.7 &         NaN &         True &  False &           0 &      0.00 \\
 77 &   1.91 &              86.0 &      0.54 &  44.6 &     44.7 &     45.3 &         NaN &        False &  False &           0 &      0.00 \\
 78 &   0.18 &              76.8 &      0.25 &  46.1 &     45.1 &     46.7 &         NaN &         True &  False &           0 &      0.00 \\
 79 &   0.33 &              12.6 &      0.12 &  44.5 &     43.8 &     45.1 &         NaN &         True &  False &           0 &      0.00 \\
 80 &   0.21 &             166.5 &      0.40 &  46.6 &     45.7 &     46.9 &         NaN &         True &  False &           4 &      0.00 \\
 81 &   0.34 &              23.0 &      0.19 &  44.8 &     44.2 &     45.7 &         NaN &        False &  False &           0 &      0.00 \\
 82 &   0.37 &             195.8 &      0.49 &  46.3 &     45.7 &     46.6 &         NaN &         True &  False &           3 &      0.00 \\
 83 &   0.41 &              33.5 &      0.25 &  45.0 &     44.4 &     45.6 &         NaN &        False &  False &           0 &      0.00 \\
 84 &   0.29 &             188.0 &      0.45 &  46.4 &     45.7 &     46.8 &         NaN &        False &  False &           4 &      0.00 \\
 85 &   0.54 &              80.6 &      0.42 &  45.5 &     45.0 &     46.0 &         NaN &        False &  False &           0 &      0.00 \\
 86 &   2.09 &             290.4 &      0.77 &  45.3 &     45.4 &     46.1 &         NaN &        False &  False &           0 &      0.00 \\
 87 &   0.44 &            1939.2 &      1.43 &  48.0 &     47.4 &     47.2 &         NaN &        False &   True &           5 &      0.00 \\
 88 &   2.72 &             170.7 &      0.75 &  44.8 &     45.1 &     45.6 &         NaN &        False &  False &           0 &      0.00 \\
 89 &   0.66 &             155.0 &      0.52 &  45.7 &     45.4 &     46.3 &         NaN &        False &  False &           0 &      0.00 \\
 90 &   0.34 &             667.8 &      0.97 &  47.4 &     46.8 &     46.8 &         NaN &        False &   True &           2 &      0.00 \\
 91 &   0.18 &             108.0 &      0.38 &  46.5 &     45.5 &     46.5 &         NaN &        False &  False &           2 &      0.00 \\
 92 &   0.63 &              64.2 &      0.39 &  45.2 &     44.8 &     45.8 &         NaN &        False &  False &           0 &      0.00 \\
 93 &   0.18 &              85.1 &      0.31 &  46.2 &     45.3 &     46.6 &         NaN &        False &  False &           1 &      0.00 \\
 94 &   0.24 &              36.2 &      0.24 &  45.4 &     44.6 &     46.0 &         NaN &        False &  False &           0 &      0.00 \\
 95 &   0.55 &              37.5 &      0.32 &  45.0 &     44.5 &     45.4 &         NaN &        False &  False &           0 &      0.00 \\
 96 &   0.72 &              58.9 &      0.40 &  45.1 &     44.7 &     45.6 &         NaN &         True &  False &           0 &      0.00 \\
 97 &   0.24 &              98.8 &      0.34 &  46.1 &     45.3 &     46.6 &         NaN &         True &  False &           0 &      0.00 \\
 98 &   0.25 &              20.3 &      0.17 &  45.0 &     44.2 &     45.5 &         NaN &         True &  False &           0 &      0.00 \\
 99 &   1.01 &             234.8 &      0.71 &  45.8 &     45.6 &     46.0 &         NaN &         True &  False &           1 &      0.00 \\
\bottomrule
\end{tabular}

